Stage-parallel fully implicit Runge-Kutta implementations with optimal multilevel preconditioners at the scaling limit

We present an implementation of a fully stage-parallel preconditioner for Radau IIA type fully implicit Runge--Kutta methods, which approximates the inverse of $A_Q$ from the Butcher tableau by the lower triangular matrix resulting from an LU decomposition and diagonalizes the system with as many blocks as stages. For the transformed system, we employ a block preconditioner where each block is distributed and solved by a subgroup of processes in parallel. For combination of partial results, we either use a communication pattern resembling Cannon's algorithm or shared memory. A performance model and a large set of performance studies (including strong scaling runs with up to 150k processes on 3k compute nodes) conducted for a time-dependent heat problem, using matrix-free finite element methods, indicate that the stage-parallel implementation can reach higher throughputs when the block solvers operate at lower parallel efficiencies, which occurs near the scaling limit. Achievable speedup increases linearly with number of stages and are bounded by the number of stages. Furthermore, we show that the presented stage-parallel concepts are also applicable to the case that $A_Q$ is directly diagonalized, which requires complex arithmetic or the solution of two-by-two blocks and sequentializes parts of the algorithm. Alternatively to distributing stages and assigning them to distinct processes, we discuss the possibility of batching operations from different stages together.

==> data/gmg-batched/data_0.tex <==
dofs t speedup
7.290000e+02 5.033600e-04 8.000000e+00
4.913000e+03 8.438100e-04 8.000000e+00
3.593700e+04 1.286400e-03 8.000000e+00
2.746250e+05 1.940800e-03 8.000000e+00
2.146689e+06 4.373300e-03 8.000000e+00
1.697459e+07 2.259600e-02 8.000000e+00


==> data/gmg-batched/data_1.tex <==
dofs t speedup
7.290000e+02 7.210300e-04 5.584899e+00
4.913000e+03 1.183000e-03 5.706238e+00
3.593700e+04 1.926200e-03 5.342747e+00
2.746250e+05 4.183200e-03 3.711608e+00
2.146689e+06 2.144300e-02 1.631600e+00
1.697459e+07 1.440800e-01 1.254636e+00


==> data/gmg-batched/data_2.tex <==
dofs t speedup
7.290000e+02 4.513000e-04 8.922845e+00
4.913000e+03 8.721000e-04 7.740488e+00
3.593700e+04 1.429300e-03 7.200168e+00
2.746250e+05 3.758500e-03 4.131010e+00
2.146689e+06 2.135700e-02 1.638170e+00
1.697459e+07 1.640400e-01 1.101975e+00


==> data/gmg-batched/data_3.tex <==
dofs t speedup
7.290000e+02 3.088900e-03 1.303661e+00
4.913000e+03 5.823600e-03 1.159159e+00
3.593700e+04 9.143300e-03 1.125545e+00
2.746250e+05 1.433900e-02 1.082809e+00
2.146689e+06 3.018600e-02 1.159027e+00
1.697459e+07 2.171300e-01 8.325335e-01


==> data/gmg-batched/plot_vs_a_3.tex <==
\begin{tikzpicture}[thick,scale=0.7, every node/.style={scale=0.75}]
  \begin{loglogaxis}[
    width=1.4\textwidth,
    height=1.2\textwidth,
    title style={font=\tiny},every axis title/.style={above left,at={(1,1)},draw=black,fill=white},
    title={$Q=8$},
    xlabel={DoFs},
    ylabel={Time per iterations [sec]},
    legend pos={south west},
    legend cell align={left},
    cycle list name=colorGPL,
    grid,
    semithick,
    mark options={solid}
    ]

\addplot+[solid, red,every mark/.append style={fill=blue!80!black},mark=o] table [x=dofs,y=t_0] {data/parameters-all/parameters-q/data_3.tex};
\addplot+[solid, blue,every mark/.append style={fill=blue!80!black},mark=x] table [x=dofs,y=t_1] {data/parameters-all/parameters-q/data_3.tex};
\addplot+[solid, orange,every mark/.append style={fill=orange!80!black},mark=square] table [x=dofs,y=t_2] {data/parameters-all/parameters-q/data_3.tex};


  \end{loglogaxis}
\end{tikzpicture}


==> data/gmg/data_0004_0.tex <==
ranks time dofs
1 3.263600e-04 1.518750e+01
2 3.096300e-04 7.593750e+00
4 3.299800e-04 3.796875e+00
8 3.267200e-04 1.898438e+00
16 3.322600e-04 9.492188e-01
32 3.848900e-04 4.746094e-01
64 3.475300e-04 2.373047e-01
128 3.599500e-04 1.186523e-01
256 4.590600e-04 5.932617e-02
512 4.615100e-04 2.966309e-02
1024 5.242900e-04 1.483154e-02
2048 5.251800e-04 7.415771e-03


==> data/gmg/data_0005_0.tex <==
ranks time dofs
1 5.025000e-04 1.023542e+02
2 6.034000e-04 5.117708e+01
4 6.133800e-04 2.558854e+01
8 6.533100e-04 1.279427e+01
16 6.199000e-04 6.397135e+00
32 5.998600e-04 3.198568e+00
64 6.256100e-04 1.599284e+00
128 6.105700e-04 7.996419e-01
256 6.509000e-04 3.998210e-01
512 7.057700e-04 1.999105e-01
1024 7.875600e-04 9.995524e-02
2048 7.601500e-04 4.997762e-02


==> data/gmg/data_0006_0.tex <==
ranks time dofs
1 1.200400e-03 7.486875e+02
2 1.041200e-03 3.743438e+02
4 9.641900e-04 1.871719e+02
8 9.340200e-04 9.358594e+01
16 8.812800e-04 4.679297e+01
32 9.124500e-04 2.339648e+01
64 9.175700e-04 1.169824e+01
128 8.543600e-04 5.849121e+00
256 9.916900e-04 2.924561e+00
512 9.842000e-04 1.462280e+00
1024 1.156600e-03 7.311401e-01
2048 1.129700e-03 3.655701e-01


==> data/gmg/data_0007_0.tex <==
ranks time dofs
1 5.555200e-03 5.721354e+03
2 3.294100e-03 2.860677e+03
4 2.188700e-03 1.430339e+03
8 1.705900e-03 7.151693e+02
16 1.416100e-03 3.575846e+02
32 1.320100e-03 1.787923e+02
64 1.267600e-03 8.939616e+01
128 1.368600e-03 4.469808e+01
256 1.655600e-03 2.234904e+01
512 1.898900e-03 1.117452e+01
1024 2.073600e-03 5.587260e+00
2048 1.634200e-03 2.793630e+00


==> data/gmg/data_0008_0.tex <==
ranks time dofs
1 3.809700e-02 4.472269e+04
2 2.092000e-02 2.236134e+04
4 1.088600e-02 1.118067e+04
8 6.127400e-03 5.590336e+03
16 3.695200e-03 2.795168e+03
32 2.735900e-03 1.397584e+03
64 2.326200e-03 6.987920e+02
128 2.114200e-03 3.493960e+02
256 2.422900e-03 1.746980e+02
512 2.571200e-03 8.734900e+01
1024 4.374200e-03 4.367450e+01
2048 5.284800e-03 2.183725e+01


==> data/gmg/data_0009_0.tex <==
ranks time dofs
1 3.050300e-01 3.536374e+05
2 1.518400e-01 1.768187e+05
4 7.595100e-02 8.840934e+04
8 4.050200e-02 4.420467e+04
16 2.151400e-02 2.210233e+04
32 1.239200e-02 1.105117e+04
64 7.208600e-03 5.525584e+03
128 4.984200e-03 2.762792e+03
256 4.096800e-03 1.381396e+03
512 3.588400e-03 6.906980e+02
1024 4.250100e-03 3.453490e+02
2048 5.396500e-03 1.726745e+02


==> data/gmg/data_0010_0.tex <==
ranks time dofs
4 6.077700e-01 7.031547e+05
8 3.120200e-01 3.515773e+05
16 1.658100e-01 1.757887e+05
32 8.424600e-02 8.789433e+04
64 4.887900e-02 4.394717e+04
128 2.389800e-02 2.197358e+04
256 1.480300e-02 1.098679e+04
512 9.360200e-03 5.493396e+03
1024 7.396400e-03 2.746698e+03
2048 6.034000e-03 1.373349e+03


==> data/gmg/data_0011_0.tex <==
ranks time dofs
32 6.286300e-01 7.011007e+05
64 3.271600e-01 3.505503e+05
128 1.686500e-01 1.752752e+05
256 8.487700e-02 8.763758e+04
512 4.523500e-02 4.381879e+04
1024 3.436300e-02 2.190940e+04
2048 1.835100e-02 1.095470e+04


==> data/gmg/data_0012_0.tex <==
ranks time dofs
256 6.702500e-01 7.000752e+05
512 3.490900e-01 3.500376e+05
1024 1.862900e-01 1.750188e+05
2048 8.795200e-02 8.750940e+04


==> data/gmg/data_0013_0.tex <==
ranks time dofs
2048 7.170900e-01 6.995628e+05


==> data/iterations-all/data_4.tex <==
\begin{tabular}{C{0.75cm}C{1.50cm}C{1.50cm}C{1.50cm}}
\hline
&\multicolumn{3}{c}{\textbf{non-complex} (Sections~\ref{sec:methods}--\ref{sec:performance})}\\ \hline
&\multicolumn{1}{c}{\textbf{IRK}}&\multicolumn{1}{c}{\textbf{SPIRK}}&\multicolumn{1}{c}{\textbf{batched}} \\ \hline
$Q$& \#G (\#V$^1$) & \#G (\#V$^1$) & \#G (\#V$^Q$) \\ \hline
2 & 6.0 (14.0) & 6.0 (7.0) & 6.0 (7.0)
\\
4 & 8.9 (39.6) & 8.9 (9.9) & 8.9 (9.9)
\\
6 & 11.9 (77.3) & 11.9 (12.9) & 11.9 (12.9)
\\
8 & 14.0 (120.0) & 14.0 (15.0) & 13.0 (14.0)
\\\hline
\end{tabular}

\vspace{0.2cm}

\begin{tabular}{C{0.75cm}C{2.00cm}C{2.0cm}C{2.50cm}C{2.5cm}}
\hline
&\multicolumn{4}{c}{\textbf{complex} (Section~\ref{sec:complex})} \\ \hline
&\multicolumn{1}{c}{\textbf{IRK-PRESB}}&\multicolumn{1}{c}{\textbf{IRK-GMG}}&\multicolumn{1}{c}{\textbf{SPIRK-PRESB}}&\multicolumn{1}{c}{\textbf{SPIRK-GMG}} \\ \hline
$Q$& \#G (\#V$^1$)& \#G (\#V$^2$)& \#G (\#V$^1$)& \#G (\#V$^2$) \\ \hline
2 & 6.0 (14.0) & 7.0 (8.0) & 6.0 (14.0) & 7.0 (8.0)
\\
4 & 13.6 (31.1) & 13.0 (15.0) & 6.6--7.0 (15.1--16.0) & 6.0--7.0 (7.0--8.0)
\\
6 & 22.0 (50.0) & 19.0 (22.0) & 7.0--8.0 (16.0--18.0) & 6.0--7.0 (7.0--8.0)
\\
8 & 29.9 (67.8) & 27.6 (31.6) & 6.0--8.0 (14.0--18.0) & 6.0--8.8 (7.0--9.8)
\\\hline
\end{tabular}


==> data/iterations-all/data_5.tex <==
\begin{tabular}{C{0.75cm}C{1.50cm}C{1.50cm}C{1.50cm}}
\hline
&\multicolumn{3}{c}{\textbf{non-complex} (Sections~\ref{sec:methods}--\ref{sec:performance})}\\ \hline
&\multicolumn{1}{c}{\textbf{IRK}}&\multicolumn{1}{c}{\textbf{SPIRK}}&\multicolumn{1}{c}{\textbf{batched}} \\ \hline
$Q$& \#G (\#V$^1$) & \#G (\#V$^1$) & \#G (\#V$^Q$) \\ \hline
2 & 6.0 (14.0) & 6.0 (7.0) & 6.0 (7.0)
\\
4 & 8.9 (39.6) & 8.9 (9.9) & 8.9 (9.9)
\\
6 & 11.0 (72.0) & 11.0 (12.0) & 10.9 (11.9)
\\
8 & 13.0 (112.0) & 13.0 (14.0) & 12.9 (13.9)
\\\hline
\end{tabular}

\vspace{0.2cm}

\begin{tabular}{C{0.75cm}C{2.00cm}C{2.0cm}C{2.50cm}C{2.5cm}}
\hline
&\multicolumn{4}{c}{\textbf{complex} (Section~\ref{sec:complex})} \\ \hline
&\multicolumn{1}{c}{\textbf{IRK-PRESB}}&\multicolumn{1}{c}{\textbf{IRK-GMG}}&\multicolumn{1}{c}{\textbf{SPIRK-PRESB}}&\multicolumn{1}{c}{\textbf{SPIRK-GMG}} \\ \hline
$Q$& \#G (\#V$^1$)& \#G (\#V$^2$)& \#G (\#V$^1$)& \#G (\#V$^2$) \\ \hline
2 & 6.0 (14.0) & 8.0 (9.0) & 6.0 (14.0) & 8.0 (9.0)
\\
4 & 13.3 (30.7) & 16.0 (18.0) & 6.0--7.3 (14.0--16.7) & 8.0--8.0 (9.0--9.0)
\\
6 & 21.0 (48.0) & 24.0 (27.0) & 6.0--8.0 (14.0--18.0) & 8.0--8.0 (9.0--9.0)
\\
8 & 29.7 (67.3) & 32.8 (36.8) & 6.0--8.7 (14.0--19.3) & 7.0--9.6 (8.0--10.6)
\\\hline
\end{tabular}


==> data/iterations-all/data_6.tex <==
\begin{tabular}{C{0.75cm}C{1.50cm}C{1.50cm}C{1.50cm}}
\hline
&\multicolumn{3}{c}{\textbf{non-complex} (Sections~\ref{sec:methods}--\ref{sec:performance})}\\ \hline
&\multicolumn{1}{c}{\textbf{IRK}}&\multicolumn{1}{c}{\textbf{SPIRK}}&\multicolumn{1}{c}{\textbf{batched}} \\ \hline
$Q$& \#G (\#V$^1$) & \#G (\#V$^1$) & \#G (\#V$^Q$) \\ \hline
2 & 6.0 (14.0) & 6.0 (7.0) & 6.0 (7.0)
\\
4 & 7.9 (35.6) & 7.9 (8.9) & 7.9 (8.9)
\\
6 & 9.9 (65.3) & 9.9 (10.9) & 9.9 (10.9)
\\
8 & 11.9 (103.1) & 11.9 (12.9) & 11.9 (12.9)
\\\hline
\end{tabular}

\vspace{0.2cm}

\begin{tabular}{C{0.75cm}C{2.00cm}C{2.0cm}C{2.50cm}C{2.5cm}}
\hline
&\multicolumn{4}{c}{\textbf{complex} (Section~\ref{sec:complex})} \\ \hline
&\multicolumn{1}{c}{\textbf{IRK-PRESB}}&\multicolumn{1}{c}{\textbf{IRK-GMG}}&\multicolumn{1}{c}{\textbf{SPIRK-PRESB}}&\multicolumn{1}{c}{\textbf{SPIRK-GMG}} \\ \hline
$Q$& \#G (\#V$^1$)& \#G (\#V$^2$)& \#G (\#V$^1$)& \#G (\#V$^2$) \\ \hline
2 & 6.0 (14.0) & 8.0 (9.0) & 6.0 (14.0) & 8.0 (9.0)
\\
4 & 12.9 (29.8) & 15.0 (17.0) & 5.9--7.0 (13.8--16.0) & 7.0--8.0 (8.0--9.0)
\\
6 & 19.0 (44.0) & 23.0 (26.0) & 6.0--7.0 (14.0--16.0) & 7.0--8.0 (8.0--9.0)
\\
8 & 26.1 (60.2) & 32.6 (36.6) & 6.0--7.1 (14.0--16.2) & 7.0--9.8 (8.0--10.8)
\\\hline
\end{tabular}


==> data/iterations-all/data_7.tex <==
\begin{tabular}{C{0.75cm}C{1.50cm}C{1.50cm}C{1.50cm}}
\hline
&\multicolumn{3}{c}{\textbf{non-complex} (Sections~\ref{sec:methods}--\ref{sec:performance})}\\ \hline
&\multicolumn{1}{c}{\textbf{IRK}}&\multicolumn{1}{c}{\textbf{SPIRK}}&\multicolumn{1}{c}{\textbf{batched}} \\ \hline
$Q$& \#G (\#V$^1$) & \#G (\#V$^1$) & \#G (\#V$^Q$) \\ \hline
2 & 6.0 (14.0) & 6.0 (7.0) & 6.0 (7.0)
\\
4 & 7.9 (35.6) & 7.9 (8.9) & 7.9 (8.9)
\\
6 & 9.9 (65.3) & 9.9 (10.9) & 9.9 (10.9)
\\
8 & 11.9 (103.1) & 11.9 (12.9) & 11.7 (12.7)
\\\hline
\end{tabular}

\vspace{0.2cm}

\begin{tabular}{C{0.75cm}C{2.00cm}C{2.0cm}C{2.50cm}C{2.5cm}}
\hline
&\multicolumn{4}{c}{\textbf{complex} (Section~\ref{sec:complex})} \\ \hline
&\multicolumn{1}{c}{\textbf{IRK-PRESB}}&\multicolumn{1}{c}{\textbf{IRK-GMG}}&\multicolumn{1}{c}{\textbf{SPIRK-PRESB}}&\multicolumn{1}{c}{\textbf{SPIRK-GMG}} \\ \hline
$Q$& \#G (\#V$^1$)& \#G (\#V$^2$)& \#G (\#V$^1$)& \#G (\#V$^2$) \\ \hline
2 & 6.0 (14.0) & 7.0 (8.0) & 6.0 (14.0) & 7.0 (8.0)
\\
4 & 12.8 (29.6) & 15.0 (17.0) & 6.0--6.8 (14.0--15.6) & 7.0--8.0 (8.0--9.0)
\\
6 & 19.0 (44.0) & 22.0 (25.0) & 6.0--7.0 (14.0--16.0) & 7.0--8.0 (8.0--9.0)
\\
8 & 25.0 (58.0) & 31.3 (35.3) & 5.0--7.0 (12.0--16.0) & 7.0--9.4 (8.0--10.4)
\\\hline
\end{tabular}


==> data/iterations-all/data_8.tex <==
\begin{tabular}{C{0.75cm}C{1.50cm}C{1.50cm}C{1.50cm}}
\hline
&\multicolumn{3}{c}{\textbf{non-complex} (Sections~\ref{sec:methods}--\ref{sec:performance})}\\ \hline
&\multicolumn{1}{c}{\textbf{IRK}}&\multicolumn{1}{c}{\textbf{SPIRK}}&\multicolumn{1}{c}{\textbf{batched}} \\ \hline
$Q$& \#G (\#V$^1$) & \#G (\#V$^1$) & \#G (\#V$^Q$) \\ \hline
2 & 5.9 (13.8) & 5.9 (6.9) & 5.9 (6.9)
\\
4 & 7.9 (35.6) & 7.9 (8.9) & 7.9 (8.9)
\\
6 & 9.9 (65.3) & 9.9 (10.9) & 9.9 (10.9)
\\
8 & 11.9 (103.1) & 11.9 (12.9) & 11.1 (12.1)
\\\hline
\end{tabular}

\vspace{0.2cm}

\begin{tabular}{C{0.75cm}C{2.00cm}C{2.0cm}C{2.50cm}C{2.5cm}}
\hline
&\multicolumn{4}{c}{\textbf{complex} (Section~\ref{sec:complex})} \\ \hline
&\multicolumn{1}{c}{\textbf{IRK-PRESB}}&\multicolumn{1}{c}{\textbf{IRK-GMG}}&\multicolumn{1}{c}{\textbf{SPIRK-PRESB}}&\multicolumn{1}{c}{\textbf{SPIRK-GMG}} \\ \hline
$Q$& \#G (\#V$^1$)& \#G (\#V$^2$)& \#G (\#V$^1$)& \#G (\#V$^2$) \\ \hline
2 & 6.0 (14.0) & 7.0 (8.0) & 6.0 (14.0) & 7.0 (8.0)
\\
4 & 11.9 (27.8) & 14.0 (16.0) & 5.9--6.0 (13.8--14.0) & 7.0--7.0 (8.0--8.0)
\\
6 & 18.6 (43.1) & 22.0 (25.0) & 6.0--6.6 (14.0--15.1) & 7.0--8.0 (8.0--9.0)
\\
8 & 23.1 (54.2) & 31.3 (35.3) & 5.0--6.1 (12.0--14.2) & 7.0--9.3 (8.0--10.3)
\\\hline
\end{tabular}


==> data/large-scaling/large-scaling-2-1/data_0004_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 7.102333e-03 1.518750e+01 9.000000e+00 1.026423e+05 7.290000e+02 4.000000e+00 2.000000e+00
2 7.369444e-03 7.593750e+00 9.000000e+00 4.946099e+04 7.290000e+02 4.000000e+00 2.000000e+00
4 7.496111e-03 3.796875e+00 9.000000e+00 2.431261e+04 7.290000e+02 4.000000e+00 2.000000e+00
8 7.472556e-03 1.898438e+00 9.000000e+00 1.219462e+04 7.290000e+02 4.000000e+00 2.000000e+00
16 7.520667e-03 9.492188e-01 9.000000e+00 6.058306e+03 7.290000e+02 4.000000e+00 2.000000e+00
32 7.805333e-03 4.746094e-01 9.000000e+00 2.918677e+03 7.290000e+02 4.000000e+00 2.000000e+00
64 7.834222e-03 2.373047e-01 9.000000e+00 1.453957e+03 7.290000e+02 4.000000e+00 2.000000e+00
128 7.732222e-03 1.186523e-01 9.000000e+00 7.365687e+02 7.290000e+02 4.000000e+00 2.000000e+00
256 8.843889e-03 5.932617e-02 9.000000e+00 3.219914e+02 7.290000e+02 4.000000e+00 2.000000e+00
512 1.440444e-02 2.966309e-02 9.000000e+00 9.884644e+01 7.290000e+02 4.000000e+00 2.000000e+00
1024 9.211667e-03 1.483154e-02 9.000000e+00 7.728396e+01 7.290000e+02 4.000000e+00 2.000000e+00
2048 9.776444e-03 7.415771e-03 9.000000e+00 3.640966e+01 7.290000e+02 4.000000e+00 2.000000e+00
3072 8.931778e-03 4.943848e-03 9.000000e+00 2.656858e+01 7.290000e+02 4.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-1/data_0004_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 3.696444e-03 1.518750e+01 9.000000e+00 1.972165e+05 7.290000e+02 4.000000e+00 2.000000e+00
2 4.095778e-03 7.593750e+00 9.000000e+00 8.899409e+04 7.290000e+02 4.000000e+00 2.000000e+00
4 4.400000e-03 3.796875e+00 9.000000e+00 4.142045e+04 7.290000e+02 4.000000e+00 2.000000e+00
8 4.229778e-03 1.898438e+00 9.000000e+00 2.154368e+04 7.290000e+02 4.000000e+00 2.000000e+00
16 4.196667e-03 9.492188e-01 9.000000e+00 1.085683e+04 7.290000e+02 4.000000e+00 2.000000e+00
32 4.351000e-03 4.746094e-01 9.000000e+00 5.235865e+03 7.290000e+02 4.000000e+00 2.000000e+00
64 1.450667e-02 2.373047e-01 9.000000e+00 7.851993e+02 7.290000e+02 4.000000e+00 2.000000e+00
128 1.003300e-02 1.186523e-01 9.000000e+00 5.676580e+02 7.290000e+02 4.000000e+00 2.000000e+00
256 4.926222e-03 5.932617e-02 9.000000e+00 5.780609e+02 7.290000e+02 4.000000e+00 2.000000e+00
512 6.517778e-03 2.966309e-02 9.000000e+00 2.184530e+02 7.290000e+02 4.000000e+00 2.000000e+00
1024 5.989778e-03 1.483154e-02 9.000000e+00 1.188548e+02 7.290000e+02 4.000000e+00 2.000000e+00
2048 6.484444e-03 7.415771e-03 9.000000e+00 5.489399e+01 7.290000e+02 4.000000e+00 2.000000e+00
3072 6.288778e-03 4.943848e-03 9.000000e+00 3.773463e+01 7.290000e+02 4.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-1/data_0005_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 1.163444e-02 1.023542e+02 9.000000e+00 4.222806e+05 4.913000e+03 5.000000e+00 2.000000e+00
2 1.316000e-02 5.117708e+01 9.000000e+00 1.866641e+05 4.913000e+03 5.000000e+00 2.000000e+00
4 1.353333e-02 2.558854e+01 9.000000e+00 9.075739e+04 4.913000e+03 5.000000e+00 2.000000e+00
8 1.395000e-02 1.279427e+01 9.000000e+00 4.402330e+04 4.913000e+03 5.000000e+00 2.000000e+00
16 1.259556e-02 6.397135e+00 9.000000e+00 2.437864e+04 4.913000e+03 5.000000e+00 2.000000e+00
32 1.242111e-02 3.198568e+00 9.000000e+00 1.236051e+04 4.913000e+03 5.000000e+00 2.000000e+00
64 1.494889e-02 1.599284e+00 9.000000e+00 5.135206e+03 4.913000e+03 5.000000e+00 2.000000e+00
128 1.435556e-02 7.996419e-01 9.000000e+00 2.673725e+03 4.913000e+03 5.000000e+00 2.000000e+00
256 1.617111e-02 3.998210e-01 9.000000e+00 1.186771e+03 4.913000e+03 5.000000e+00 2.000000e+00
512 1.915889e-02 1.999105e-01 9.000000e+00 5.008486e+02 4.913000e+03 5.000000e+00 2.000000e+00
1024 1.345000e-02 9.995524e-02 9.000000e+00 3.567176e+02 4.913000e+03 5.000000e+00 2.000000e+00
2048 1.511000e-02 4.997762e-02 9.000000e+00 1.587641e+02 4.913000e+03 5.000000e+00 2.000000e+00
3072 1.397111e-02 3.331841e-02 9.000000e+00 1.144708e+02 4.913000e+03 5.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-1/data_0005_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 6.510111e-03 1.023542e+02 9.000000e+00 7.546722e+05 4.913000e+03 5.000000e+00 2.000000e+00
2 6.687222e-03 5.117708e+01 9.000000e+00 3.673424e+05 4.913000e+03 5.000000e+00 2.000000e+00
4 8.029556e-03 2.558854e+01 9.000000e+00 1.529661e+05 4.913000e+03 5.000000e+00 2.000000e+00
8 7.369778e-03 1.279427e+01 9.000000e+00 8.333019e+04 4.913000e+03 5.000000e+00 2.000000e+00
16 7.877000e-03 6.397135e+00 9.000000e+00 3.898216e+04 4.913000e+03 5.000000e+00 2.000000e+00
32 7.199556e-03 3.198568e+00 9.000000e+00 2.132510e+04 4.913000e+03 5.000000e+00 2.000000e+00
64 1.627222e-02 1.599284e+00 9.000000e+00 4.717587e+03 4.913000e+03 5.000000e+00 2.000000e+00
128 1.236667e-02 7.996419e-01 9.000000e+00 3.103731e+03 4.913000e+03 5.000000e+00 2.000000e+00
256 1.147333e-02 3.998210e-01 9.000000e+00 1.672697e+03 4.913000e+03 5.000000e+00 2.000000e+00
512 1.093289e-02 1.999105e-01 9.000000e+00 8.776915e+02 4.913000e+03 5.000000e+00 2.000000e+00
1024 7.622111e-03 9.995524e-02 9.000000e+00 6.294649e+02 4.913000e+03 5.000000e+00 2.000000e+00
2048 8.351111e-03 4.997762e-02 9.000000e+00 2.872583e+02 4.913000e+03 5.000000e+00 2.000000e+00
3072 8.325778e-03 3.331841e-02 9.000000e+00 1.920882e+02 4.913000e+03 5.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-1/data_0006_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 2.526222e-02 7.486875e+02 9.000000e+00 1.422559e+06 3.593700e+04 6.000000e+00 2.000000e+00
2 2.250000e-02 3.743438e+02 9.000000e+00 7.986000e+05 3.593700e+04 6.000000e+00 2.000000e+00
4 2.229889e-02 1.871719e+02 9.000000e+00 4.029012e+05 3.593700e+04 6.000000e+00 2.000000e+00
8 2.135778e-02 9.358594e+01 9.000000e+00 2.103274e+05 3.593700e+04 6.000000e+00 2.000000e+00
16 1.932889e-02 4.679297e+01 9.000000e+00 1.162024e+05 3.593700e+04 6.000000e+00 2.000000e+00
32 2.005222e-02 2.339648e+01 9.000000e+00 5.600533e+04 3.593700e+04 6.000000e+00 2.000000e+00
64 2.612778e-02 1.169824e+01 9.000000e+00 2.149114e+04 3.593700e+04 6.000000e+00 2.000000e+00
128 2.240222e-02 5.849121e+00 9.000000e+00 1.253259e+04 3.593700e+04 6.000000e+00 2.000000e+00
256 2.894333e-02 2.924561e+00 9.000000e+00 4.850129e+03 3.593700e+04 6.000000e+00 2.000000e+00
512 2.530333e-02 1.462280e+00 9.000000e+00 2.773921e+03 3.593700e+04 6.000000e+00 2.000000e+00
1024 1.807111e-02 7.311401e-01 9.000000e+00 1.942035e+03 3.593700e+04 6.000000e+00 2.000000e+00
2048 2.097778e-02 3.655701e-01 9.000000e+00 8.364739e+02 3.593700e+04 6.000000e+00 2.000000e+00
3072 2.136889e-02 2.437134e-01 9.000000e+00 5.474427e+02 3.593700e+04 6.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-1/data_0006_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 1.859889e-02 7.486875e+02 9.000000e+00 1.932212e+06 3.593700e+04 6.000000e+00 2.000000e+00
2 1.396000e-02 3.743438e+02 9.000000e+00 1.287142e+06 3.593700e+04 6.000000e+00 2.000000e+00
4 1.262111e-02 1.871719e+02 9.000000e+00 7.118430e+05 3.593700e+04 6.000000e+00 2.000000e+00
8 1.134889e-02 9.358594e+01 9.000000e+00 3.958207e+05 3.593700e+04 6.000000e+00 2.000000e+00
16 1.098800e-02 4.679297e+01 9.000000e+00 2.044105e+05 3.593700e+04 6.000000e+00 2.000000e+00
32 1.118222e-02 2.339648e+01 9.000000e+00 1.004301e+05 3.593700e+04 6.000000e+00 2.000000e+00
64 1.476222e-02 1.169824e+01 9.000000e+00 3.803734e+04 3.593700e+04 6.000000e+00 2.000000e+00
128 1.445889e-02 5.849121e+00 9.000000e+00 1.941766e+04 3.593700e+04 6.000000e+00 2.000000e+00
256 1.303000e-02 2.924561e+00 9.000000e+00 1.077352e+04 3.593700e+04 6.000000e+00 2.000000e+00
512 1.155778e-02 1.462280e+00 9.000000e+00 6.072919e+03 3.593700e+04 6.000000e+00 2.000000e+00
1024 1.090989e-02 7.311401e-01 9.000000e+00 3.216781e+03 3.593700e+04 6.000000e+00 2.000000e+00
2048 1.426222e-02 3.655701e-01 9.000000e+00 1.230339e+03 3.593700e+04 6.000000e+00 2.000000e+00
3072 1.404889e-02 2.437134e-01 9.000000e+00 8.326810e+02 3.593700e+04 6.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-1/data_0007_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 1.122222e-01 5.721354e+03 9.000000e+00 2.447153e+06 2.746250e+05 7.000000e+00 2.000000e+00
2 6.689556e-02 2.860677e+03 9.000000e+00 2.052640e+06 2.746250e+05 7.000000e+00 2.000000e+00
4 4.769000e-02 1.430339e+03 9.000000e+00 1.439636e+06 2.746250e+05 7.000000e+00 2.000000e+00
8 3.607111e-02 7.151693e+02 9.000000e+00 9.516792e+05 2.746250e+05 7.000000e+00 2.000000e+00
16 2.950889e-02 3.575846e+02 9.000000e+00 5.816574e+05 2.746250e+05 7.000000e+00 2.000000e+00
32 2.818889e-02 1.787923e+02 9.000000e+00 3.044473e+05 2.746250e+05 7.000000e+00 2.000000e+00
64 4.085556e-02 8.939616e+01 9.000000e+00 1.050289e+05 2.746250e+05 7.000000e+00 2.000000e+00
128 3.798778e-02 4.469808e+01 9.000000e+00 5.647890e+04 2.746250e+05 7.000000e+00 2.000000e+00
256 4.743222e-02 2.234904e+01 9.000000e+00 2.261656e+04 2.746250e+05 7.000000e+00 2.000000e+00
512 3.827444e-02 1.117452e+01 9.000000e+00 1.401397e+04 2.746250e+05 7.000000e+00 2.000000e+00
1024 3.360667e-02 5.587260e+00 9.000000e+00 7.980217e+03 2.746250e+05 7.000000e+00 2.000000e+00
2048 3.470111e-02 2.793630e+00 9.000000e+00 3.864264e+03 2.746250e+05 7.000000e+00 2.000000e+00
3072 2.848889e-02 1.862420e+00 9.000000e+00 3.137931e+03 2.746250e+05 7.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-1/data_0007_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 1.081989e-01 5.721354e+03 9.000000e+00 2.538150e+06 2.746250e+05 7.000000e+00 2.000000e+00
2 5.957000e-02 2.860677e+03 9.000000e+00 2.305061e+06 2.746250e+05 7.000000e+00 2.000000e+00
4 3.714222e-02 1.430339e+03 9.000000e+00 1.848469e+06 2.746250e+05 7.000000e+00 2.000000e+00
8 2.454556e-02 7.151693e+02 9.000000e+00 1.398547e+06 2.746250e+05 7.000000e+00 2.000000e+00
16 1.955778e-02 3.575846e+02 9.000000e+00 8.776080e+05 2.746250e+05 7.000000e+00 2.000000e+00
32 1.707222e-02 1.787923e+02 9.000000e+00 5.026898e+05 2.746250e+05 7.000000e+00 2.000000e+00
64 2.092111e-02 8.939616e+01 9.000000e+00 2.051046e+05 2.746250e+05 7.000000e+00 2.000000e+00
128 2.458667e-02 4.469808e+01 9.000000e+00 8.726306e+04 2.746250e+05 7.000000e+00 2.000000e+00
256 3.352333e-02 2.234904e+01 9.000000e+00 3.200022e+04 2.746250e+05 7.000000e+00 2.000000e+00
512 3.886444e-02 1.117452e+01 9.000000e+00 1.380123e+04 2.746250e+05 7.000000e+00 2.000000e+00
1024 2.666444e-02 5.587260e+00 9.000000e+00 1.005791e+04 2.746250e+05 7.000000e+00 2.000000e+00
2048 2.655778e-02 2.793630e+00 9.000000e+00 5.049151e+03 2.746250e+05 7.000000e+00 2.000000e+00
3072 2.941556e-02 1.862420e+00 9.000000e+00 3.039078e+03 2.746250e+05 7.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-1/data_0008_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 7.299222e-01 4.472269e+04 9.000000e+00 2.940983e+06 2.146689e+06 8.000000e+00 2.000000e+00
2 3.850111e-01 2.236134e+04 9.000000e+00 2.787827e+06 2.146689e+06 8.000000e+00 2.000000e+00
4 2.145556e-01 1.118067e+04 9.000000e+00 2.501321e+06 2.146689e+06 8.000000e+00 2.000000e+00
8 1.417889e-01 5.590336e+03 9.000000e+00 1.892505e+06 2.146689e+06 8.000000e+00 2.000000e+00
16 7.496556e-02 2.795168e+03 9.000000e+00 1.789729e+06 2.146689e+06 8.000000e+00 2.000000e+00
32 5.555444e-02 1.397584e+03 9.000000e+00 1.207537e+06 2.146689e+06 8.000000e+00 2.000000e+00
64 4.686667e-02 6.987920e+02 9.000000e+00 7.156902e+05 2.146689e+06 8.000000e+00 2.000000e+00
128 4.935000e-02 3.493960e+02 9.000000e+00 3.398381e+05 2.146689e+06 8.000000e+00 2.000000e+00
256 5.059222e-02 1.746980e+02 9.000000e+00 1.657469e+05 2.146689e+06 8.000000e+00 2.000000e+00
512 4.656000e-02 8.734900e+01 9.000000e+00 9.005051e+04 2.146689e+06 8.000000e+00 2.000000e+00
1024 6.029778e-02 4.367450e+01 9.000000e+00 3.476705e+04 2.146689e+06 8.000000e+00 2.000000e+00
2048 7.075778e-02 2.183725e+01 9.000000e+00 1.481375e+04 2.146689e+06 8.000000e+00 2.000000e+00
3072 8.533556e-02 1.455817e+01 9.000000e+00 8.188755e+03 2.146689e+06 8.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-1/data_0008_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 7.466667e-01 4.472269e+04 9.000000e+00 2.875030e+06 2.146689e+06 8.000000e+00 2.000000e+00
2 3.831000e-01 2.236134e+04 9.000000e+00 2.801735e+06 2.146689e+06 8.000000e+00 2.000000e+00
4 2.134889e-01 1.118067e+04 9.000000e+00 2.513818e+06 2.146689e+06 8.000000e+00 2.000000e+00
8 1.248778e-01 5.590336e+03 9.000000e+00 2.148790e+06 2.146689e+06 8.000000e+00 2.000000e+00
16 6.658333e-02 2.795168e+03 9.000000e+00 2.015040e+06 2.146689e+06 8.000000e+00 2.000000e+00
32 4.306333e-02 1.397584e+03 9.000000e+00 1.557799e+06 2.146689e+06 8.000000e+00 2.000000e+00
64 4.029444e-02 6.987920e+02 9.000000e+00 8.324228e+05 2.146689e+06 8.000000e+00 2.000000e+00
128 2.926667e-02 3.493960e+02 9.000000e+00 5.730413e+05 2.146689e+06 8.000000e+00 2.000000e+00
256 3.490778e-02 1.746980e+02 9.000000e+00 2.402188e+05 2.146689e+06 8.000000e+00 2.000000e+00
512 2.371889e-01 8.734900e+01 9.000000e+00 1.767685e+04 2.146689e+06 8.000000e+00 2.000000e+00
1024 4.046556e-02 4.367450e+01 9.000000e+00 5.180643e+04 2.146689e+06 8.000000e+00 2.000000e+00
2048 5.457667e-02 2.183725e+01 9.000000e+00 1.920579e+04 2.146689e+06 8.000000e+00 2.000000e+00
3072 7.065333e-02 1.455817e+01 9.000000e+00 9.890432e+03 2.146689e+06 8.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-1/data_0009_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 4.933000e+00 3.536374e+05 9.000000e+00 3.441028e+06 1.697459e+07 9.000000e+00 2.000000e+00
2 2.601667e+00 1.768187e+05 9.000000e+00 3.262254e+06 1.697459e+07 9.000000e+00 2.000000e+00
4 1.317333e+00 8.840934e+04 9.000000e+00 3.221393e+06 1.697459e+07 9.000000e+00 2.000000e+00
8 6.947111e-01 4.420467e+04 9.000000e+00 3.054254e+06 1.697459e+07 9.000000e+00 2.000000e+00
16 3.518222e-01 2.210233e+04 9.000000e+00 3.015478e+06 1.697459e+07 9.000000e+00 2.000000e+00
32 2.114556e-01 1.105117e+04 9.000000e+00 2.508593e+06 1.697459e+07 9.000000e+00 2.000000e+00
64 1.371444e-01 5.525584e+03 9.000000e+00 1.933932e+06 1.697459e+07 9.000000e+00 2.000000e+00
128 9.022444e-02 2.762792e+03 9.000000e+00 1.469823e+06 1.697459e+07 9.000000e+00 2.000000e+00
256 8.083889e-02 1.381396e+03 9.000000e+00 8.202365e+05 1.697459e+07 9.000000e+00 2.000000e+00
512 5.632111e-02 6.906980e+02 9.000000e+00 5.886514e+05 1.697459e+07 9.000000e+00 2.000000e+00
1024 6.239889e-02 3.453490e+02 9.000000e+00 2.656578e+05 1.697459e+07 9.000000e+00 2.000000e+00
2048 6.597778e-02 1.726745e+02 9.000000e+00 1.256237e+05 1.697459e+07 9.000000e+00 2.000000e+00
3072 7.875556e-02 1.151163e+02 9.000000e+00 7.016119e+04 1.697459e+07 9.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-1/data_0009_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 5.139667e+00 3.536374e+05 9.000000e+00 3.302664e+06 1.697459e+07 9.000000e+00 2.000000e+00
2 3.280556e+00 1.768187e+05 9.000000e+00 2.587152e+06 1.697459e+07 9.000000e+00 2.000000e+00
4 1.433444e+00 8.840934e+04 9.000000e+00 2.960455e+06 1.697459e+07 9.000000e+00 2.000000e+00
8 8.291111e-01 4.420467e+04 9.000000e+00 2.559155e+06 1.697459e+07 9.000000e+00 2.000000e+00
16 3.720556e-01 2.210233e+04 9.000000e+00 2.851488e+06 1.697459e+07 9.000000e+00 2.000000e+00
32 2.071111e-01 1.105117e+04 9.000000e+00 2.561215e+06 1.697459e+07 9.000000e+00 2.000000e+00
64 1.175667e-01 5.525584e+03 9.000000e+00 2.255980e+06 1.697459e+07 9.000000e+00 2.000000e+00
128 7.236000e-02 2.762792e+03 9.000000e+00 1.832698e+06 1.697459e+07 9.000000e+00 2.000000e+00
256 6.087000e-02 1.381396e+03 9.000000e+00 1.089322e+06 1.697459e+07 9.000000e+00 2.000000e+00
512 4.632444e-02 6.906980e+02 9.000000e+00 7.156805e+05 1.697459e+07 9.000000e+00 2.000000e+00
1024 1.835000e-01 3.453490e+02 9.000000e+00 9.033652e+04 1.697459e+07 9.000000e+00 2.000000e+00
2048 4.662556e-02 1.726745e+02 9.000000e+00 1.777646e+05 1.697459e+07 9.000000e+00 2.000000e+00
3072 5.739444e-02 1.151163e+02 9.000000e+00 9.627384e+04 1.697459e+07 9.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-1/data_0010_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
4 1.246111e+01 7.031547e+05 9.000000e+00 2.708541e+06 1.350057e+08 1.000000e+01 2.000000e+00
8 6.302556e+00 3.515773e+05 9.000000e+00 2.677598e+06 1.350057e+08 1.000000e+01 2.000000e+00
16 2.699556e+00 1.757887e+05 9.000000e+00 3.125646e+06 1.350057e+08 1.000000e+01 2.000000e+00
32 1.434556e+00 8.789433e+04 9.000000e+00 2.940930e+06 1.350057e+08 1.000000e+01 2.000000e+00
64 7.451444e-01 4.394717e+04 9.000000e+00 2.830946e+06 1.350057e+08 1.000000e+01 2.000000e+00
128 3.931889e-01 2.197358e+04 9.000000e+00 2.682507e+06 1.350057e+08 1.000000e+01 2.000000e+00
256 2.715444e-01 1.098679e+04 9.000000e+00 1.942098e+06 1.350057e+08 1.000000e+01 2.000000e+00
512 1.583444e-01 5.493396e+03 9.000000e+00 1.665249e+06 1.350057e+08 1.000000e+01 2.000000e+00
1024 4.094111e-01 2.746698e+03 9.000000e+00 3.220272e+05 1.350057e+08 1.000000e+01 2.000000e+00
2048 1.147000e-01 1.373349e+03 9.000000e+00 5.747232e+05 1.350057e+08 1.000000e+01 2.000000e+00
3072 1.161444e-01 9.155660e+02 9.000000e+00 3.783837e+05 1.350057e+08 1.000000e+01 2.000000e+00


==> data/large-scaling/large-scaling-2-1/data_0010_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
4 -inf -5.208333e-03 0.000000e+00 0.000000e+00 -1.000000e+00 -1.000000e+00 -1.000000e+00
8 -inf -2.604167e-03 0.000000e+00 0.000000e+00 -1.000000e+00 -1.000000e+00 -1.000000e+00
16 2.916889e+00 1.757887e+05 9.000000e+00 2.892759e+06 1.350057e+08 1.000000e+01 2.000000e+00
32 1.477556e+00 8.789433e+04 9.000000e+00 2.855343e+06 1.350057e+08 1.000000e+01 2.000000e+00
64 9.113000e-01 4.394717e+04 9.000000e+00 2.314785e+06 1.350057e+08 1.000000e+01 2.000000e+00
128 5.633556e-01 2.197358e+04 9.000000e+00 1.872231e+06 1.350057e+08 1.000000e+01 2.000000e+00
256 2.814333e-01 1.098679e+04 9.000000e+00 1.873858e+06 1.350057e+08 1.000000e+01 2.000000e+00
512 2.034556e-01 5.493396e+03 9.000000e+00 1.296023e+06 1.350057e+08 1.000000e+01 2.000000e+00
1024 2.378333e-01 2.746698e+03 9.000000e+00 5.543441e+05 1.350057e+08 1.000000e+01 2.000000e+00
2048 9.371667e-02 1.373349e+03 9.000000e+00 7.034048e+05 1.350057e+08 1.000000e+01 2.000000e+00
3072 8.067778e-02 9.155660e+02 9.000000e+00 5.447246e+05 1.350057e+08 1.000000e+01 2.000000e+00


==> data/large-scaling/large-scaling-2-1/data_0011_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
64 6.948111e+00 3.505503e+05 9.000000e+00 2.421725e+06 1.076891e+09 1.100000e+01 2.000000e+00
128 4.162889e+00 1.752752e+05 9.000000e+00 2.021002e+06 1.076891e+09 1.100000e+01 2.000000e+00
256 2.131222e+00 8.763758e+04 9.000000e+00 1.973799e+06 1.076891e+09 1.100000e+01 2.000000e+00
512 1.188444e+00 4.381879e+04 9.000000e+00 1.769794e+06 1.076891e+09 1.100000e+01 2.000000e+00
1024 1.198444e+00 2.190940e+04 9.000000e+00 8.775134e+05 1.076891e+09 1.100000e+01 2.000000e+00
2048 4.203222e-01 1.095470e+04 9.000000e+00 1.251006e+06 1.076891e+09 1.100000e+01 2.000000e+00
3072 3.151778e-01 7.303132e+03 9.000000e+00 1.112230e+06 1.076891e+09 1.100000e+01 2.000000e+00


==> data/large-scaling/large-scaling-2-1/data_0011_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
64 -inf -3.255208e-04 0.000000e+00 0.000000e+00 -1.000000e+00 -1.000000e+00 -1.000000e+00
128 4.275444e+00 1.752752e+05 9.000000e+00 1.967797e+06 1.076891e+09 1.100000e+01 2.000000e+00
256 2.232889e+00 8.763758e+04 9.000000e+00 1.883929e+06 1.076891e+09 1.100000e+01 2.000000e+00
512 1.151556e+00 4.381879e+04 9.000000e+00 1.826488e+06 1.076891e+09 1.100000e+01 2.000000e+00
1024 1.022233e+00 2.190940e+04 9.000000e+00 1.028778e+06 1.076891e+09 1.100000e+01 2.000000e+00
2048 3.686333e-01 1.095470e+04 9.000000e+00 1.426419e+06 1.076891e+09 1.100000e+01 2.000000e+00
3072 2.702333e-01 7.303132e+03 9.000000e+00 1.297214e+06 1.076891e+09 1.100000e+01 2.000000e+00


==> data/large-scaling/large-scaling-2-1/data_0012_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
512 8.352778e+00 3.500376e+05 9.000000e+00 2.011523e+06 8.602524e+09 1.200000e+01 2.000000e+00
1024 5.333667e+00 1.750188e+05 9.000000e+00 1.575071e+06 8.602524e+09 1.200000e+01 2.000000e+00
2048 2.836222e+00 8.750940e+04 9.000000e+00 1.481002e+06 8.602524e+09 1.200000e+01 2.000000e+00
3072 1.945889e+00 5.833960e+04 9.000000e+00 1.439086e+06 8.602524e+09 1.200000e+01 2.000000e+00


==> data/large-scaling/large-scaling-2-1/data_0012_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
512 -inf -4.069010e-05 0.000000e+00 0.000000e+00 -1.000000e+00 -1.000000e+00 -1.000000e+00
1024 6.196000e+00 1.750188e+05 9.000000e+00 1.355859e+06 8.602524e+09 1.200000e+01 2.000000e+00
2048 2.598778e+00 8.750940e+04 9.000000e+00 1.616318e+06 8.602524e+09 1.200000e+01 2.000000e+00
3072 1.812889e+00 5.833960e+04 9.000000e+00 1.544662e+06 8.602524e+09 1.200000e+01 2.000000e+00


==> data/large-scaling/large-scaling-2-1/data_0013_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
3072 1.443222e+01 4.663752e+05 9.000000e+00 1.551113e+06 6.876982e+10 1.300000e+01 2.000000e+00


==> data/large-scaling/large-scaling-2-1/data_0013_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
3072 -inf -6.781684e-06 0.000000e+00 0.000000e+00 -1.000000e+00 -1.000000e+00 -1.000000e+00


==> data/large-scaling/large-scaling-2-1/speedup_0.tex <==
speedup n_dofs n_dofs_norm ranks
1.921396e+00 7.290000e+02 1.518750e+01 4.800000e+01
1.787135e+00 4.913000e+03 1.023542e+02 4.800000e+01
1.358265e+00 3.593700e+04 7.486875e+02 4.800000e+01
1.799278e+00 7.290000e+02 7.593750e+00 9.600000e+01
1.967932e+00 4.913000e+03 5.117708e+01 9.600000e+01
1.611748e+00 3.593700e+04 3.743438e+02 9.600000e+01
1.703662e+00 7.290000e+02 3.796875e+00 1.920000e+02
1.685440e+00 4.913000e+03 2.558854e+01 1.920000e+02
1.766793e+00 3.593700e+04 1.871719e+02 1.920000e+02
1.766654e+00 7.290000e+02 1.898438e+00 3.840000e+02
1.892866e+00 4.913000e+03 1.279427e+01 3.840000e+02
1.881927e+00 3.593700e+04 9.358594e+01 3.840000e+02
1.469558e+00 2.746250e+05 7.151693e+02 3.840000e+02
1.792057e+00 7.290000e+02 9.492188e-01 7.680000e+02
1.599030e+00 4.913000e+03 6.397135e+00 7.680000e+02
1.759091e+00 3.593700e+04 4.679297e+01 7.680000e+02
1.508806e+00 2.746250e+05 3.575846e+02 7.680000e+02
1.793917e+00 7.290000e+02 4.746094e-01 1.536000e+03
1.725261e+00 4.913000e+03 3.198568e+00 1.536000e+03
1.793223e+00 3.593700e+04 2.339648e+01 1.536000e+03
1.651155e+00 2.746250e+05 1.787923e+02 1.536000e+03
5.400429e-01 7.290000e+02 2.373047e-01 3.072000e+03
9.186753e-01 4.913000e+03 1.599284e+00 3.072000e+03
1.769908e+00 3.593700e+04 1.169824e+01 3.072000e+03
1.952839e+00 2.746250e+05 8.939616e+01 3.072000e+03
1.163105e+00 2.146689e+06 6.987920e+02 3.072000e+03
7.706790e-01 7.290000e+02 1.186523e-01 6.144000e+03
1.160827e+00 4.913000e+03 7.996419e-01 6.144000e+03
1.549374e+00 3.593700e+04 5.849121e+00 6.144000e+03
1.545056e+00 2.746250e+05 4.469808e+01 6.144000e+03
1.686219e+00 2.146689e+06 3.493960e+02 6.144000e+03
1.795268e+00 7.290000e+02 5.932617e-02 1.228800e+04
1.409452e+00 4.913000e+03 3.998210e-01 1.228800e+04
2.221284e+00 3.593700e+04 2.924561e+00 1.228800e+04
1.414902e+00 2.746250e+05 2.234904e+01 1.228800e+04
1.449311e+00 2.146689e+06 1.746980e+02 1.228800e+04
2.210024e+00 7.290000e+02 2.966309e-02 2.457600e+04
1.752409e+00 4.913000e+03 1.999105e-01 2.457600e+04
2.189291e+00 3.593700e+04 1.462280e+00 2.457600e+04
9.848190e-01 2.746250e+05 1.117452e+01 2.457600e+04
1.962992e-01 2.146689e+06 8.734900e+01 2.457600e+04
1.215797e+00 1.697459e+07 6.906980e+02 2.457600e+04
1.537898e+00 7.290000e+02 1.483154e-02 4.915200e+04
1.764603e+00 4.913000e+03 9.995524e-02 4.915200e+04
1.656397e+00 3.593700e+04 7.311401e-01 4.915200e+04
1.260355e+00 2.746250e+05 5.587260e+00 4.915200e+04
1.490101e+00 2.146689e+06 4.367450e+01 4.915200e+04
3.400484e-01 1.697459e+07 3.453490e+02 4.915200e+04
1.507676e+00 7.290000e+02 7.415771e-03 9.830400e+04
1.809340e+00 4.913000e+03 4.997762e-02 9.830400e+04
1.470863e+00 3.593700e+04 3.655701e-01 9.830400e+04
1.306627e+00 2.746250e+05 2.793630e+00 9.830400e+04
1.296484e+00 2.146689e+06 2.183725e+01 9.830400e+04
1.415056e+00 1.697459e+07 1.726745e+02 9.830400e+04
1.420272e+00 7.290000e+02 4.943848e-03 1.474560e+05
1.678055e+00 4.913000e+03 3.331841e-02 1.474560e+05
1.521038e+00 3.593700e+04 2.437134e-01 1.474560e+05
9.684974e-01 2.746250e+05 1.862420e+00 1.474560e+05
1.207807e+00 2.146689e+06 1.455817e+01 1.474560e+05
1.372181e+00 1.697459e+07 1.151163e+02 1.474560e+05
1.439609e+00 1.350057e+08 9.155660e+02 1.474560e+05


==> data/large-scaling/large-scaling-2-1/speedup_1.tex <==
speedup n_dofs n_dofs_norm ranks
1.037185e+00 2.746250e+05 5.721354e+03 4.800000e+01
1.122974e+00 2.746250e+05 2.860677e+03 9.600000e+01
1.283983e+00 2.746250e+05 1.430339e+03 1.920000e+02
1.135421e+00 2.146689e+06 5.590336e+03 3.840000e+02
1.125891e+00 2.146689e+06 2.795168e+03 7.680000e+02
1.290064e+00 2.146689e+06 1.397584e+03 1.536000e+03
1.166525e+00 1.697459e+07 5.525584e+03 3.072000e+03
1.246883e+00 1.697459e+07 2.762792e+03 6.144000e+03
1.328058e+00 1.697459e+07 1.381396e+03 1.228800e+04
7.782754e-01 1.350057e+08 5.493396e+03 2.457600e+04
1.721420e+00 1.350057e+08 2.746698e+03 4.915200e+04
1.223902e+00 1.350057e+08 1.373349e+03 9.830400e+04
1.166317e+00 1.076891e+09 7.303132e+03 1.474560e+05


==> data/large-scaling/large-scaling-2-1/speedup_2.tex <==
speedup n_dofs n_dofs_norm ranks
9.775744e-01 2.146689e+06 4.472269e+04 4.800000e+01
1.004989e+00 2.146689e+06 2.236134e+04 9.600000e+01
1.004996e+00 2.146689e+06 1.118067e+04 1.920000e+02
9.189985e-01 1.697459e+07 8.840934e+04 1.920000e+02
8.378987e-01 1.697459e+07 4.420467e+04 3.840000e+02
9.456174e-01 1.697459e+07 2.210233e+04 7.680000e+02
1.020976e+00 1.697459e+07 1.105117e+04 1.536000e+03
9.708979e-01 1.350057e+08 8.789433e+04 1.536000e+03
8.176719e-01 1.350057e+08 4.394717e+04 3.072000e+03
6.979409e-01 1.350057e+08 2.197358e+04 6.144000e+03
9.648624e-01 1.350057e+08 1.098679e+04 1.228800e+04
9.544686e-01 1.076891e+09 8.763758e+04 1.228800e+04
1.032034e+00 1.076891e+09 4.381879e+04 2.457600e+04
1.172379e+00 1.076891e+09 2.190940e+04 4.915200e+04
1.140218e+00 1.076891e+09 1.095470e+04 9.830400e+04
1.091368e+00 8.602524e+09 8.750940e+04 9.830400e+04
1.073364e+00 8.602524e+09 5.833960e+04 1.474560e+05


==> data/large-scaling/large-scaling-2-1/speedup_3.tex <==
speedup n_dofs n_dofs_norm ranks
9.597899e-01 1.697459e+07 3.536374e+05 4.800000e+01
7.930567e-01 1.697459e+07 1.768187e+05 9.600000e+01
9.254914e-01 1.350057e+08 1.757887e+05 7.680000e+02
9.736740e-01 1.076891e+09 1.752752e+05 6.144000e+03
8.608242e-01 8.602524e+09 1.750188e+05 4.915200e+04


==> data/large-scaling/large-scaling-2-4/data_0004_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 1.690800e-02 7.486875e+02 1.000000e+01 2.125444e+06 3.593700e+04 4.000000e+00 2.000000e+00
2 1.528500e-02 3.743438e+02 1.000000e+01 1.175564e+06 3.593700e+04 4.000000e+00 2.000000e+00
4 1.495100e-02 1.871719e+02 1.000000e+01 6.009130e+05 3.593700e+04 4.000000e+00 2.000000e+00
8 1.489000e-02 9.358594e+01 1.000000e+01 3.016874e+05 3.593700e+04 4.000000e+00 2.000000e+00
16 1.531100e-02 4.679297e+01 1.000000e+01 1.466960e+05 3.593700e+04 4.000000e+00 2.000000e+00
32 2.215200e-02 2.339648e+01 1.000000e+01 5.069661e+04 3.593700e+04 4.000000e+00 2.000000e+00
64 2.225900e-02 1.169824e+01 1.000000e+01 2.522645e+04 3.593700e+04 4.000000e+00 2.000000e+00
128 1.563600e-02 5.849121e+00 1.000000e+01 1.795586e+04 3.593700e+04 4.000000e+00 2.000000e+00
256 1.917800e-02 2.924561e+00 1.000000e+01 7.319789e+03 3.593700e+04 4.000000e+00 2.000000e+00
512 1.585400e-02 1.462280e+00 1.000000e+01 4.427239e+03 3.593700e+04 4.000000e+00 2.000000e+00
1024 1.624500e-02 7.311401e-01 1.000000e+01 2.160340e+03 3.593700e+04 4.000000e+00 2.000000e+00
2048 1.802000e-02 3.655701e-01 1.000000e+01 9.737715e+02 3.593700e+04 4.000000e+00 2.000000e+00
3072 1.870900e-02 2.437134e-01 1.000000e+01 6.252735e+02 3.593700e+04 4.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-4/data_0004_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 9.657900e-03 7.486875e+02 1.000000e+01 3.720995e+06 3.593700e+04 4.000000e+00 2.000000e+00
2 9.160000e-03 3.743438e+02 1.000000e+01 1.961627e+06 3.593700e+04 4.000000e+00 2.000000e+00
4 8.367300e-03 1.871719e+02 1.000000e+01 1.073733e+06 3.593700e+04 4.000000e+00 2.000000e+00
8 9.380600e-03 9.358594e+01 1.000000e+01 4.788740e+05 3.593700e+04 4.000000e+00 2.000000e+00
16 8.420100e-03 4.679297e+01 1.000000e+01 2.667501e+05 3.593700e+04 4.000000e+00 2.000000e+00
32 9.587300e-03 2.339648e+01 1.000000e+01 1.171374e+05 3.593700e+04 4.000000e+00 2.000000e+00
64 8.704700e-03 1.169824e+01 1.000000e+01 6.450718e+04 3.593700e+04 4.000000e+00 2.000000e+00
128 1.007900e-02 5.849121e+00 1.000000e+01 2.785572e+04 3.593700e+04 4.000000e+00 2.000000e+00
256 1.014600e-02 2.924561e+00 1.000000e+01 1.383589e+04 3.593700e+04 4.000000e+00 2.000000e+00
512 9.787800e-03 1.462280e+00 1.000000e+01 7.171116e+03 3.593700e+04 4.000000e+00 2.000000e+00
1024 9.744000e-03 7.311401e-01 1.000000e+01 3.601676e+03 3.593700e+04 4.000000e+00 2.000000e+00
2048 9.466800e-03 3.655701e-01 1.000000e+01 1.853569e+03 3.593700e+04 4.000000e+00 2.000000e+00
3072 1.091500e-02 2.437134e-01 1.000000e+01 1.071758e+03 3.593700e+04 4.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-4/data_0005_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 4.297600e-02 5.721354e+03 1.000000e+01 6.390195e+06 2.746250e+05 5.000000e+00 2.000000e+00
2 3.527600e-02 2.860677e+03 1.000000e+01 3.892519e+06 2.746250e+05 5.000000e+00 2.000000e+00
4 3.137100e-02 1.430339e+03 1.000000e+01 2.188526e+06 2.746250e+05 5.000000e+00 2.000000e+00
8 3.018900e-02 7.151693e+02 1.000000e+01 1.137107e+06 2.746250e+05 5.000000e+00 2.000000e+00
16 2.729300e-02 3.575846e+02 1.000000e+01 6.288815e+05 2.746250e+05 5.000000e+00 2.000000e+00
32 2.813300e-02 1.787923e+02 1.000000e+01 3.050521e+05 2.746250e+05 5.000000e+00 2.000000e+00
64 3.493800e-02 8.939616e+01 1.000000e+01 1.228180e+05 2.746250e+05 5.000000e+00 2.000000e+00
128 2.982400e-02 4.469808e+01 1.000000e+01 7.193897e+04 2.746250e+05 5.000000e+00 2.000000e+00
256 3.159100e-02 2.234904e+01 1.000000e+01 3.395758e+04 2.746250e+05 5.000000e+00 2.000000e+00
512 2.928500e-02 1.117452e+01 1.000000e+01 1.831576e+04 2.746250e+05 5.000000e+00 2.000000e+00
1024 3.056900e-02 5.587260e+00 1.000000e+01 8.773217e+03 2.746250e+05 5.000000e+00 2.000000e+00
2048 3.073100e-02 2.793630e+00 1.000000e+01 4.363484e+03 2.746250e+05 5.000000e+00 2.000000e+00
3072 2.986000e-02 1.862420e+00 1.000000e+01 2.993843e+03 2.746250e+05 5.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-4/data_0005_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 3.252800e-02 5.721354e+03 1.000000e+01 8.442726e+06 2.746250e+05 5.000000e+00 2.000000e+00
2 2.175000e-02 2.860677e+03 1.000000e+01 6.313218e+06 2.746250e+05 5.000000e+00 2.000000e+00
4 1.901600e-02 1.430339e+03 1.000000e+01 3.610446e+06 2.746250e+05 5.000000e+00 2.000000e+00
8 1.820000e-02 7.151693e+02 1.000000e+01 1.886161e+06 2.746250e+05 5.000000e+00 2.000000e+00
16 1.579800e-02 3.575846e+02 1.000000e+01 1.086471e+06 2.746250e+05 5.000000e+00 2.000000e+00
32 1.809000e-02 1.787923e+02 1.000000e+01 4.744075e+05 2.746250e+05 5.000000e+00 2.000000e+00
64 1.768300e-02 8.939616e+01 1.000000e+01 2.426633e+05 2.746250e+05 5.000000e+00 2.000000e+00
128 1.513200e-02 4.469808e+01 1.000000e+01 1.417861e+05 2.746250e+05 5.000000e+00 2.000000e+00
256 1.726500e-02 2.234904e+01 1.000000e+01 6.213460e+04 2.746250e+05 5.000000e+00 2.000000e+00
512 1.506700e-02 1.117452e+01 1.000000e+01 3.559945e+04 2.746250e+05 5.000000e+00 2.000000e+00
1024 1.513200e-02 5.587260e+00 1.000000e+01 1.772327e+04 2.746250e+05 5.000000e+00 2.000000e+00
2048 1.609500e-02 2.793630e+00 1.000000e+01 8.331422e+03 2.746250e+05 5.000000e+00 2.000000e+00
3072 1.591600e-02 1.862420e+00 1.000000e+01 5.616748e+03 2.746250e+05 5.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-4/data_0006_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 2.151400e-01 4.472269e+04 1.000000e+01 9.978103e+06 2.146689e+06 6.000000e+00 2.000000e+00
2 1.147500e-01 2.236134e+04 1.000000e+01 9.353765e+06 2.146689e+06 6.000000e+00 2.000000e+00
4 7.077200e-02 1.118067e+04 1.000000e+01 7.583115e+06 2.146689e+06 6.000000e+00 2.000000e+00
8 5.094200e-02 5.590336e+03 1.000000e+01 5.267483e+06 2.146689e+06 6.000000e+00 2.000000e+00
16 4.545900e-02 2.795168e+03 1.000000e+01 2.951408e+06 2.146689e+06 6.000000e+00 2.000000e+00
32 4.338200e-02 1.397584e+03 1.000000e+01 1.546356e+06 2.146689e+06 6.000000e+00 2.000000e+00
64 4.784800e-02 6.987920e+02 1.000000e+01 7.010119e+05 2.146689e+06 6.000000e+00 2.000000e+00
128 3.757800e-02 3.493960e+02 1.000000e+01 4.462986e+05 2.146689e+06 6.000000e+00 2.000000e+00
256 3.879700e-02 1.746980e+02 1.000000e+01 2.161379e+05 2.146689e+06 6.000000e+00 2.000000e+00
512 3.557500e-02 8.734900e+01 1.000000e+01 1.178567e+05 2.146689e+06 6.000000e+00 2.000000e+00
1024 3.725000e-02 4.367450e+01 1.000000e+01 5.627855e+04 2.146689e+06 6.000000e+00 2.000000e+00
2048 3.743000e-02 2.183725e+01 1.000000e+01 2.800395e+04 2.146689e+06 6.000000e+00 2.000000e+00
3072 3.658900e-02 1.455817e+01 1.000000e+01 1.909842e+04 2.146689e+06 6.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-4/data_0006_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 2.732000e-01 4.472269e+04 1.000000e+01 7.857573e+06 2.146689e+06 6.000000e+00 2.000000e+00
2 1.280200e-01 2.236134e+04 1.000000e+01 8.384194e+06 2.146689e+06 6.000000e+00 2.000000e+00
4 6.686300e-02 1.118067e+04 1.000000e+01 8.026446e+06 2.146689e+06 6.000000e+00 2.000000e+00
8 4.172800e-02 5.590336e+03 1.000000e+01 6.430601e+06 2.146689e+06 6.000000e+00 2.000000e+00
16 2.967800e-02 2.795168e+03 1.000000e+01 4.520792e+06 2.146689e+06 6.000000e+00 2.000000e+00
32 3.468500e-02 1.397584e+03 1.000000e+01 1.934093e+06 2.146689e+06 6.000000e+00 2.000000e+00
64 2.491400e-02 6.987920e+02 1.000000e+01 1.346312e+06 2.146689e+06 6.000000e+00 2.000000e+00
128 2.364500e-02 3.493960e+02 1.000000e+01 7.092835e+05 2.146689e+06 6.000000e+00 2.000000e+00
256 2.321000e-02 1.746980e+02 1.000000e+01 3.612884e+05 2.146689e+06 6.000000e+00 2.000000e+00
512 2.289600e-02 8.734900e+01 1.000000e+01 1.831216e+05 2.146689e+06 6.000000e+00 2.000000e+00
1024 2.056900e-02 4.367450e+01 1.000000e+01 1.019192e+05 2.146689e+06 6.000000e+00 2.000000e+00
2048 2.188900e-02 2.183725e+01 1.000000e+01 4.788652e+04 2.146689e+06 6.000000e+00 2.000000e+00
3072 2.183700e-02 1.455817e+01 1.000000e+01 3.200037e+04 2.146689e+06 6.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-4/data_0007_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 2.094700e+00 3.536374e+05 1.000000e+01 8.103591e+06 1.697459e+07 7.000000e+00 2.000000e+00
2 1.030800e+00 1.768187e+05 1.000000e+01 8.233699e+06 1.697459e+07 7.000000e+00 2.000000e+00
4 4.831700e-01 8.840934e+04 1.000000e+01 8.782930e+06 1.697459e+07 7.000000e+00 2.000000e+00
8 2.306500e-01 4.420467e+04 1.000000e+01 9.199324e+06 1.697459e+07 7.000000e+00 2.000000e+00
16 1.273900e-01 2.210233e+04 1.000000e+01 8.328064e+06 1.697459e+07 7.000000e+00 2.000000e+00
32 9.388700e-02 1.105117e+04 1.000000e+01 5.649941e+06 1.697459e+07 7.000000e+00 2.000000e+00
64 6.664000e-02 5.525584e+03 1.000000e+01 3.980012e+06 1.697459e+07 7.000000e+00 2.000000e+00
128 6.175700e-02 2.762792e+03 1.000000e+01 2.147352e+06 1.697459e+07 7.000000e+00 2.000000e+00
256 5.885400e-02 1.381396e+03 1.000000e+01 1.126635e+06 1.697459e+07 7.000000e+00 2.000000e+00
512 5.257800e-02 6.906980e+02 1.000000e+01 6.305584e+05 1.697459e+07 7.000000e+00 2.000000e+00
1024 5.049100e-02 3.453490e+02 1.000000e+01 3.283110e+05 1.697459e+07 7.000000e+00 2.000000e+00
2048 4.851100e-02 1.726745e+02 1.000000e+01 1.708556e+05 1.697459e+07 7.000000e+00 2.000000e+00
3072 4.872100e-02 1.151163e+02 1.000000e+01 1.134128e+05 1.697459e+07 7.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-4/data_0007_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 2.581700e+00 3.536374e+05 1.000000e+01 6.574967e+06 1.697459e+07 7.000000e+00 2.000000e+00
2 1.281300e+00 1.768187e+05 1.000000e+01 6.623973e+06 1.697459e+07 7.000000e+00 2.000000e+00
4 6.231100e-01 8.840934e+04 1.000000e+01 6.810432e+06 1.697459e+07 7.000000e+00 2.000000e+00
8 2.966000e-01 4.420467e+04 1.000000e+01 7.153824e+06 1.697459e+07 7.000000e+00 2.000000e+00
16 1.411000e-01 2.210233e+04 1.000000e+01 7.518866e+06 1.697459e+07 7.000000e+00 2.000000e+00
32 7.888400e-02 1.105117e+04 1.000000e+01 6.724507e+06 1.697459e+07 7.000000e+00 2.000000e+00
64 5.853500e-02 5.525584e+03 1.000000e+01 4.531101e+06 1.697459e+07 7.000000e+00 2.000000e+00
128 3.948100e-02 2.762792e+03 1.000000e+01 3.358932e+06 1.697459e+07 7.000000e+00 2.000000e+00
256 4.249000e-02 1.381396e+03 1.000000e+01 1.560532e+06 1.697459e+07 7.000000e+00 2.000000e+00
512 3.320600e-02 6.906980e+02 1.000000e+01 9.984190e+05 1.697459e+07 7.000000e+00 2.000000e+00
1024 1.661700e-01 3.453490e+02 1.000000e+01 9.975778e+04 1.697459e+07 7.000000e+00 2.000000e+00
2048 2.919100e-02 1.726745e+02 1.000000e+01 2.839360e+05 1.697459e+07 7.000000e+00 2.000000e+00
3072 3.136100e-02 1.151163e+02 1.000000e+01 1.761928e+05 1.697459e+07 7.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-4/data_0008_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
2 9.048800e+00 1.406309e+06 1.000000e+01 7.459867e+06 1.350057e+08 8.000000e+00 2.000000e+00
4 4.418500e+00 7.031547e+05 1.000000e+01 7.638661e+06 1.350057e+08 8.000000e+00 2.000000e+00
8 2.126000e+00 3.515773e+05 1.000000e+01 7.937776e+06 1.350057e+08 8.000000e+00 2.000000e+00
16 1.070300e+00 1.757887e+05 1.000000e+01 7.883636e+06 1.350057e+08 8.000000e+00 2.000000e+00
32 5.219500e-01 8.789433e+04 1.000000e+01 8.083012e+06 1.350057e+08 8.000000e+00 2.000000e+00
64 2.640900e-01 4.394717e+04 1.000000e+01 7.987671e+06 1.350057e+08 8.000000e+00 2.000000e+00
128 1.539100e-01 2.197358e+04 1.000000e+01 6.852914e+06 1.350057e+08 8.000000e+00 2.000000e+00
256 1.118200e-01 1.098679e+04 1.000000e+01 4.716205e+06 1.350057e+08 8.000000e+00 2.000000e+00
512 7.711500e-02 5.493396e+03 1.000000e+01 3.419348e+06 1.350057e+08 8.000000e+00 2.000000e+00
1024 8.878300e-02 2.746698e+03 1.000000e+01 1.484986e+06 1.350057e+08 8.000000e+00 2.000000e+00
2048 7.960400e-02 1.373349e+03 1.000000e+01 8.281085e+05 1.350057e+08 8.000000e+00 2.000000e+00
3072 8.238300e-02 9.155660e+02 1.000000e+01 5.334495e+05 1.350057e+08 8.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-4/data_0008_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
4 5.574000e+00 7.031547e+05 1.000000e+01 6.055153e+06 1.350057e+08 8.000000e+00 2.000000e+00
8 2.690600e+00 3.515773e+05 1.000000e+01 6.272100e+06 1.350057e+08 8.000000e+00 2.000000e+00
16 1.327100e+00 1.757887e+05 1.000000e+01 6.358116e+06 1.350057e+08 8.000000e+00 2.000000e+00
32 6.499800e-01 8.789433e+04 1.000000e+01 6.490858e+06 1.350057e+08 8.000000e+00 2.000000e+00
64 3.136100e-01 4.394717e+04 1.000000e+01 6.726393e+06 1.350057e+08 8.000000e+00 2.000000e+00
128 1.580300e-01 2.197358e+04 1.000000e+01 6.674252e+06 1.350057e+08 8.000000e+00 2.000000e+00
256 9.418000e-02 1.098679e+04 1.000000e+01 5.599554e+06 1.350057e+08 8.000000e+00 2.000000e+00
512 6.557200e-02 5.493396e+03 1.000000e+01 4.021274e+06 1.350057e+08 8.000000e+00 2.000000e+00
1024 1.048200e-01 2.746698e+03 1.000000e+01 1.257790e+06 1.350057e+08 8.000000e+00 2.000000e+00
2048 5.751400e-02 1.373349e+03 1.000000e+01 1.146169e+06 1.350057e+08 8.000000e+00 2.000000e+00
3072 6.286200e-02 9.155660e+02 1.000000e+01 6.991055e+05 1.350057e+08 8.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-4/data_0009_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
16 8.798900e+00 1.402201e+06 1.000000e+01 7.649327e+06 1.076891e+09 9.000000e+00 2.000000e+00
32 4.688000e+00 7.011007e+05 1.000000e+01 7.178505e+06 1.076891e+09 9.000000e+00 2.000000e+00
64 2.206900e+00 3.505503e+05 1.000000e+01 7.624458e+06 1.076891e+09 9.000000e+00 2.000000e+00
128 1.119100e+00 1.752752e+05 1.000000e+01 7.517834e+06 1.076891e+09 9.000000e+00 2.000000e+00
256 5.487000e-01 8.763758e+04 1.000000e+01 7.666492e+06 1.076891e+09 9.000000e+00 2.000000e+00
512 2.796300e-01 4.381879e+04 1.000000e+01 7.521732e+06 1.076891e+09 9.000000e+00 2.000000e+00
1024 4.694400e-01 2.190940e+04 1.000000e+01 2.240225e+06 1.076891e+09 9.000000e+00 2.000000e+00
2048 1.590800e-01 1.095470e+04 1.000000e+01 3.305416e+06 1.076891e+09 9.000000e+00 2.000000e+00
3072 1.417600e-01 7.303132e+03 1.000000e+01 2.472844e+06 1.076891e+09 9.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-4/data_0009_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
32 5.661900e+00 7.011007e+05 1.000000e+01 5.943735e+06 1.076891e+09 9.000000e+00 2.000000e+00
64 2.853700e+00 3.505503e+05 1.000000e+01 5.896351e+06 1.076891e+09 9.000000e+00 2.000000e+00
128 1.523600e+00 1.752752e+05 1.000000e+01 5.521927e+06 1.076891e+09 9.000000e+00 2.000000e+00
256 7.856500e-01 8.763758e+04 1.000000e+01 5.354298e+06 1.076891e+09 9.000000e+00 2.000000e+00
512 3.163900e-01 4.381879e+04 1.000000e+01 6.647814e+06 1.076891e+09 9.000000e+00 2.000000e+00
1024 2.699400e-01 2.190940e+04 1.000000e+01 3.895869e+06 1.076891e+09 9.000000e+00 2.000000e+00
2048 1.395900e-01 1.095470e+04 1.000000e+01 3.766928e+06 1.076891e+09 9.000000e+00 2.000000e+00
3072 1.107600e-01 7.303132e+03 1.000000e+01 3.164954e+06 1.076891e+09 9.000000e+00 2.000000e+00


==> data/large-scaling/large-scaling-2-4/data_0010_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
128 1.039500e+01 1.400150e+06 1.000000e+01 6.465341e+06 8.602524e+09 1.000000e+01 2.000000e+00
256 5.339200e+00 7.000752e+05 1.000000e+01 6.293753e+06 8.602524e+09 1.000000e+01 2.000000e+00
512 3.013200e+00 3.500376e+05 1.000000e+01 5.576067e+06 8.602524e+09 1.000000e+01 2.000000e+00
1024 1.767300e+00 1.750188e+05 1.000000e+01 4.753523e+06 8.602524e+09 1.000000e+01 2.000000e+00
2048 7.495000e-01 8.750940e+04 1.000000e+01 5.604338e+06 8.602524e+09 1.000000e+01 2.000000e+00
3072 5.358100e-01 5.833960e+04 1.000000e+01 5.226294e+06 8.602524e+09 1.000000e+01 2.000000e+00


==> data/large-scaling/large-scaling-2-4/data_0010_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
256 6.320900e+00 7.000752e+05 1.000000e+01 5.316270e+06 8.602524e+09 1.000000e+01 2.000000e+00
512 3.566900e+00 3.500376e+05 1.000000e+01 4.710478e+06 8.602524e+09 1.000000e+01 2.000000e+00
1024 1.955100e+00 1.750188e+05 1.000000e+01 4.296917e+06 8.602524e+09 1.000000e+01 2.000000e+00
2048 9.010800e-01 8.750940e+04 1.000000e+01 4.661574e+06 8.602524e+09 1.000000e+01 2.000000e+00
3072 6.425900e-01 5.833960e+04 1.000000e+01 4.357834e+06 8.602524e+09 1.000000e+01 2.000000e+00


==> data/large-scaling/large-scaling-2-4/data_0011_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1024 1.144500e+01 1.399126e+06 1.000000e+01 5.867892e+06 6.876982e+10 1.100000e+01 2.000000e+00
2048 5.941700e+00 6.995628e+05 1.000000e+01 5.651415e+06 6.876982e+10 1.100000e+01 2.000000e+00
3072 4.370900e+00 4.663752e+05 1.000000e+01 5.121602e+06 6.876982e+10 1.100000e+01 2.000000e+00


==> data/large-scaling/large-scaling-2-4/data_0011_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
2048 7.033100e+00 6.995628e+05 1.000000e+01 4.774426e+06 6.876982e+10 1.100000e+01 2.000000e+00
3072 4.672100e+00 4.663752e+05 1.000000e+01 4.791423e+06 6.876982e+10 1.100000e+01 2.000000e+00


==> data/large-scaling/large-scaling-2-4/speedup_0.tex <==
speedup n_dofs n_dofs_norm ranks
1.750691e+00 3.593700e+04 7.486875e+02 4.800000e+01
1.668668e+00 3.593700e+04 3.743438e+02 9.600000e+01
1.786837e+00 3.593700e+04 1.871719e+02 1.920000e+02
1.587319e+00 3.593700e+04 9.358594e+01 3.840000e+02
1.658736e+00 2.746250e+05 7.151693e+02 3.840000e+02
1.818387e+00 3.593700e+04 4.679297e+01 7.680000e+02
1.727624e+00 2.746250e+05 3.575846e+02 7.680000e+02
2.310557e+00 3.593700e+04 2.339648e+01 1.536000e+03
1.555169e+00 2.746250e+05 1.787923e+02 1.536000e+03
2.557124e+00 3.593700e+04 1.169824e+01 3.072000e+03
1.975796e+00 2.746250e+05 8.939616e+01 3.072000e+03
1.920527e+00 2.146689e+06 6.987920e+02 3.072000e+03
1.551344e+00 3.593700e+04 5.849121e+00 6.144000e+03
1.970923e+00 2.746250e+05 4.469808e+01 6.144000e+03
1.589258e+00 2.146689e+06 3.493960e+02 6.144000e+03
1.890203e+00 3.593700e+04 2.924561e+00 1.228800e+04
1.829771e+00 2.746250e+05 2.234904e+01 1.228800e+04
1.671564e+00 2.146689e+06 1.746980e+02 1.228800e+04
1.619772e+00 3.593700e+04 1.462280e+00 2.457600e+04
1.943652e+00 2.746250e+05 1.117452e+01 2.457600e+04
1.553765e+00 2.146689e+06 8.734900e+01 2.457600e+04
1.583389e+00 1.697459e+07 6.906980e+02 2.457600e+04
1.667180e+00 3.593700e+04 7.311401e-01 4.915200e+04
2.020156e+00 2.746250e+05 5.587260e+00 4.915200e+04
1.810978e+00 2.146689e+06 4.367450e+01 4.915200e+04
3.038515e-01 1.697459e+07 3.453490e+02 4.915200e+04
1.903494e+00 3.593700e+04 3.655701e-01 9.830400e+04
1.909351e+00 2.746250e+05 2.793630e+00 9.830400e+04
1.709991e+00 2.146689e+06 2.183725e+01 9.830400e+04
1.661848e+00 1.697459e+07 1.726745e+02 9.830400e+04
1.714063e+00 3.593700e+04 2.437134e-01 1.474560e+05
1.876100e+00 2.746250e+05 1.862420e+00 1.474560e+05
1.675551e+00 2.146689e+06 1.455817e+01 1.474560e+05
1.553554e+00 1.697459e+07 1.151163e+02 1.474560e+05
1.310537e+00 1.350057e+08 9.155660e+02 1.474560e+05


==> data/large-scaling/large-scaling-2-4/speedup_1.tex <==
speedup n_dofs n_dofs_norm ranks
1.321200e+00 2.746250e+05 5.721354e+03 4.800000e+01
1.621885e+00 2.746250e+05 2.860677e+03 9.600000e+01
1.649716e+00 2.746250e+05 1.430339e+03 1.920000e+02
1.220811e+00 2.146689e+06 5.590336e+03 3.840000e+02
1.531741e+00 2.146689e+06 2.795168e+03 7.680000e+02
1.250742e+00 2.146689e+06 1.397584e+03 1.536000e+03
1.138464e+00 1.697459e+07 5.525584e+03 3.072000e+03
1.564221e+00 1.697459e+07 2.762792e+03 6.144000e+03
1.385126e+00 1.697459e+07 1.381396e+03 1.228800e+04
1.176036e+00 1.350057e+08 5.493396e+03 2.457600e+04
8.470044e-01 1.350057e+08 2.746698e+03 4.915200e+04
1.384080e+00 1.350057e+08 1.373349e+03 9.830400e+04
1.279884e+00 1.076891e+09 7.303132e+03 1.474560e+05


==> data/large-scaling/large-scaling-2-4/speedup_2.tex <==
speedup n_dofs n_dofs_norm ranks
7.874817e-01 2.146689e+06 4.472269e+04 4.800000e+01
8.963443e-01 2.146689e+06 2.236134e+04 9.600000e+01
1.058463e+00 2.146689e+06 1.118067e+04 1.920000e+02
7.754169e-01 1.697459e+07 8.840934e+04 1.920000e+02
7.776467e-01 1.697459e+07 4.420467e+04 3.840000e+02
9.028349e-01 1.697459e+07 2.210233e+04 7.680000e+02
1.190191e+00 1.697459e+07 1.105117e+04 1.536000e+03
8.030247e-01 1.350057e+08 8.789433e+04 1.536000e+03
8.420969e-01 1.350057e+08 4.394717e+04 3.072000e+03
9.739290e-01 1.350057e+08 2.197358e+04 6.144000e+03
1.187301e+00 1.350057e+08 1.098679e+04 1.228800e+04
6.984026e-01 1.076891e+09 8.763758e+04 1.228800e+04
8.838143e-01 1.076891e+09 4.381879e+04 2.457600e+04
1.739053e+00 1.076891e+09 2.190940e+04 4.915200e+04
1.139623e+00 1.076891e+09 1.095470e+04 9.830400e+04
8.317796e-01 8.602524e+09 8.750940e+04 9.830400e+04
8.338287e-01 8.602524e+09 5.833960e+04 1.474560e+05


==> data/large-scaling/large-scaling-2-4/speedup_3.tex <==
speedup n_dofs n_dofs_norm ranks
8.113646e-01 1.697459e+07 3.536374e+05 4.800000e+01
8.044954e-01 1.697459e+07 1.768187e+05 9.600000e+01
7.926982e-01 1.350057e+08 7.031547e+05 1.920000e+02
7.901583e-01 1.350057e+08 3.515773e+05 3.840000e+02
8.064954e-01 1.350057e+08 1.757887e+05 7.680000e+02
8.279906e-01 1.076891e+09 7.011007e+05 1.536000e+03
7.733469e-01 1.076891e+09 3.505503e+05 3.072000e+03
7.345104e-01 1.076891e+09 1.752752e+05 6.144000e+03
8.446898e-01 8.602524e+09 7.000752e+05 1.228800e+04
8.447672e-01 8.602524e+09 3.500376e+05 2.457600e+04
9.039435e-01 8.602524e+09 1.750188e+05 4.915200e+04
8.448195e-01 6.876982e+10 6.995628e+05 9.830400e+04
9.355322e-01 6.876982e+10 4.663752e+05 1.474560e+05


==> data/large-scaling/large-scaling-4-1/data_0004_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 1.718800e-02 1.518750e+01 1.000000e+01 4.241331e+04 7.290000e+02 4.000000e+00 4.000000e+00
2 1.749100e-02 7.593750e+00 1.000000e+01 2.083929e+04 7.290000e+02 4.000000e+00 4.000000e+00
4 1.775300e-02 3.796875e+00 1.000000e+01 1.026587e+04 7.290000e+02 4.000000e+00 4.000000e+00
8 1.910500e-02 1.898438e+00 1.000000e+01 4.769694e+03 7.290000e+02 4.000000e+00 4.000000e+00
16 2.663100e-02 9.492188e-01 1.000000e+01 1.710882e+03 7.290000e+02 4.000000e+00 4.000000e+00
32 2.009400e-02 4.746094e-01 1.000000e+01 1.133734e+03 7.290000e+02 4.000000e+00 4.000000e+00
64 2.576500e-02 2.373047e-01 1.000000e+01 4.420968e+02 7.290000e+02 4.000000e+00 4.000000e+00
128 2.921800e-02 1.186523e-01 1.000000e+01 1.949248e+02 7.290000e+02 4.000000e+00 4.000000e+00
256 2.453400e-02 5.932617e-02 1.000000e+01 1.160698e+02 7.290000e+02 4.000000e+00 4.000000e+00
512 2.140100e-02 2.966309e-02 1.000000e+01 6.653092e+01 7.290000e+02 4.000000e+00 4.000000e+00
1024 2.859100e-02 1.483154e-02 1.000000e+01 2.489994e+01 7.290000e+02 4.000000e+00 4.000000e+00
2048 1.815800e-02 7.415771e-03 1.000000e+01 1.960332e+01 7.290000e+02 4.000000e+00 4.000000e+00
3072 2.142700e-02 4.943848e-03 1.000000e+01 1.107503e+01 7.290000e+02 4.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-1/data_0004_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 4.792100e-03 1.518750e+01 1.000000e+01 1.521254e+05 7.290000e+02 4.000000e+00 4.000000e+00
2 5.471100e-03 7.593750e+00 1.000000e+01 6.662280e+04 7.290000e+02 4.000000e+00 4.000000e+00
4 5.721100e-03 3.796875e+00 1.000000e+01 3.185576e+04 7.290000e+02 4.000000e+00 4.000000e+00
8 6.616200e-03 1.898438e+00 1.000000e+01 1.377301e+04 7.290000e+02 4.000000e+00 4.000000e+00
16 8.847400e-03 9.492188e-01 1.000000e+01 5.149818e+03 7.290000e+02 4.000000e+00 4.000000e+00
32 6.089500e-03 4.746094e-01 1.000000e+01 3.741071e+03 7.290000e+02 4.000000e+00 4.000000e+00
64 8.580500e-03 2.373047e-01 1.000000e+01 1.327501e+03 7.290000e+02 4.000000e+00 4.000000e+00
128 6.465900e-03 1.186523e-01 1.000000e+01 8.808229e+02 7.290000e+02 4.000000e+00 4.000000e+00
256 8.129000e-03 5.932617e-02 1.000000e+01 3.503083e+02 7.290000e+02 4.000000e+00 4.000000e+00
512 8.232500e-03 2.966309e-02 1.000000e+01 1.729521e+02 7.290000e+02 4.000000e+00 4.000000e+00
1024 1.587500e-02 1.483154e-02 1.000000e+01 4.484498e+01 7.290000e+02 4.000000e+00 4.000000e+00
2048 8.525200e-03 7.415771e-03 1.000000e+01 4.175351e+01 7.290000e+02 4.000000e+00 4.000000e+00
3072 8.224200e-03 4.943848e-03 1.000000e+01 2.885444e+01 7.290000e+02 4.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-1/data_0005_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 2.890400e-02 1.023542e+02 1.000000e+01 1.699765e+05 4.913000e+03 5.000000e+00 4.000000e+00
2 3.224100e-02 5.117708e+01 1.000000e+01 7.619181e+04 4.913000e+03 5.000000e+00 4.000000e+00
4 3.220200e-02 2.558854e+01 1.000000e+01 3.814204e+04 4.913000e+03 5.000000e+00 4.000000e+00
8 3.578700e-02 1.279427e+01 1.000000e+01 1.716056e+04 4.913000e+03 5.000000e+00 4.000000e+00
16 3.820700e-02 6.397135e+00 1.000000e+01 8.036813e+03 4.913000e+03 5.000000e+00 4.000000e+00
32 3.981100e-02 3.198568e+00 1.000000e+01 3.856503e+03 4.913000e+03 5.000000e+00 4.000000e+00
64 3.629600e-02 1.599284e+00 1.000000e+01 2.114989e+03 4.913000e+03 5.000000e+00 4.000000e+00
128 3.391400e-02 7.996419e-01 1.000000e+01 1.131769e+03 4.913000e+03 5.000000e+00 4.000000e+00
256 4.729500e-02 3.998210e-01 1.000000e+01 4.057809e+02 4.913000e+03 5.000000e+00 4.000000e+00
512 3.635800e-02 1.999105e-01 1.000000e+01 2.639227e+02 4.913000e+03 5.000000e+00 4.000000e+00
1024 2.940700e-02 9.995524e-02 1.000000e+01 1.631534e+02 4.913000e+03 5.000000e+00 4.000000e+00
2048 3.332600e-02 4.997762e-02 1.000000e+01 7.198361e+01 4.913000e+03 5.000000e+00 4.000000e+00
3072 3.373000e-02 3.331841e-02 1.000000e+01 4.741429e+01 4.913000e+03 5.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-1/data_0005_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 1.011100e-02 1.023542e+02 1.000000e+01 4.859064e+05 4.913000e+03 5.000000e+00 4.000000e+00
2 9.922700e-03 5.117708e+01 1.000000e+01 2.475637e+05 4.913000e+03 5.000000e+00 4.000000e+00
4 9.715400e-03 2.558854e+01 1.000000e+01 1.264230e+05 4.913000e+03 5.000000e+00 4.000000e+00
8 1.082900e-02 1.279427e+01 1.000000e+01 5.671115e+04 4.913000e+03 5.000000e+00 4.000000e+00
16 1.115400e-02 6.397135e+00 1.000000e+01 2.752936e+04 4.913000e+03 5.000000e+00 4.000000e+00
32 1.228800e-02 3.198568e+00 1.000000e+01 1.249441e+04 4.913000e+03 5.000000e+00 4.000000e+00
64 1.368300e-02 1.599284e+00 1.000000e+01 5.610292e+03 4.913000e+03 5.000000e+00 4.000000e+00
128 1.364600e-02 7.996419e-01 1.000000e+01 2.812752e+03 4.913000e+03 5.000000e+00 4.000000e+00
256 1.287800e-02 3.998210e-01 1.000000e+01 1.490247e+03 4.913000e+03 5.000000e+00 4.000000e+00
512 1.286000e-02 1.999105e-01 1.000000e+01 7.461667e+02 4.913000e+03 5.000000e+00 4.000000e+00
1024 1.594100e-02 9.995524e-02 1.000000e+01 3.009756e+02 4.913000e+03 5.000000e+00 4.000000e+00
2048 1.572900e-02 4.997762e-02 1.000000e+01 1.525161e+02 4.913000e+03 5.000000e+00 4.000000e+00
3072 1.311800e-02 3.331841e-02 1.000000e+01 1.219152e+02 4.913000e+03 5.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-1/data_0006_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 5.736300e-02 7.486875e+02 1.000000e+01 6.264840e+05 3.593700e+04 6.000000e+00 4.000000e+00
2 5.085100e-02 3.743438e+02 1.000000e+01 3.533559e+05 3.593700e+04 6.000000e+00 4.000000e+00
4 4.598800e-02 1.871719e+02 1.000000e+01 1.953607e+05 3.593700e+04 6.000000e+00 4.000000e+00
8 4.860700e-02 9.358594e+01 1.000000e+01 9.241724e+04 3.593700e+04 6.000000e+00 4.000000e+00
16 5.143600e-02 4.679297e+01 1.000000e+01 4.366713e+04 3.593700e+04 6.000000e+00 4.000000e+00
32 5.320600e-02 2.339648e+01 1.000000e+01 2.110723e+04 3.593700e+04 6.000000e+00 4.000000e+00
64 6.156200e-02 1.169824e+01 1.000000e+01 9.121140e+03 3.593700e+04 6.000000e+00 4.000000e+00
128 4.781900e-02 5.849121e+00 1.000000e+01 5.871261e+03 3.593700e+04 6.000000e+00 4.000000e+00
256 5.210600e-02 2.924561e+00 1.000000e+01 2.694103e+03 3.593700e+04 6.000000e+00 4.000000e+00
512 5.374900e-02 1.462280e+00 1.000000e+01 1.305875e+03 3.593700e+04 6.000000e+00 4.000000e+00
1024 3.895600e-02 7.311401e-01 1.000000e+01 9.008812e+02 3.593700e+04 6.000000e+00 4.000000e+00
2048 4.772400e-02 3.655701e-01 1.000000e+01 3.676843e+02 3.593700e+04 6.000000e+00 4.000000e+00
3072 4.145900e-02 2.437134e-01 1.000000e+01 2.821641e+02 3.593700e+04 6.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-1/data_0006_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 3.536900e-02 7.486875e+02 1.000000e+01 1.016059e+06 3.593700e+04 6.000000e+00 4.000000e+00
2 2.336800e-02 3.743438e+02 1.000000e+01 7.689362e+05 3.593700e+04 6.000000e+00 4.000000e+00
4 1.752600e-02 1.871719e+02 1.000000e+01 5.126241e+05 3.593700e+04 6.000000e+00 4.000000e+00
8 1.733400e-02 9.358594e+01 1.000000e+01 2.591511e+05 3.593700e+04 6.000000e+00 4.000000e+00
16 1.668300e-02 4.679297e+01 1.000000e+01 1.346318e+05 3.593700e+04 6.000000e+00 4.000000e+00
32 1.580800e-02 2.339648e+01 1.000000e+01 7.104196e+04 3.593700e+04 6.000000e+00 4.000000e+00
64 2.516300e-02 1.169824e+01 1.000000e+01 2.231513e+04 3.593700e+04 6.000000e+00 4.000000e+00
128 3.448700e-02 5.849121e+00 1.000000e+01 8.140975e+03 3.593700e+04 6.000000e+00 4.000000e+00
256 2.913400e-02 2.924561e+00 1.000000e+01 4.818388e+03 3.593700e+04 6.000000e+00 4.000000e+00
512 2.783200e-02 1.462280e+00 1.000000e+01 2.521898e+03 3.593700e+04 6.000000e+00 4.000000e+00
1024 1.931700e-02 7.311401e-01 1.000000e+01 1.816779e+03 3.593700e+04 6.000000e+00 4.000000e+00
2048 2.090900e-02 3.655701e-01 1.000000e+01 8.392254e+02 3.593700e+04 6.000000e+00 4.000000e+00
3072 2.160500e-02 2.437134e-01 1.000000e+01 5.414599e+02 3.593700e+04 6.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-1/data_0007_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 2.389800e-01 5.721354e+03 1.000000e+01 1.149155e+06 2.746250e+05 7.000000e+00 4.000000e+00
2 1.494900e-01 2.860677e+03 1.000000e+01 9.185397e+05 2.746250e+05 7.000000e+00 4.000000e+00
4 1.020800e-01 1.430339e+03 1.000000e+01 6.725730e+05 2.746250e+05 7.000000e+00 4.000000e+00
8 8.562900e-02 7.151693e+02 1.000000e+01 4.008937e+05 2.746250e+05 7.000000e+00 4.000000e+00
16 7.955900e-02 3.575846e+02 1.000000e+01 2.157400e+05 2.746250e+05 7.000000e+00 4.000000e+00
32 7.850900e-02 1.787923e+02 1.000000e+01 1.093127e+05 2.746250e+05 7.000000e+00 4.000000e+00
64 9.188500e-02 8.939616e+01 1.000000e+01 4.669985e+04 2.746250e+05 7.000000e+00 4.000000e+00
128 8.326300e-02 4.469808e+01 1.000000e+01 2.576784e+04 2.746250e+05 7.000000e+00 4.000000e+00
256 9.477300e-02 2.234904e+01 1.000000e+01 1.131919e+04 2.746250e+05 7.000000e+00 4.000000e+00
512 8.436900e-02 1.117452e+01 1.000000e+01 6.357512e+03 2.746250e+05 7.000000e+00 4.000000e+00
1024 7.962600e-02 5.587260e+00 1.000000e+01 3.368102e+03 2.746250e+05 7.000000e+00 4.000000e+00
2048 7.521500e-02 2.793630e+00 1.000000e+01 1.782812e+03 2.746250e+05 7.000000e+00 4.000000e+00
3072 7.100100e-02 1.862420e+00 1.000000e+01 1.259083e+03 2.746250e+05 7.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-1/data_0007_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 2.197400e-01 5.721354e+03 1.000000e+01 1.249772e+06 2.746250e+05 7.000000e+00 4.000000e+00
2 1.184100e-01 2.860677e+03 1.000000e+01 1.159636e+06 2.746250e+05 7.000000e+00 4.000000e+00
4 7.176800e-02 1.430339e+03 1.000000e+01 9.566415e+05 2.746250e+05 7.000000e+00 4.000000e+00
8 4.385700e-02 7.151693e+02 1.000000e+01 7.827285e+05 2.746250e+05 7.000000e+00 4.000000e+00
16 3.291700e-02 3.575846e+02 1.000000e+01 5.214346e+05 2.746250e+05 7.000000e+00 4.000000e+00
32 3.133900e-02 1.787923e+02 1.000000e+01 2.738451e+05 2.746250e+05 7.000000e+00 4.000000e+00
64 3.885800e-02 8.939616e+01 1.000000e+01 1.104281e+05 2.746250e+05 7.000000e+00 4.000000e+00
128 3.986800e-02 4.469808e+01 1.000000e+01 5.381529e+04 2.746250e+05 7.000000e+00 4.000000e+00
256 4.143600e-02 2.234904e+01 1.000000e+01 2.588942e+04 2.746250e+05 7.000000e+00 4.000000e+00
512 5.534200e-02 1.117452e+01 1.000000e+01 9.692041e+03 2.746250e+05 7.000000e+00 4.000000e+00
1024 5.687300e-02 5.587260e+00 1.000000e+01 4.715568e+03 2.746250e+05 7.000000e+00 4.000000e+00
2048 5.430800e-02 2.793630e+00 1.000000e+01 2.469143e+03 2.746250e+05 7.000000e+00 4.000000e+00
3072 6.784900e-02 1.862420e+00 1.000000e+01 1.317575e+03 2.746250e+05 7.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-1/data_0008_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 1.679400e+00 4.472269e+04 1.000000e+01 1.278248e+06 2.146689e+06 8.000000e+00 4.000000e+00
2 8.652200e-01 2.236134e+04 1.000000e+01 1.240545e+06 2.146689e+06 8.000000e+00 4.000000e+00
4 4.495600e-01 1.118067e+04 1.000000e+01 1.193772e+06 2.146689e+06 8.000000e+00 4.000000e+00
8 2.788700e-01 5.590336e+03 1.000000e+01 9.622266e+05 2.146689e+06 8.000000e+00 4.000000e+00
16 1.908300e-01 2.795168e+03 1.000000e+01 7.030764e+05 2.146689e+06 8.000000e+00 4.000000e+00
32 1.456600e-01 1.397584e+03 1.000000e+01 4.605522e+05 2.146689e+06 8.000000e+00 4.000000e+00
64 1.398100e-01 6.987920e+02 1.000000e+01 2.399114e+05 2.146689e+06 8.000000e+00 4.000000e+00
128 1.163300e-01 3.493960e+02 1.000000e+01 1.441675e+05 2.146689e+06 8.000000e+00 4.000000e+00
256 1.219800e-01 1.746980e+02 1.000000e+01 6.874491e+04 2.146689e+06 8.000000e+00 4.000000e+00
512 4.395800e-01 8.734900e+01 1.000000e+01 9.538086e+03 2.146689e+06 8.000000e+00 4.000000e+00
1024 1.378800e-01 4.367450e+01 1.000000e+01 1.520435e+04 2.146689e+06 8.000000e+00 4.000000e+00
2048 1.613100e-01 2.183725e+01 1.000000e+01 6.497973e+03 2.146689e+06 8.000000e+00 4.000000e+00
3072 1.934400e-01 1.455817e+01 1.000000e+01 3.612448e+03 2.146689e+06 8.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-1/data_0008_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 1.800700e+00 4.472269e+04 1.000000e+01 1.192141e+06 2.146689e+06 8.000000e+00 4.000000e+00
2 8.616100e-01 2.236134e+04 1.000000e+01 1.245743e+06 2.146689e+06 8.000000e+00 4.000000e+00
4 4.417800e-01 1.118067e+04 1.000000e+01 1.214795e+06 2.146689e+06 8.000000e+00 4.000000e+00
8 2.306100e-01 5.590336e+03 1.000000e+01 1.163593e+06 2.146689e+06 8.000000e+00 4.000000e+00
16 1.378000e-01 2.795168e+03 1.000000e+01 9.736434e+05 2.146689e+06 8.000000e+00 4.000000e+00
32 8.870600e-02 1.397584e+03 1.000000e+01 7.562513e+05 2.146689e+06 8.000000e+00 4.000000e+00
64 7.638900e-02 6.987920e+02 1.000000e+01 4.390948e+05 2.146689e+06 8.000000e+00 4.000000e+00
128 5.178300e-02 3.493960e+02 1.000000e+01 3.238709e+05 2.146689e+06 8.000000e+00 4.000000e+00
256 5.324000e-02 1.746980e+02 1.000000e+01 1.575038e+05 2.146689e+06 8.000000e+00 4.000000e+00
512 5.370900e-02 8.734900e+01 1.000000e+01 7.806423e+04 2.146689e+06 8.000000e+00 4.000000e+00
1024 2.113900e-01 4.367450e+01 1.000000e+01 9.917101e+03 2.146689e+06 8.000000e+00 4.000000e+00
2048 7.054800e-02 2.183725e+01 1.000000e+01 1.485780e+04 2.146689e+06 8.000000e+00 4.000000e+00
3072 1.060200e-01 1.455817e+01 1.000000e+01 6.591134e+03 2.146689e+06 8.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-1/data_0009_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 1.204500e+01 3.536374e+05 1.000000e+01 1.409265e+06 1.697459e+07 9.000000e+00 4.000000e+00
2 5.998400e+00 1.768187e+05 1.000000e+01 1.414927e+06 1.697459e+07 9.000000e+00 4.000000e+00
4 3.673300e+00 8.840934e+04 1.000000e+01 1.155269e+06 1.697459e+07 9.000000e+00 4.000000e+00
8 1.639500e+00 4.420467e+04 1.000000e+01 1.294190e+06 1.697459e+07 9.000000e+00 4.000000e+00
16 8.371400e-01 2.210233e+04 1.000000e+01 1.267305e+06 1.697459e+07 9.000000e+00 4.000000e+00
32 4.621100e-01 1.105117e+04 1.000000e+01 1.147900e+06 1.697459e+07 9.000000e+00 4.000000e+00
64 3.931800e-01 5.525584e+03 1.000000e+01 6.745715e+05 1.697459e+07 9.000000e+00 4.000000e+00
128 2.052800e-01 2.762792e+03 1.000000e+01 6.460152e+05 1.697459e+07 9.000000e+00 4.000000e+00
256 3.933900e-01 1.381396e+03 1.000000e+01 1.685528e+05 1.697459e+07 9.000000e+00 4.000000e+00
512 1.414200e-01 6.906980e+02 1.000000e+01 2.344329e+05 1.697459e+07 9.000000e+00 4.000000e+00
1024 2.503000e-01 3.453490e+02 1.000000e+01 6.622753e+04 1.697459e+07 9.000000e+00 4.000000e+00
2048 1.431600e-01 1.726745e+02 1.000000e+01 5.789589e+04 1.697459e+07 9.000000e+00 4.000000e+00
3072 1.792200e-01 1.151163e+02 1.000000e+01 3.083129e+04 1.697459e+07 9.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-1/data_0009_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
2 8.108500e+00 1.768187e+05 1.000000e+01 1.046716e+06 1.697459e+07 9.000000e+00 4.000000e+00
4 4.031700e+00 8.840934e+04 1.000000e+01 1.052570e+06 1.697459e+07 9.000000e+00 4.000000e+00
8 1.665700e+00 4.420467e+04 1.000000e+01 1.273833e+06 1.697459e+07 9.000000e+00 4.000000e+00
16 9.786500e-01 2.210233e+04 1.000000e+01 1.084057e+06 1.697459e+07 9.000000e+00 4.000000e+00
32 5.249700e-01 1.105117e+04 1.000000e+01 1.010450e+06 1.697459e+07 9.000000e+00 4.000000e+00
64 2.748100e-01 5.525584e+03 1.000000e+01 9.651323e+05 1.697459e+07 9.000000e+00 4.000000e+00
128 1.559400e-01 2.762792e+03 1.000000e+01 8.504169e+05 1.697459e+07 9.000000e+00 4.000000e+00
256 9.524200e-02 1.381396e+03 1.000000e+01 6.961950e+05 1.697459e+07 9.000000e+00 4.000000e+00
512 1.861600e-01 6.906980e+02 1.000000e+01 1.780914e+05 1.697459e+07 9.000000e+00 4.000000e+00
1024 1.460800e-01 3.453490e+02 1.000000e+01 1.134772e+05 1.697459e+07 9.000000e+00 4.000000e+00
2048 6.345000e-02 1.726745e+02 1.000000e+01 1.306285e+05 1.697459e+07 9.000000e+00 4.000000e+00
3072 7.642800e-02 1.151163e+02 1.000000e+01 7.229790e+04 1.697459e+07 9.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-1/data_0010_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
8 1.470400e+01 3.515773e+05 1.000000e+01 1.147695e+06 1.350057e+08 1.000000e+01 4.000000e+00
16 7.303100e+00 1.757887e+05 1.000000e+01 1.155380e+06 1.350057e+08 1.000000e+01 4.000000e+00
32 4.048100e+00 8.789433e+04 1.000000e+01 1.042200e+06 1.350057e+08 1.000000e+01 4.000000e+00
64 2.035500e+00 4.394717e+04 1.000000e+01 1.036337e+06 1.350057e+08 1.000000e+01 4.000000e+00
128 1.314700e+00 2.197358e+04 1.000000e+01 8.022606e+05 1.350057e+08 1.000000e+01 4.000000e+00
256 7.709700e-01 1.098679e+04 1.000000e+01 6.840292e+05 1.350057e+08 1.000000e+01 4.000000e+00
512 6.220300e-01 5.493396e+03 1.000000e+01 4.239072e+05 1.350057e+08 1.000000e+01 4.000000e+00
1024 9.357600e-01 2.746698e+03 1.000000e+01 1.408924e+05 1.350057e+08 1.000000e+01 4.000000e+00
2048 2.442600e-01 1.373349e+03 1.000000e+01 2.698794e+05 1.350057e+08 1.000000e+01 4.000000e+00
3072 2.418800e-01 9.155660e+02 1.000000e+01 1.816900e+05 1.350057e+08 1.000000e+01 4.000000e+00


==> data/large-scaling/large-scaling-4-1/data_0010_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
32 4.003300e+00 8.789433e+04 1.000000e+01 1.053863e+06 1.350057e+08 1.000000e+01 4.000000e+00
64 2.240100e+00 4.394717e+04 1.000000e+01 9.416830e+05 1.350057e+08 1.000000e+01 4.000000e+00
128 1.283900e+00 2.197358e+04 1.000000e+01 8.215064e+05 1.350057e+08 1.000000e+01 4.000000e+00
256 6.838200e-01 1.098679e+04 1.000000e+01 7.712059e+05 1.350057e+08 1.000000e+01 4.000000e+00
512 3.984400e-01 5.493396e+03 1.000000e+01 6.617885e+05 1.350057e+08 1.000000e+01 4.000000e+00
1024 3.380900e-01 2.746698e+03 1.000000e+01 3.899598e+05 1.350057e+08 1.000000e+01 4.000000e+00
2048 1.557000e-01 1.373349e+03 1.000000e+01 4.233831e+05 1.350057e+08 1.000000e+01 4.000000e+00
3072 1.474100e-01 9.155660e+02 1.000000e+01 2.981288e+05 1.350057e+08 1.000000e+01 4.000000e+00


==> data/large-scaling/large-scaling-4-1/data_0011_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
64 1.532900e+01 3.505503e+05 1.000000e+01 1.097685e+06 1.076891e+09 1.100000e+01 4.000000e+00
128 9.554000e+00 1.752752e+05 1.000000e+01 8.805954e+05 1.076891e+09 1.100000e+01 4.000000e+00
256 4.995300e+00 8.763758e+04 1.000000e+01 8.421124e+05 1.076891e+09 1.100000e+01 4.000000e+00
512 2.812400e+00 4.381879e+04 1.000000e+01 7.478673e+05 1.076891e+09 1.100000e+01 4.000000e+00
1024 2.576300e+00 2.190940e+04 1.000000e+01 4.082021e+05 1.076891e+09 1.100000e+01 4.000000e+00
2048 8.729700e-01 1.095470e+04 1.000000e+01 6.023409e+05 1.076891e+09 1.100000e+01 4.000000e+00
3072 7.309100e-01 7.303132e+03 1.000000e+01 4.796081e+05 1.076891e+09 1.100000e+01 4.000000e+00


==> data/large-scaling/large-scaling-4-1/data_0011_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
256 5.367600e+00 8.763758e+04 1.000000e+01 7.837030e+05 1.076891e+09 1.100000e+01 4.000000e+00
512 2.663400e+00 4.381879e+04 1.000000e+01 7.897056e+05 1.076891e+09 1.100000e+01 4.000000e+00
1024 1.740800e+00 2.190940e+04 1.000000e+01 6.041194e+05 1.076891e+09 1.100000e+01 4.000000e+00
2048 8.955000e-01 1.095470e+04 1.000000e+01 5.871865e+05 1.076891e+09 1.100000e+01 4.000000e+00
3072 6.236500e-01 7.303132e+03 1.000000e+01 5.620947e+05 1.076891e+09 1.100000e+01 4.000000e+00


==> data/large-scaling/large-scaling-4-1/data_0012_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
512 1.961600e+01 3.500376e+05 1.000000e+01 8.565357e+05 8.602524e+09 1.200000e+01 4.000000e+00
1024 1.270900e+01 1.750188e+05 1.000000e+01 6.610199e+05 8.602524e+09 1.200000e+01 4.000000e+00
2048 6.251800e+00 8.750940e+04 1.000000e+01 6.718787e+05 8.602524e+09 1.200000e+01 4.000000e+00
3072 4.193500e+00 5.833960e+04 1.000000e+01 6.677717e+05 8.602524e+09 1.200000e+01 4.000000e+00


==> data/large-scaling/large-scaling-4-1/data_0012_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
2048 6.837400e+00 8.750940e+04 1.000000e+01 6.143345e+05 8.602524e+09 1.200000e+01 4.000000e+00
3072 4.673200e+00 5.833960e+04 1.000000e+01 5.992255e+05 8.602524e+09 1.200000e+01 4.000000e+00


==> data/large-scaling/large-scaling-4-1/speedup_0.tex <==
speedup n_dofs n_dofs_norm ranks
3.586737e+00 7.290000e+02 1.518750e+01 4.800000e+01
2.858669e+00 4.913000e+03 1.023542e+02 4.800000e+01
1.621844e+00 3.593700e+04 7.486875e+02 4.800000e+01
3.196980e+00 7.290000e+02 7.593750e+00 9.600000e+01
3.249216e+00 4.913000e+03 5.117708e+01 9.600000e+01
2.176096e+00 3.593700e+04 3.743438e+02 9.600000e+01
3.103075e+00 7.290000e+02 3.796875e+00 1.920000e+02
3.314532e+00 4.913000e+03 2.558854e+01 1.920000e+02
2.623987e+00 3.593700e+04 1.871719e+02 1.920000e+02
2.887609e+00 7.290000e+02 1.898438e+00 3.840000e+02
3.304737e+00 4.913000e+03 1.279427e+01 3.840000e+02
2.804142e+00 3.593700e+04 9.358594e+01 3.840000e+02
1.952459e+00 2.746250e+05 7.151693e+02 3.840000e+02
3.010037e+00 7.290000e+02 9.492188e-01 7.680000e+02
3.425408e+00 4.913000e+03 6.397135e+00 7.680000e+02
3.083139e+00 3.593700e+04 4.679297e+01 7.680000e+02
2.416958e+00 2.746250e+05 3.575846e+02 7.680000e+02
3.299778e+00 7.290000e+02 4.746094e-01 1.536000e+03
3.239827e+00 4.913000e+03 3.198568e+00 1.536000e+03
3.365764e+00 3.593700e+04 2.339648e+01 1.536000e+03
2.505153e+00 2.746250e+05 1.787923e+02 1.536000e+03
3.002739e+00 7.290000e+02 2.373047e-01 3.072000e+03
2.652635e+00 4.913000e+03 1.599284e+00 3.072000e+03
2.446529e+00 3.593700e+04 1.169824e+01 3.072000e+03
2.364635e+00 2.746250e+05 8.939616e+01 3.072000e+03
1.830237e+00 2.146689e+06 6.987920e+02 3.072000e+03
4.518783e+00 7.290000e+02 1.186523e-01 6.144000e+03
2.485270e+00 4.913000e+03 7.996419e-01 6.144000e+03
1.386580e+00 3.593700e+04 5.849121e+00 6.144000e+03
2.088467e+00 2.746250e+05 4.469808e+01 6.144000e+03
2.246490e+00 2.146689e+06 3.493960e+02 6.144000e+03
3.018083e+00 7.290000e+02 5.932617e-02 1.228800e+04
3.672542e+00 4.913000e+03 3.998210e-01 1.228800e+04
1.788495e+00 3.593700e+04 2.924561e+00 1.228800e+04
2.287214e+00 2.746250e+05 2.234904e+01 1.228800e+04
2.291134e+00 2.146689e+06 1.746980e+02 1.228800e+04
2.599575e+00 7.290000e+02 2.966309e-02 2.457600e+04
2.827216e+00 4.913000e+03 1.999105e-01 2.457600e+04
1.931194e+00 3.593700e+04 1.462280e+00 2.457600e+04
1.524502e+00 2.746250e+05 1.117452e+01 2.457600e+04
8.184476e+00 2.146689e+06 8.734900e+01 2.457600e+04
7.596691e-01 1.697459e+07 6.906980e+02 2.457600e+04
1.801008e+00 7.290000e+02 1.483154e-02 4.915200e+04
1.844740e+00 4.913000e+03 9.995524e-02 4.915200e+04
2.016669e+00 3.593700e+04 7.311401e-01 4.915200e+04
1.400067e+00 2.746250e+05 5.587260e+00 4.915200e+04
6.522541e-01 2.146689e+06 4.367450e+01 4.915200e+04
1.713445e+00 1.697459e+07 3.453490e+02 4.915200e+04
2.129921e+00 7.290000e+02 7.415771e-03 9.830400e+04
2.118762e+00 4.913000e+03 4.997762e-02 9.830400e+04
2.282462e+00 3.593700e+04 3.655701e-01 9.830400e+04
1.384971e+00 2.746250e+05 2.793630e+00 9.830400e+04
2.286528e+00 2.146689e+06 2.183725e+01 9.830400e+04
2.256265e+00 1.697459e+07 1.726745e+02 9.830400e+04
2.605360e+00 7.290000e+02 4.943848e-03 1.474560e+05
2.571276e+00 4.913000e+03 3.331841e-02 1.474560e+05
1.918954e+00 3.593700e+04 2.437134e-01 1.474560e+05
1.046456e+00 2.746250e+05 1.862420e+00 1.474560e+05
1.824561e+00 2.146689e+06 1.455817e+01 1.474560e+05
2.344952e+00 1.697459e+07 1.151163e+02 1.474560e+05
1.640866e+00 1.350057e+08 9.155660e+02 1.474560e+05


==> data/large-scaling/large-scaling-4-1/speedup_1.tex <==
speedup n_dofs n_dofs_norm ranks
1.087558e+00 2.746250e+05 5.721354e+03 4.800000e+01
1.262478e+00 2.746250e+05 2.860677e+03 9.600000e+01
1.422361e+00 2.746250e+05 1.430339e+03 1.920000e+02
1.209271e+00 2.146689e+06 5.590336e+03 3.840000e+02
1.384833e+00 2.146689e+06 2.795168e+03 7.680000e+02
1.642054e+00 2.146689e+06 1.397584e+03 1.536000e+03
1.430734e+00 1.697459e+07 5.525584e+03 3.072000e+03
1.316404e+00 1.697459e+07 2.762792e+03 6.144000e+03
4.130426e+00 1.697459e+07 1.381396e+03 1.228800e+04
1.561164e+00 1.350057e+08 5.493396e+03 2.457600e+04
2.767784e+00 1.350057e+08 2.746698e+03 4.915200e+04
1.568786e+00 1.350057e+08 1.373349e+03 9.830400e+04
1.171987e+00 1.076891e+09 7.303132e+03 1.474560e+05


==> data/large-scaling/large-scaling-4-1/speedup_2.tex <==
speedup n_dofs n_dofs_norm ranks
9.326373e-01 2.146689e+06 4.472269e+04 4.800000e+01
1.004190e+00 2.146689e+06 2.236134e+04 9.600000e+01
1.017611e+00 2.146689e+06 1.118067e+04 1.920000e+02
9.111045e-01 1.697459e+07 8.840934e+04 1.920000e+02
9.842709e-01 1.697459e+07 4.420467e+04 3.840000e+02
8.554029e-01 1.697459e+07 2.210233e+04 7.680000e+02
8.802598e-01 1.697459e+07 1.105117e+04 1.536000e+03
1.011191e+00 1.350057e+08 8.789433e+04 1.536000e+03
9.086648e-01 1.350057e+08 4.394717e+04 3.072000e+03
1.023989e+00 1.350057e+08 2.197358e+04 6.144000e+03
1.127446e+00 1.350057e+08 1.098679e+04 1.228800e+04
9.306394e-01 1.076891e+09 8.763758e+04 1.228800e+04
1.055944e+00 1.076891e+09 4.381879e+04 2.457600e+04
1.479952e+00 1.076891e+09 2.190940e+04 4.915200e+04
9.748409e-01 1.076891e+09 1.095470e+04 9.830400e+04
9.143534e-01 8.602524e+09 8.750940e+04 9.830400e+04
8.973509e-01 8.602524e+09 5.833960e+04 1.474560e+05


==> data/large-scaling/large-scaling-4-1/speedup_3.tex <==
speedup n_dofs n_dofs_norm ranks
7.397669e-01 1.697459e+07 1.768187e+05 9.600000e+01


==> data/large-scaling/large-scaling-4-4/data_0004_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 4.478100e-02 7.486875e+02 1.000000e+01 8.025055e+05 3.593700e+04 4.000000e+00 4.000000e+00
2 3.955800e-02 3.743438e+02 1.000000e+01 4.542318e+05 3.593700e+04 4.000000e+00 4.000000e+00
4 3.940000e-02 1.871719e+02 1.000000e+01 2.280266e+05 3.593700e+04 4.000000e+00 4.000000e+00
8 3.914300e-02 9.358594e+01 1.000000e+01 1.147619e+05 3.593700e+04 4.000000e+00 4.000000e+00
16 3.964300e-02 4.679297e+01 1.000000e+01 5.665723e+04 3.593700e+04 4.000000e+00 4.000000e+00
32 4.598200e-02 2.339648e+01 1.000000e+01 2.442328e+04 3.593700e+04 4.000000e+00 4.000000e+00
64 5.316800e-02 1.169824e+01 1.000000e+01 1.056116e+04 3.593700e+04 4.000000e+00 4.000000e+00
128 4.389800e-02 5.849121e+00 1.000000e+01 6.395686e+03 3.593700e+04 4.000000e+00 4.000000e+00
256 4.719600e-02 2.924561e+00 1.000000e+01 2.974381e+03 3.593700e+04 4.000000e+00 4.000000e+00
512 4.511500e-02 1.462280e+00 1.000000e+01 1.555790e+03 3.593700e+04 4.000000e+00 4.000000e+00
1024 4.579900e-02 7.311401e-01 1.000000e+01 7.662771e+02 3.593700e+04 4.000000e+00 4.000000e+00
2048 3.933200e-02 3.655701e-01 1.000000e+01 4.461345e+02 3.593700e+04 4.000000e+00 4.000000e+00
3072 1.828900e-01 2.437134e-01 1.000000e+01 6.396327e+01 3.593700e+04 4.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-4/data_0004_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 1.725200e-02 7.486875e+02 1.000000e+01 2.083063e+06 3.593700e+04 4.000000e+00 4.000000e+00
2 1.496600e-02 3.743438e+02 1.000000e+01 1.200621e+06 3.593700e+04 4.000000e+00 4.000000e+00
4 1.444800e-02 1.871719e+02 1.000000e+01 6.218335e+05 3.593700e+04 4.000000e+00 4.000000e+00
8 1.347700e-02 9.358594e+01 1.000000e+01 3.333179e+05 3.593700e+04 4.000000e+00 4.000000e+00
16 1.343900e-02 4.679297e+01 1.000000e+01 1.671302e+05 3.593700e+04 4.000000e+00 4.000000e+00
32 1.372500e-02 2.339648e+01 1.000000e+01 8.182377e+04 3.593700e+04 4.000000e+00 4.000000e+00
64 1.359300e-02 1.169824e+01 1.000000e+01 4.130918e+04 3.593700e+04 4.000000e+00 4.000000e+00
128 1.513200e-02 5.849121e+00 1.000000e+01 1.855391e+04 3.593700e+04 4.000000e+00 4.000000e+00
256 1.562300e-02 2.924561e+00 1.000000e+01 8.985400e+03 3.593700e+04 4.000000e+00 4.000000e+00
512 1.788200e-02 1.462280e+00 1.000000e+01 3.925146e+03 3.593700e+04 4.000000e+00 4.000000e+00
1024 1.981100e-02 7.311401e-01 1.000000e+01 1.771477e+03 3.593700e+04 4.000000e+00 4.000000e+00
2048 1.566300e-02 3.655701e-01 1.000000e+01 1.120307e+03 3.593700e+04 4.000000e+00 4.000000e+00
3072 1.793600e-01 2.437134e-01 1.000000e+01 6.522214e+01 3.593700e+04 4.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-4/data_0005_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 1.106100e-01 5.721354e+03 1.000000e+01 2.482823e+06 2.746250e+05 5.000000e+00 4.000000e+00
2 9.154200e-02 2.860677e+03 1.000000e+01 1.499995e+06 2.746250e+05 5.000000e+00 4.000000e+00
4 8.505900e-02 1.430339e+03 1.000000e+01 8.071603e+05 2.746250e+05 5.000000e+00 4.000000e+00
8 8.595200e-02 7.151693e+02 1.000000e+01 3.993872e+05 2.746250e+05 5.000000e+00 4.000000e+00
16 7.793900e-02 3.575846e+02 1.000000e+01 2.202243e+05 2.746250e+05 5.000000e+00 4.000000e+00
32 8.279400e-02 1.787923e+02 1.000000e+01 1.036552e+05 2.746250e+05 5.000000e+00 4.000000e+00
64 8.228400e-02 8.939616e+01 1.000000e+01 5.214885e+04 2.746250e+05 5.000000e+00 4.000000e+00
128 7.613300e-02 4.469808e+01 1.000000e+01 2.818105e+04 2.746250e+05 5.000000e+00 4.000000e+00
256 7.873800e-02 2.234904e+01 1.000000e+01 1.362435e+04 2.746250e+05 5.000000e+00 4.000000e+00
512 7.923600e-02 1.117452e+01 1.000000e+01 6.769359e+03 2.746250e+05 5.000000e+00 4.000000e+00
1024 8.057200e-02 5.587260e+00 1.000000e+01 3.328557e+03 2.746250e+05 5.000000e+00 4.000000e+00
2048 8.121500e-02 2.793630e+00 1.000000e+01 1.651102e+03 2.746250e+05 5.000000e+00 4.000000e+00
3072 7.638200e-02 1.862420e+00 1.000000e+01 1.170383e+03 2.746250e+05 5.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-4/data_0005_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 7.468300e-02 5.721354e+03 1.000000e+01 3.677209e+06 2.746250e+05 5.000000e+00 4.000000e+00
2 4.337800e-02 2.860677e+03 1.000000e+01 3.165487e+06 2.746250e+05 5.000000e+00 4.000000e+00
4 2.956300e-02 1.430339e+03 1.000000e+01 2.322371e+06 2.746250e+05 5.000000e+00 4.000000e+00
8 2.803700e-02 7.151693e+02 1.000000e+01 1.224387e+06 2.746250e+05 5.000000e+00 4.000000e+00
16 2.330200e-02 3.575846e+02 1.000000e+01 7.365918e+05 2.746250e+05 5.000000e+00 4.000000e+00
32 2.224500e-02 1.787923e+02 1.000000e+01 3.857960e+05 2.746250e+05 5.000000e+00 4.000000e+00
64 2.058500e-02 8.939616e+01 1.000000e+01 2.084535e+05 2.746250e+05 5.000000e+00 4.000000e+00
128 2.105700e-02 4.469808e+01 1.000000e+01 1.018905e+05 2.746250e+05 5.000000e+00 4.000000e+00
256 2.285900e-02 2.234904e+01 1.000000e+01 4.692917e+04 2.746250e+05 5.000000e+00 4.000000e+00
512 1.998800e-02 1.117452e+01 1.000000e+01 2.683495e+04 2.746250e+05 5.000000e+00 4.000000e+00
1024 2.453400e-02 5.587260e+00 1.000000e+01 1.093130e+04 2.746250e+05 5.000000e+00 4.000000e+00
2048 2.328100e-02 2.793630e+00 1.000000e+01 5.759814e+03 2.746250e+05 5.000000e+00 4.000000e+00
3072 2.319700e-02 1.862420e+00 1.000000e+01 3.853781e+03 2.746250e+05 5.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-4/data_0006_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 6.630100e-01 4.472269e+04 1.000000e+01 3.237793e+06 2.146689e+06 6.000000e+00 4.000000e+00
2 3.395000e-01 2.236134e+04 1.000000e+01 3.161545e+06 2.146689e+06 6.000000e+00 4.000000e+00
4 2.034200e-01 1.118067e+04 1.000000e+01 2.638247e+06 2.146689e+06 6.000000e+00 4.000000e+00
8 1.587700e-01 5.590336e+03 1.000000e+01 1.690093e+06 2.146689e+06 6.000000e+00 4.000000e+00
16 1.336700e-01 2.795168e+03 1.000000e+01 1.003726e+06 2.146689e+06 6.000000e+00 4.000000e+00
32 1.194200e-01 1.397584e+03 1.000000e+01 5.617487e+05 2.146689e+06 6.000000e+00 4.000000e+00
64 1.230500e-01 6.987920e+02 1.000000e+01 2.725885e+05 2.146689e+06 6.000000e+00 4.000000e+00
128 1.060400e-01 3.493960e+02 1.000000e+01 1.581574e+05 2.146689e+06 6.000000e+00 4.000000e+00
256 1.124400e-01 1.746980e+02 1.000000e+01 7.457759e+04 2.146689e+06 6.000000e+00 4.000000e+00
512 1.074700e-01 8.734900e+01 1.000000e+01 3.901323e+04 2.146689e+06 6.000000e+00 4.000000e+00
1024 1.041600e-01 4.367450e+01 1.000000e+01 2.012650e+04 2.146689e+06 6.000000e+00 4.000000e+00
2048 1.093100e-01 2.183725e+01 1.000000e+01 9.589132e+03 2.146689e+06 6.000000e+00 4.000000e+00
3072 1.054200e-01 1.455817e+01 1.000000e+01 6.628647e+03 2.146689e+06 6.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-4/data_0006_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 8.553200e-01 4.472269e+04 1.000000e+01 2.509808e+06 2.146689e+06 6.000000e+00 4.000000e+00
2 3.653800e-01 2.236134e+04 1.000000e+01 2.937612e+06 2.146689e+06 6.000000e+00 4.000000e+00
4 1.662300e-01 1.118067e+04 1.000000e+01 3.228492e+06 2.146689e+06 6.000000e+00 4.000000e+00
8 8.759500e-02 5.590336e+03 1.000000e+01 3.063373e+06 2.146689e+06 6.000000e+00 4.000000e+00
16 5.333800e-02 2.795168e+03 1.000000e+01 2.515431e+06 2.146689e+06 6.000000e+00 4.000000e+00
32 4.106400e-02 1.397584e+03 1.000000e+01 1.633646e+06 2.146689e+06 6.000000e+00 4.000000e+00
64 4.307400e-02 6.987920e+02 1.000000e+01 7.787068e+05 2.146689e+06 6.000000e+00 4.000000e+00
128 3.513400e-02 3.493960e+02 1.000000e+01 4.773441e+05 2.146689e+06 6.000000e+00 4.000000e+00
256 3.478400e-02 1.746980e+02 1.000000e+01 2.410736e+05 2.146689e+06 6.000000e+00 4.000000e+00
512 2.902100e-02 8.734900e+01 1.000000e+01 1.444730e+05 2.146689e+06 6.000000e+00 4.000000e+00
1024 3.202100e-02 4.367450e+01 1.000000e+01 6.546879e+04 2.146689e+06 6.000000e+00 4.000000e+00
2048 2.975100e-02 2.183725e+01 1.000000e+01 3.523203e+04 2.146689e+06 6.000000e+00 4.000000e+00
3072 3.302700e-02 1.455817e+01 1.000000e+01 2.115820e+04 2.146689e+06 6.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-4/data_0007_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 6.544700e+00 3.536374e+05 1.000000e+01 2.593640e+06 1.697459e+07 7.000000e+00 4.000000e+00
2 3.185700e+00 1.768187e+05 1.000000e+01 2.664186e+06 1.697459e+07 7.000000e+00 4.000000e+00
4 1.514900e+00 8.840934e+04 1.000000e+01 2.801273e+06 1.697459e+07 7.000000e+00 4.000000e+00
8 7.586300e-01 4.420467e+04 1.000000e+01 2.796916e+06 1.697459e+07 7.000000e+00 4.000000e+00
16 3.887600e-01 2.210233e+04 1.000000e+01 2.728964e+06 1.697459e+07 7.000000e+00 4.000000e+00
32 2.664400e-01 1.105117e+04 1.000000e+01 1.990902e+06 1.697459e+07 7.000000e+00 4.000000e+00
64 2.171200e-01 5.525584e+03 1.000000e+01 1.221573e+06 1.697459e+07 7.000000e+00 4.000000e+00
128 1.821100e-01 2.762792e+03 1.000000e+01 7.282083e+05 1.697459e+07 7.000000e+00 4.000000e+00
256 1.780100e-01 1.381396e+03 1.000000e+01 3.724903e+05 1.697459e+07 7.000000e+00 4.000000e+00
512 1.559900e-01 6.906980e+02 1.000000e+01 2.125361e+05 1.697459e+07 7.000000e+00 4.000000e+00
1024 2.251400e-01 3.453490e+02 1.000000e+01 7.362864e+04 1.697459e+07 7.000000e+00 4.000000e+00
2048 1.429000e-01 1.726745e+02 1.000000e+01 5.800123e+04 1.697459e+07 7.000000e+00 4.000000e+00
3072 1.398400e-01 1.151163e+02 1.000000e+01 3.951361e+04 1.697459e+07 7.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-4/data_0007_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 7.218100e+00 3.536374e+05 1.000000e+01 2.351671e+06 1.697459e+07 7.000000e+00 4.000000e+00
2 3.831600e+00 1.768187e+05 1.000000e+01 2.215079e+06 1.697459e+07 7.000000e+00 4.000000e+00
4 1.816100e+00 8.840934e+04 1.000000e+01 2.336682e+06 1.697459e+07 7.000000e+00 4.000000e+00
8 8.888300e-01 4.420467e+04 1.000000e+01 2.387210e+06 1.697459e+07 7.000000e+00 4.000000e+00
16 3.855600e-01 2.210233e+04 1.000000e+01 2.751613e+06 1.697459e+07 7.000000e+00 4.000000e+00
32 1.832600e-01 1.105117e+04 1.000000e+01 2.894554e+06 1.697459e+07 7.000000e+00 4.000000e+00
64 1.034700e-01 5.525584e+03 1.000000e+01 2.563333e+06 1.697459e+07 7.000000e+00 4.000000e+00
128 6.744900e-02 2.762792e+03 1.000000e+01 1.966137e+06 1.697459e+07 7.000000e+00 4.000000e+00
256 5.589800e-02 1.381396e+03 1.000000e+01 1.186214e+06 1.697459e+07 7.000000e+00 4.000000e+00
512 4.824600e-02 6.906980e+02 1.000000e+01 6.871762e+05 1.697459e+07 7.000000e+00 4.000000e+00
1024 5.950900e-02 3.453490e+02 1.000000e+01 2.785587e+05 1.697459e+07 7.000000e+00 4.000000e+00
2048 4.910500e-02 1.726745e+02 1.000000e+01 1.687888e+05 1.697459e+07 7.000000e+00 4.000000e+00
3072 4.635900e-02 1.151163e+02 1.000000e+01 1.191912e+05 1.697459e+07 7.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-4/data_0008_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
4 1.437200e+01 7.031547e+05 1.000000e+01 2.348415e+06 1.350057e+08 8.000000e+00 4.000000e+00
8 7.019400e+00 3.515773e+05 1.000000e+01 2.404153e+06 1.350057e+08 8.000000e+00 4.000000e+00
16 3.282900e+00 1.757887e+05 1.000000e+01 2.570245e+06 1.350057e+08 8.000000e+00 4.000000e+00
32 1.593100e+00 8.789433e+04 1.000000e+01 2.648251e+06 1.350057e+08 8.000000e+00 4.000000e+00
64 8.507900e-01 4.394717e+04 1.000000e+01 2.479418e+06 1.350057e+08 8.000000e+00 4.000000e+00
128 5.469900e-01 2.197358e+04 1.000000e+01 1.928247e+06 1.350057e+08 8.000000e+00 4.000000e+00
256 4.954100e-01 1.098679e+04 1.000000e+01 1.064504e+06 1.350057e+08 8.000000e+00 4.000000e+00
512 2.351500e-01 5.493396e+03 1.000000e+01 1.121340e+06 1.350057e+08 8.000000e+00 4.000000e+00
1024 8.328900e-01 2.746698e+03 1.000000e+01 1.582940e+05 1.350057e+08 8.000000e+00 4.000000e+00
2048 3.322200e-01 1.373349e+03 1.000000e+01 1.984250e+05 1.350057e+08 8.000000e+00 4.000000e+00
3072 2.423500e-01 9.155660e+02 1.000000e+01 1.813376e+05 1.350057e+08 8.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-4/data_0008_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
8 7.488900e+00 3.515773e+05 1.000000e+01 2.253430e+06 1.350057e+08 8.000000e+00 4.000000e+00
16 3.841300e+00 1.757887e+05 1.000000e+01 2.196615e+06 1.350057e+08 8.000000e+00 4.000000e+00
32 1.886400e+00 8.789433e+04 1.000000e+01 2.236497e+06 1.350057e+08 8.000000e+00 4.000000e+00
64 9.191200e-01 4.394717e+04 1.000000e+01 2.295091e+06 1.350057e+08 8.000000e+00 4.000000e+00
128 3.982300e-01 2.197358e+04 1.000000e+01 2.648550e+06 1.350057e+08 8.000000e+00 4.000000e+00
256 1.930400e-01 1.098679e+04 1.000000e+01 2.731900e+06 1.350057e+08 8.000000e+00 4.000000e+00
512 1.144900e-01 5.493396e+03 1.000000e+01 2.303109e+06 1.350057e+08 8.000000e+00 4.000000e+00
1024 2.188800e-01 2.746698e+03 1.000000e+01 6.023460e+05 1.350057e+08 8.000000e+00 4.000000e+00
2048 7.872000e-02 1.373349e+03 1.000000e+01 8.374079e+05 1.350057e+08 8.000000e+00 4.000000e+00
3072 7.734400e-02 9.155660e+02 1.000000e+01 5.682040e+05 1.350057e+08 8.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-4/data_0009_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
32 1.395000e+01 7.011007e+05 1.000000e+01 2.412389e+06 1.076891e+09 9.000000e+00 4.000000e+00
64 7.082000e+00 3.505503e+05 1.000000e+01 2.375941e+06 1.076891e+09 9.000000e+00 4.000000e+00
128 4.052800e+00 1.752752e+05 1.000000e+01 2.075900e+06 1.076891e+09 9.000000e+00 4.000000e+00
256 2.116500e+00 8.763758e+04 1.000000e+01 1.987528e+06 1.076891e+09 9.000000e+00 4.000000e+00
512 1.261500e+00 4.381879e+04 1.000000e+01 1.667302e+06 1.076891e+09 9.000000e+00 4.000000e+00
1024 1.299800e+00 2.190940e+04 1.000000e+01 8.090868e+05 1.076891e+09 9.000000e+00 4.000000e+00
2048 4.601400e-01 1.095470e+04 1.000000e+01 1.142751e+06 1.076891e+09 9.000000e+00 4.000000e+00
3072 4.065200e-01 7.303132e+03 1.000000e+01 8.623200e+05 1.076891e+09 9.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-4/data_0009_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
64 7.490000e+00 3.505503e+05 1.000000e+01 2.246517e+06 1.076891e+09 9.000000e+00 4.000000e+00
128 4.324600e+00 1.752752e+05 1.000000e+01 1.945430e+06 1.076891e+09 9.000000e+00 4.000000e+00
256 2.185800e+00 8.763758e+04 1.000000e+01 1.924515e+06 1.076891e+09 9.000000e+00 4.000000e+00
512 1.102400e+00 4.381879e+04 1.000000e+01 1.907930e+06 1.076891e+09 9.000000e+00 4.000000e+00
1024 6.639600e-01 2.190940e+04 1.000000e+01 1.583907e+06 1.076891e+09 9.000000e+00 4.000000e+00
2048 2.903000e-01 1.095470e+04 1.000000e+01 1.811318e+06 1.076891e+09 9.000000e+00 4.000000e+00
3072 2.174400e-01 7.303132e+03 1.000000e+01 1.612170e+06 1.076891e+09 9.000000e+00 4.000000e+00


==> data/large-scaling/large-scaling-4-4/data_0010_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
256 1.623800e+01 7.000752e+05 1.000000e+01 2.069443e+06 8.602524e+09 1.000000e+01 4.000000e+00
512 8.464100e+00 3.500376e+05 1.000000e+01 1.985067e+06 8.602524e+09 1.000000e+01 4.000000e+00
1024 5.204900e+00 1.750188e+05 1.000000e+01 1.614037e+06 8.602524e+09 1.000000e+01 4.000000e+00
2048 3.658900e+00 8.750940e+04 1.000000e+01 1.148009e+06 8.602524e+09 1.000000e+01 4.000000e+00
3072 1.660500e+00 5.833960e+04 1.000000e+01 1.686420e+06 8.602524e+09 1.000000e+01 4.000000e+00


==> data/large-scaling/large-scaling-4-4/data_0010_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
512 8.496500e+00 3.500376e+05 1.000000e+01 1.977497e+06 8.602524e+09 1.000000e+01 4.000000e+00
1024 4.936900e+00 1.750188e+05 1.000000e+01 1.701655e+06 8.602524e+09 1.000000e+01 4.000000e+00
2048 3.100900e+00 8.750940e+04 1.000000e+01 1.354591e+06 8.602524e+09 1.000000e+01 4.000000e+00
3072 1.799400e+00 5.833960e+04 1.000000e+01 1.556241e+06 8.602524e+09 1.000000e+01 4.000000e+00


==> data/large-scaling/large-scaling-4-4/data_0011_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
2048 2.062000e+01 6.995628e+05 1.000000e+01 1.628468e+06 6.876982e+10 1.100000e+01 4.000000e+00
3072 1.290000e+01 4.663752e+05 1.000000e+01 1.735350e+06 6.876982e+10 1.100000e+01 4.000000e+00


==> data/large-scaling/large-scaling-4-4/data_0011_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
3072 1.322100e+01 4.663752e+05 1.000000e+01 1.693216e+06 6.876982e+10 1.100000e+01 4.000000e+00


==> data/large-scaling/large-scaling-4-4/speedup_0.tex <==
speedup n_dofs n_dofs_norm ranks
2.595699e+00 3.593700e+04 7.486875e+02 4.800000e+01
2.643191e+00 3.593700e+04 3.743438e+02 9.600000e+01
2.727021e+00 3.593700e+04 1.871719e+02 1.920000e+02
2.904430e+00 3.593700e+04 9.358594e+01 3.840000e+02
3.065663e+00 2.746250e+05 7.151693e+02 3.840000e+02
2.949847e+00 3.593700e+04 4.679297e+01 7.680000e+02
3.344734e+00 2.746250e+05 3.575846e+02 7.680000e+02
3.350237e+00 3.593700e+04 2.339648e+01 1.536000e+03
3.721915e+00 2.746250e+05 1.787923e+02 1.536000e+03
3.911425e+00 3.593700e+04 1.169824e+01 3.072000e+03
3.997280e+00 2.746250e+05 8.939616e+01 3.072000e+03
2.856712e+00 2.146689e+06 6.987920e+02 3.072000e+03
2.901004e+00 3.593700e+04 5.849121e+00 6.144000e+03
3.615567e+00 2.746250e+05 4.469808e+01 6.144000e+03
3.018159e+00 2.146689e+06 3.493960e+02 6.144000e+03
3.020931e+00 3.593700e+04 2.924561e+00 1.228800e+04
3.444508e+00 2.746250e+05 2.234904e+01 1.228800e+04
3.232521e+00 2.146689e+06 1.746980e+02 1.228800e+04
2.522928e+00 3.593700e+04 1.462280e+00 2.457600e+04
3.964179e+00 2.746250e+05 1.117452e+01 2.457600e+04
3.703180e+00 2.146689e+06 8.734900e+01 2.457600e+04
3.233221e+00 1.697459e+07 6.906980e+02 2.457600e+04
2.311796e+00 3.593700e+04 7.311401e-01 4.915200e+04
3.284096e+00 2.746250e+05 5.587260e+00 4.915200e+04
3.252865e+00 2.146689e+06 4.367450e+01 4.915200e+04
3.783293e+00 1.697459e+07 3.453490e+02 4.915200e+04
2.511141e+00 3.593700e+04 3.655701e-01 9.830400e+04
3.488467e+00 2.746250e+05 2.793630e+00 9.830400e+04
3.674162e+00 2.146689e+06 2.183725e+01 9.830400e+04
2.910091e+00 1.697459e+07 1.726745e+02 9.830400e+04
1.019681e+00 3.593700e+04 2.437134e-01 1.474560e+05
3.292753e+00 2.746250e+05 1.862420e+00 1.474560e+05
3.191934e+00 2.146689e+06 1.455817e+01 1.474560e+05
3.016459e+00 1.697459e+07 1.151163e+02 1.474560e+05
3.133404e+00 1.350057e+08 9.155660e+02 1.474560e+05


==> data/large-scaling/large-scaling-4-4/speedup_1.tex <==
speedup n_dofs n_dofs_norm ranks
1.481060e+00 2.746250e+05 5.721354e+03 4.800000e+01
2.110332e+00 2.746250e+05 2.860677e+03 9.600000e+01
2.877211e+00 2.746250e+05 1.430339e+03 1.920000e+02
1.812546e+00 2.146689e+06 5.590336e+03 3.840000e+02
2.506093e+00 2.146689e+06 2.795168e+03 7.680000e+02
2.908143e+00 2.146689e+06 1.397584e+03 1.536000e+03
2.098386e+00 1.697459e+07 5.525584e+03 3.072000e+03
2.699966e+00 1.697459e+07 2.762792e+03 6.144000e+03
3.184550e+00 1.697459e+07 1.381396e+03 1.228800e+04
2.053891e+00 1.350057e+08 5.493396e+03 2.457600e+04
3.805236e+00 1.350057e+08 2.746698e+03 4.915200e+04
4.220274e+00 1.350057e+08 1.373349e+03 9.830400e+04
1.869573e+00 1.076891e+09 7.303132e+03 1.474560e+05


==> data/large-scaling/large-scaling-4-4/speedup_2.tex <==
speedup n_dofs n_dofs_norm ranks
7.751602e-01 2.146689e+06 4.472269e+04 4.800000e+01
9.291696e-01 2.146689e+06 2.236134e+04 9.600000e+01
1.223726e+00 2.146689e+06 1.118067e+04 1.920000e+02
8.341501e-01 1.697459e+07 8.840934e+04 1.920000e+02
8.535153e-01 1.697459e+07 4.420467e+04 3.840000e+02
1.008300e+00 1.697459e+07 2.210233e+04 7.680000e+02
1.453891e+00 1.697459e+07 1.105117e+04 1.536000e+03
8.445187e-01 1.350057e+08 8.789433e+04 1.536000e+03
9.256572e-01 1.350057e+08 4.394717e+04 3.072000e+03
1.373553e+00 1.350057e+08 2.197358e+04 6.144000e+03
2.566359e+00 1.350057e+08 1.098679e+04 1.228800e+04
9.682954e-01 1.076891e+09 8.763758e+04 1.228800e+04
1.144321e+00 1.076891e+09 4.381879e+04 2.457600e+04
1.957648e+00 1.076891e+09 2.190940e+04 4.915200e+04
1.585050e+00 1.076891e+09 1.095470e+04 9.830400e+04
1.179948e+00 8.602524e+09 8.750940e+04 9.830400e+04
9.228076e-01 8.602524e+09 5.833960e+04 1.474560e+05


==> data/large-scaling/large-scaling-4-4/speedup_3.tex <==
speedup n_dofs n_dofs_norm ranks
9.067068e-01 1.697459e+07 3.536374e+05 4.800000e+01
8.314281e-01 1.697459e+07 1.768187e+05 9.600000e+01
9.373072e-01 1.350057e+08 3.515773e+05 3.840000e+02
8.546325e-01 1.350057e+08 1.757887e+05 7.680000e+02
9.455274e-01 1.076891e+09 3.505503e+05 3.072000e+03
9.371503e-01 1.076891e+09 1.752752e+05 6.144000e+03
9.961867e-01 8.602524e+09 3.500376e+05 2.457600e+04
1.054285e+00 8.602524e+09 1.750188e+05 4.915200e+04
9.757204e-01 6.876982e+10 4.663752e+05 1.474560e+05


==> data/large-scaling/large-scaling-9-1/data_0004_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 6.458900e-02 1.518750e+01 1.000000e+01 1.128675e+04 7.290000e+02 4.000000e+00 9.000000e+00
2 6.642100e-02 7.593750e+00 1.000000e+01 5.487722e+03 7.290000e+02 4.000000e+00 9.000000e+00
4 6.745000e-02 3.796875e+00 1.000000e+01 2.702001e+03 7.290000e+02 4.000000e+00 9.000000e+00
8 6.767900e-02 1.898438e+00 1.000000e+01 1.346429e+03 7.290000e+02 4.000000e+00 9.000000e+00
16 7.932900e-02 9.492188e-01 1.000000e+01 5.743486e+02 7.290000e+02 4.000000e+00 9.000000e+00
32 7.303500e-02 4.746094e-01 1.000000e+01 3.119224e+02 7.290000e+02 4.000000e+00 9.000000e+00
64 9.161600e-02 2.373047e-01 1.000000e+01 1.243301e+02 7.290000e+02 4.000000e+00 9.000000e+00
128 9.706600e-02 1.186523e-01 1.000000e+01 5.867464e+01 7.290000e+02 4.000000e+00 9.000000e+00
256 8.722300e-02 5.932617e-02 1.000000e+01 3.264800e+01 7.290000e+02 4.000000e+00 9.000000e+00
512 8.520700e-02 2.966309e-02 1.000000e+01 1.671022e+01 7.290000e+02 4.000000e+00 9.000000e+00
1024 8.210300e-02 1.483154e-02 1.000000e+01 8.670987e+00 7.290000e+02 4.000000e+00 9.000000e+00
2048 6.788400e-02 7.415771e-03 1.000000e+01 5.243607e+00 7.290000e+02 4.000000e+00 9.000000e+00
3072 7.640800e-02 4.943848e-03 1.000000e+01 3.105757e+00 7.290000e+02 4.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-1/data_0004_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 8.872700e-03 1.518750e+01 1.000000e+01 8.216214e+04 7.290000e+02 4.000000e+00 9.000000e+00
2 1.047200e-02 7.593750e+00 1.000000e+01 3.480710e+04 7.290000e+02 4.000000e+00 9.000000e+00
4 1.123500e-02 3.796875e+00 1.000000e+01 1.622163e+04 7.290000e+02 4.000000e+00 9.000000e+00
8 1.185500e-02 1.898438e+00 1.000000e+01 7.686630e+03 7.290000e+02 4.000000e+00 9.000000e+00
16 1.375300e-02 9.492188e-01 1.000000e+01 3.312914e+03 7.290000e+02 4.000000e+00 9.000000e+00
32 1.416500e-02 4.746094e-01 1.000000e+01 1.608277e+03 7.290000e+02 4.000000e+00 9.000000e+00
64 1.925800e-02 2.373047e-01 1.000000e+01 5.914750e+02 7.290000e+02 4.000000e+00 9.000000e+00
128 1.855400e-02 1.186523e-01 1.000000e+01 3.069587e+02 7.290000e+02 4.000000e+00 9.000000e+00
256 1.651300e-02 5.932617e-02 1.000000e+01 1.724494e+02 7.290000e+02 4.000000e+00 9.000000e+00
512 1.652300e-02 2.966309e-02 1.000000e+01 8.617249e+01 7.290000e+02 4.000000e+00 9.000000e+00
1024 1.672300e-02 1.483154e-02 1.000000e+01 4.257095e+01 7.290000e+02 4.000000e+00 9.000000e+00
2048 2.404700e-02 7.415771e-03 1.000000e+01 1.480255e+01 7.290000e+02 4.000000e+00 9.000000e+00
3072 1.728800e-02 4.943848e-03 1.000000e+01 1.372656e+01 7.290000e+02 4.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-1/data_0005_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 1.040600e-01 1.023542e+02 1.000000e+01 4.721315e+04 4.913000e+03 5.000000e+00 9.000000e+00
2 1.145300e-01 5.117708e+01 1.000000e+01 2.144853e+04 4.913000e+03 5.000000e+00 9.000000e+00
4 1.190300e-01 2.558854e+01 1.000000e+01 1.031883e+04 4.913000e+03 5.000000e+00 9.000000e+00
8 1.316400e-01 1.279427e+01 1.000000e+01 4.665185e+03 4.913000e+03 5.000000e+00 9.000000e+00
16 1.260700e-01 6.397135e+00 1.000000e+01 2.435651e+03 4.913000e+03 5.000000e+00 9.000000e+00
32 1.303000e-01 3.198568e+00 1.000000e+01 1.178290e+03 4.913000e+03 5.000000e+00 9.000000e+00
64 1.394600e-01 1.599284e+00 1.000000e+01 5.504491e+02 4.913000e+03 5.000000e+00 9.000000e+00
128 1.604900e-01 7.996419e-01 1.000000e+01 2.391602e+02 4.913000e+03 5.000000e+00 9.000000e+00
256 1.420000e-01 3.998210e-01 1.000000e+01 1.351507e+02 4.913000e+03 5.000000e+00 9.000000e+00
512 1.400900e-01 1.999105e-01 1.000000e+01 6.849670e+01 4.913000e+03 5.000000e+00 9.000000e+00
1024 1.168800e-01 9.995524e-02 1.000000e+01 4.104938e+01 4.913000e+03 5.000000e+00 9.000000e+00
2048 1.398100e-01 4.997762e-02 1.000000e+01 1.715847e+01 4.913000e+03 5.000000e+00 9.000000e+00
3072 1.157100e-01 3.331841e-02 1.000000e+01 1.382148e+01 4.913000e+03 5.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-1/data_0005_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 2.369100e-02 1.023542e+02 1.000000e+01 2.073783e+05 4.913000e+03 5.000000e+00 9.000000e+00
2 2.020200e-02 5.117708e+01 1.000000e+01 1.215969e+05 4.913000e+03 5.000000e+00 9.000000e+00
4 1.839200e-02 2.558854e+01 1.000000e+01 6.678175e+04 4.913000e+03 5.000000e+00 9.000000e+00
8 1.811900e-02 1.279427e+01 1.000000e+01 3.389398e+04 4.913000e+03 5.000000e+00 9.000000e+00
16 2.133500e-02 6.397135e+00 1.000000e+01 1.439243e+04 4.913000e+03 5.000000e+00 9.000000e+00
32 2.805600e-02 3.198568e+00 1.000000e+01 5.472314e+03 4.913000e+03 5.000000e+00 9.000000e+00
64 4.259600e-02 1.599284e+00 1.000000e+01 1.802179e+03 4.913000e+03 5.000000e+00 9.000000e+00
128 3.955700e-02 7.996419e-01 1.000000e+01 9.703166e+02 4.913000e+03 5.000000e+00 9.000000e+00
256 3.258400e-02 3.998210e-01 1.000000e+01 5.889825e+02 4.913000e+03 5.000000e+00 9.000000e+00
512 2.543600e-02 1.999105e-01 1.000000e+01 3.772489e+02 4.913000e+03 5.000000e+00 9.000000e+00
1024 2.759500e-02 9.995524e-02 1.000000e+01 1.738667e+02 4.913000e+03 5.000000e+00 9.000000e+00
2048 2.356600e-02 4.997762e-02 1.000000e+01 1.017961e+02 4.913000e+03 5.000000e+00 9.000000e+00
3072 2.613100e-02 3.331841e-02 1.000000e+01 6.120255e+01 4.913000e+03 5.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-1/data_0006_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 2.126400e-01 7.486875e+02 1.000000e+01 1.690040e+05 3.593700e+04 6.000000e+00 9.000000e+00
2 1.884100e-01 3.743438e+02 1.000000e+01 9.536914e+04 3.593700e+04 6.000000e+00 9.000000e+00
4 1.702800e-01 1.871719e+02 1.000000e+01 5.276163e+04 3.593700e+04 6.000000e+00 9.000000e+00
8 1.691700e-01 9.358594e+01 1.000000e+01 2.655391e+04 3.593700e+04 6.000000e+00 9.000000e+00
16 1.908200e-01 4.679297e+01 1.000000e+01 1.177058e+04 3.593700e+04 6.000000e+00 9.000000e+00
32 2.008700e-01 2.339648e+01 1.000000e+01 5.590836e+03 3.593700e+04 6.000000e+00 9.000000e+00
64 2.037900e-01 1.169824e+01 1.000000e+01 2.755364e+03 3.593700e+04 6.000000e+00 9.000000e+00
128 2.075900e-01 5.849121e+00 1.000000e+01 1.352463e+03 3.593700e+04 6.000000e+00 9.000000e+00
256 1.862500e-01 2.924561e+00 1.000000e+01 7.537122e+02 3.593700e+04 6.000000e+00 9.000000e+00
512 1.767200e-01 1.462280e+00 1.000000e+01 3.971789e+02 3.593700e+04 6.000000e+00 9.000000e+00
1024 2.443100e-01 7.311401e-01 1.000000e+01 1.436483e+02 3.593700e+04 6.000000e+00 9.000000e+00
2048 1.496700e-01 3.655701e-01 1.000000e+01 1.172404e+02 3.593700e+04 6.000000e+00 9.000000e+00
3072 1.493500e-01 2.437134e-01 1.000000e+01 7.832770e+01 3.593700e+04 6.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-1/data_0006_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 1.183700e-01 7.486875e+02 1.000000e+01 3.035989e+05 3.593700e+04 6.000000e+00 9.000000e+00
2 6.952200e-02 3.743438e+02 1.000000e+01 2.584578e+05 3.593700e+04 6.000000e+00 9.000000e+00
4 4.521700e-02 1.871719e+02 1.000000e+01 1.986919e+05 3.593700e+04 6.000000e+00 9.000000e+00
8 3.392000e-02 9.358594e+01 1.000000e+01 1.324329e+05 3.593700e+04 6.000000e+00 9.000000e+00
16 3.219100e-02 4.679297e+01 1.000000e+01 6.977300e+04 3.593700e+04 6.000000e+00 9.000000e+00
32 5.101600e-02 2.339648e+01 1.000000e+01 2.201331e+04 3.593700e+04 6.000000e+00 9.000000e+00
64 5.385700e-02 1.169824e+01 1.000000e+01 1.042605e+04 3.593700e+04 6.000000e+00 9.000000e+00
128 8.941600e-02 5.849121e+00 1.000000e+01 3.139906e+03 3.593700e+04 6.000000e+00 9.000000e+00
256 8.916500e-02 2.924561e+00 1.000000e+01 1.574372e+03 3.593700e+04 6.000000e+00 9.000000e+00
512 7.839300e-02 1.462280e+00 1.000000e+01 8.953536e+02 3.593700e+04 6.000000e+00 9.000000e+00
1024 7.730000e-02 7.311401e-01 1.000000e+01 4.540068e+02 3.593700e+04 6.000000e+00 9.000000e+00
2048 6.224600e-02 3.655701e-01 1.000000e+01 2.819035e+02 3.593700e+04 6.000000e+00 9.000000e+00
3072 6.829200e-02 2.437134e-01 1.000000e+01 1.712974e+02 3.593700e+04 6.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-1/data_0007_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 7.783100e-01 5.721354e+03 1.000000e+01 3.528478e+05 2.746250e+05 7.000000e+00 9.000000e+00
2 5.031500e-01 2.860677e+03 1.000000e+01 2.729057e+05 2.746250e+05 7.000000e+00 9.000000e+00
4 3.537300e-01 1.430339e+03 1.000000e+01 1.940922e+05 2.746250e+05 7.000000e+00 9.000000e+00
8 2.827600e-01 7.151693e+02 1.000000e+01 1.214038e+05 2.746250e+05 7.000000e+00 9.000000e+00
16 2.680300e-01 3.575846e+02 1.000000e+01 6.403784e+04 2.746250e+05 7.000000e+00 9.000000e+00
32 2.613000e-01 1.787923e+02 1.000000e+01 3.284359e+04 2.746250e+05 7.000000e+00 9.000000e+00
64 2.645600e-01 8.939616e+01 1.000000e+01 1.621944e+04 2.746250e+05 7.000000e+00 9.000000e+00
128 3.159100e-01 4.469808e+01 1.000000e+01 6.791516e+03 2.746250e+05 7.000000e+00 9.000000e+00
256 3.834700e-01 2.234904e+01 1.000000e+01 2.797491e+03 2.746250e+05 7.000000e+00 9.000000e+00
512 2.902400e-01 1.117452e+01 1.000000e+01 1.848046e+03 2.746250e+05 7.000000e+00 9.000000e+00
1024 8.453600e-01 5.587260e+00 1.000000e+01 3.172477e+02 2.746250e+05 7.000000e+00 9.000000e+00
2048 2.749200e-01 2.793630e+00 1.000000e+01 4.877573e+02 2.746250e+05 7.000000e+00 9.000000e+00
3072 2.446600e-01 1.862420e+00 1.000000e+01 3.653894e+02 2.746250e+05 7.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-1/data_0007_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 8.289900e-01 5.721354e+03 1.000000e+01 3.312766e+05 2.746250e+05 7.000000e+00 9.000000e+00
2 4.342600e-01 2.860677e+03 1.000000e+01 3.161988e+05 2.746250e+05 7.000000e+00 9.000000e+00
4 2.191600e-01 1.430339e+03 1.000000e+01 3.132700e+05 2.746250e+05 7.000000e+00 9.000000e+00
8 1.269100e-01 7.151693e+02 1.000000e+01 2.704919e+05 2.746250e+05 7.000000e+00 9.000000e+00
16 8.622600e-02 3.575846e+02 1.000000e+01 1.990590e+05 2.746250e+05 7.000000e+00 9.000000e+00
32 6.879600e-02 1.787923e+02 1.000000e+01 1.247461e+05 2.746250e+05 7.000000e+00 9.000000e+00
64 7.077200e-02 8.939616e+01 1.000000e+01 6.063154e+04 2.746250e+05 7.000000e+00 9.000000e+00
128 1.224100e-01 4.469808e+01 1.000000e+01 1.752723e+04 2.746250e+05 7.000000e+00 9.000000e+00
256 1.022700e-01 2.234904e+01 1.000000e+01 1.048943e+04 2.746250e+05 7.000000e+00 9.000000e+00
512 1.112400e-01 1.117452e+01 1.000000e+01 4.821799e+03 2.746250e+05 7.000000e+00 9.000000e+00
1024 2.106800e-01 5.587260e+00 1.000000e+01 1.272966e+03 2.746250e+05 7.000000e+00 9.000000e+00
2048 1.515600e-01 2.793630e+00 1.000000e+01 8.847601e+02 2.746250e+05 7.000000e+00 9.000000e+00
3072 1.546700e-01 1.862420e+00 1.000000e+01 5.779799e+02 2.746250e+05 7.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-1/data_0008_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 5.816200e+00 4.472269e+04 1.000000e+01 3.690879e+05 2.146689e+06 8.000000e+00 9.000000e+00
2 3.042100e+00 2.236134e+04 1.000000e+01 3.528301e+05 2.146689e+06 8.000000e+00 9.000000e+00
4 1.631700e+00 1.118067e+04 1.000000e+01 3.289038e+05 2.146689e+06 8.000000e+00 9.000000e+00
8 8.658000e-01 5.590336e+03 1.000000e+01 3.099285e+05 2.146689e+06 8.000000e+00 9.000000e+00
16 6.237600e-01 2.795168e+03 1.000000e+01 2.150956e+05 2.146689e+06 8.000000e+00 9.000000e+00
32 4.995100e-01 1.397584e+03 1.000000e+01 1.342997e+05 2.146689e+06 8.000000e+00 9.000000e+00
64 3.974700e-01 6.987920e+02 1.000000e+01 8.438880e+04 2.146689e+06 8.000000e+00 9.000000e+00
128 4.143000e-01 3.493960e+02 1.000000e+01 4.048035e+04 2.146689e+06 8.000000e+00 9.000000e+00
256 3.698300e-01 1.746980e+02 1.000000e+01 2.267394e+04 2.146689e+06 8.000000e+00 9.000000e+00
512 3.842000e-01 8.734900e+01 1.000000e+01 1.091294e+04 2.146689e+06 8.000000e+00 9.000000e+00
1024 1.927600e+00 4.367450e+01 1.000000e+01 1.087558e+03 2.146689e+06 8.000000e+00 9.000000e+00
2048 5.467700e-01 2.183725e+01 1.000000e+01 1.917055e+03 2.146689e+06 8.000000e+00 9.000000e+00
3072 6.471100e-01 1.455817e+01 1.000000e+01 1.079866e+03 2.146689e+06 8.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-1/data_0008_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 7.613200e+00 4.472269e+04 1.000000e+01 2.819693e+05 2.146689e+06 8.000000e+00 9.000000e+00
2 3.864100e+00 2.236134e+04 1.000000e+01 2.777735e+05 2.146689e+06 8.000000e+00 9.000000e+00
4 1.959200e+00 1.118067e+04 1.000000e+01 2.739242e+05 2.146689e+06 8.000000e+00 9.000000e+00
8 8.460000e-01 5.590336e+03 1.000000e+01 3.171822e+05 2.146689e+06 8.000000e+00 9.000000e+00
16 4.335600e-01 2.795168e+03 1.000000e+01 3.094567e+05 2.146689e+06 8.000000e+00 9.000000e+00
32 2.471300e-01 1.397584e+03 1.000000e+01 2.714524e+05 2.146689e+06 8.000000e+00 9.000000e+00
64 1.632100e-01 6.987920e+02 1.000000e+01 2.055145e+05 2.146689e+06 8.000000e+00 9.000000e+00
128 1.391900e-01 3.493960e+02 1.000000e+01 1.204900e+05 2.146689e+06 8.000000e+00 9.000000e+00
256 1.272300e-01 1.746980e+02 1.000000e+01 6.590823e+04 2.146689e+06 8.000000e+00 9.000000e+00
512 1.783900e-01 8.734900e+01 1.000000e+01 2.350329e+04 2.146689e+06 8.000000e+00 9.000000e+00
1024 2.521800e-01 4.367450e+01 1.000000e+01 8.313014e+03 2.146689e+06 8.000000e+00 9.000000e+00
2048 1.389500e-01 2.183725e+01 1.000000e+01 7.543634e+03 2.146689e+06 8.000000e+00 9.000000e+00
3072 1.215200e-01 1.455817e+01 1.000000e+01 5.750428e+03 2.146689e+06 8.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-1/data_0009_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
2 2.397400e+01 1.768187e+05 1.000000e+01 3.540209e+05 1.697459e+07 9.000000e+00 9.000000e+00
4 1.456400e+01 8.840934e+04 1.000000e+01 2.913793e+05 1.697459e+07 9.000000e+00 9.000000e+00
8 6.117200e+00 4.420467e+04 1.000000e+01 3.468620e+05 1.697459e+07 9.000000e+00 9.000000e+00
16 3.998200e+00 2.210233e+04 1.000000e+01 2.653474e+05 1.697459e+07 9.000000e+00 9.000000e+00
32 2.110100e+00 1.105117e+04 1.000000e+01 2.513890e+05 1.697459e+07 9.000000e+00 9.000000e+00
64 1.187200e+00 5.525584e+03 1.000000e+01 2.234063e+05 1.697459e+07 9.000000e+00 9.000000e+00
128 9.917300e-01 2.762792e+03 1.000000e+01 1.337199e+05 1.697459e+07 9.000000e+00 9.000000e+00
256 8.944600e-01 1.381396e+03 1.000000e+01 7.413076e+04 1.697459e+07 9.000000e+00 9.000000e+00
512 1.010300e+00 6.906980e+02 1.000000e+01 3.281550e+04 1.697459e+07 9.000000e+00 9.000000e+00
1024 2.496700e+00 3.453490e+02 1.000000e+01 6.639464e+03 1.697459e+07 9.000000e+00 9.000000e+00
2048 5.972800e-01 1.726745e+02 1.000000e+01 1.387687e+04 1.697459e+07 9.000000e+00 9.000000e+00
3072 6.955700e-01 1.151163e+02 1.000000e+01 7.943965e+03 1.697459e+07 9.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-1/data_0009_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
8 7.765600e+00 4.420467e+04 1.000000e+01 2.732338e+05 1.697459e+07 9.000000e+00 9.000000e+00
16 4.240600e+00 2.210233e+04 1.000000e+01 2.501797e+05 1.697459e+07 9.000000e+00 9.000000e+00
32 2.024800e+00 1.105117e+04 1.000000e+01 2.619795e+05 1.697459e+07 9.000000e+00 9.000000e+00
64 9.252300e-01 5.525584e+03 1.000000e+01 2.866617e+05 1.697459e+07 9.000000e+00 9.000000e+00
128 5.575500e-01 2.762792e+03 1.000000e+01 2.378513e+05 1.697459e+07 9.000000e+00 9.000000e+00
256 4.600400e-01 1.381396e+03 1.000000e+01 1.441331e+05 1.697459e+07 9.000000e+00 9.000000e+00
512 3.541300e-01 6.906980e+02 1.000000e+01 9.361958e+04 1.697459e+07 9.000000e+00 9.000000e+00
1024 3.821100e-01 3.453490e+02 1.000000e+01 4.338214e+04 1.697459e+07 9.000000e+00 9.000000e+00
2048 1.805300e-01 1.726745e+02 1.000000e+01 4.591135e+04 1.697459e+07 9.000000e+00 9.000000e+00
3072 1.463100e-01 1.151163e+02 1.000000e+01 3.776627e+04 1.697459e+07 9.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-1/data_0010_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
16 2.907300e+01 1.757887e+05 1.000000e+01 2.902300e+05 1.350057e+08 1.000000e+01 9.000000e+00
32 1.489700e+01 8.789433e+04 1.000000e+01 2.832066e+05 1.350057e+08 1.000000e+01 9.000000e+00
64 6.986600e+00 4.394717e+04 1.000000e+01 3.019300e+05 1.350057e+08 1.000000e+01 9.000000e+00
128 4.350500e+00 2.197358e+04 1.000000e+01 2.424393e+05 1.350057e+08 1.000000e+01 9.000000e+00
256 3.115400e+00 1.098679e+04 1.000000e+01 1.692771e+05 1.350057e+08 1.000000e+01 9.000000e+00
512 2.446000e+00 5.493396e+03 1.000000e+01 1.078017e+05 1.350057e+08 1.000000e+01 9.000000e+00
1024 3.777000e+00 2.746698e+03 1.000000e+01 3.490641e+04 1.350057e+08 1.000000e+01 9.000000e+00
2048 9.850800e-01 1.373349e+03 1.000000e+01 6.691918e+04 1.350057e+08 1.000000e+01 9.000000e+00
3072 9.864800e-01 9.155660e+02 1.000000e+01 4.454948e+04 1.350057e+08 1.000000e+01 9.000000e+00


==> data/large-scaling/large-scaling-9-1/data_0010_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
64 7.879400e+00 4.394717e+04 1.000000e+01 2.677189e+05 1.350057e+08 1.000000e+01 9.000000e+00
128 4.290800e+00 2.197358e+04 1.000000e+01 2.458124e+05 1.350057e+08 1.000000e+01 9.000000e+00
256 2.543300e+00 1.098679e+04 1.000000e+01 2.073550e+05 1.350057e+08 1.000000e+01 9.000000e+00
512 1.342900e+00 5.493396e+03 1.000000e+01 1.963534e+05 1.350057e+08 1.000000e+01 9.000000e+00
1024 1.123100e+00 2.746698e+03 1.000000e+01 1.173907e+05 1.350057e+08 1.000000e+01 9.000000e+00
2048 4.692200e-01 1.373349e+03 1.000000e+01 1.404901e+05 1.350057e+08 1.000000e+01 9.000000e+00
3072 3.623900e-01 9.155660e+02 1.000000e+01 1.212704e+05 1.350057e+08 1.000000e+01 9.000000e+00


==> data/large-scaling/large-scaling-9-1/data_0011_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
128 3.001800e+01 1.752752e+05 1.000000e+01 2.802721e+05 1.076891e+09 1.100000e+01 9.000000e+00
256 1.910600e+01 8.763758e+04 1.000000e+01 2.201719e+05 1.076891e+09 1.100000e+01 9.000000e+00
512 1.084900e+01 4.381879e+04 1.000000e+01 1.938706e+05 1.076891e+09 1.100000e+01 9.000000e+00
1024 9.563900e+00 2.190940e+04 1.000000e+01 1.099605e+05 1.076891e+09 1.100000e+01 9.000000e+00
2048 3.395400e+00 1.095470e+04 1.000000e+01 1.548641e+05 1.076891e+09 1.100000e+01 9.000000e+00
3072 2.683700e+00 7.303132e+03 1.000000e+01 1.306220e+05 1.076891e+09 1.100000e+01 9.000000e+00


==> data/large-scaling/large-scaling-9-1/data_0011_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
512 1.049300e+01 4.381879e+04 1.000000e+01 2.004481e+05 1.076891e+09 1.100000e+01 9.000000e+00
1024 6.435200e+00 2.190940e+04 1.000000e+01 1.634216e+05 1.076891e+09 1.100000e+01 9.000000e+00
2048 3.163800e+00 1.095470e+04 1.000000e+01 1.662006e+05 1.076891e+09 1.100000e+01 9.000000e+00
3072 2.049500e+00 7.303132e+03 1.000000e+01 1.710419e+05 1.076891e+09 1.100000e+01 9.000000e+00


==> data/large-scaling/large-scaling-9-1/data_0012_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1024 4.864200e+01 1.750188e+05 1.000000e+01 1.727088e+05 8.602524e+09 1.200000e+01 9.000000e+00
2048 2.259100e+01 8.750940e+04 1.000000e+01 1.859347e+05 8.602524e+09 1.200000e+01 9.000000e+00
3072 1.590100e+01 5.833960e+04 1.000000e+01 1.761085e+05 8.602524e+09 1.200000e+01 9.000000e+00


==> data/large-scaling/large-scaling-9-1/data_0012_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
3072 1.670700e+01 5.833960e+04 1.000000e+01 1.676124e+05 8.602524e+09 1.200000e+01 9.000000e+00


==> data/large-scaling/large-scaling-9-1/speedup_0.tex <==
speedup n_dofs n_dofs_norm ranks
7.279520e+00 7.290000e+02 1.518750e+01 4.800000e+01
4.392385e+00 4.913000e+03 1.023542e+02 4.800000e+01
1.796401e+00 3.593700e+04 7.486875e+02 4.800000e+01
6.342723e+00 7.290000e+02 7.593750e+00 9.600000e+01
5.669241e+00 4.913000e+03 5.117708e+01 9.600000e+01
2.710077e+00 3.593700e+04 3.743438e+02 9.600000e+01
6.003560e+00 7.290000e+02 3.796875e+00 1.920000e+02
6.471836e+00 4.913000e+03 2.558854e+01 1.920000e+02
3.765840e+00 3.593700e+04 1.871719e+02 1.920000e+02
5.708899e+00 7.290000e+02 1.898438e+00 3.840000e+02
7.265302e+00 4.913000e+03 1.279427e+01 3.840000e+02
4.987323e+00 3.593700e+04 9.358594e+01 3.840000e+02
2.228036e+00 2.746250e+05 7.151693e+02 3.840000e+02
5.768123e+00 7.290000e+02 9.492188e-01 7.680000e+02
5.909070e+00 4.913000e+03 6.397135e+00 7.680000e+02
5.927744e+00 3.593700e+04 4.679297e+01 7.680000e+02
3.108459e+00 2.746250e+05 3.575846e+02 7.680000e+02
5.156018e+00 7.290000e+02 4.746094e-01 1.536000e+03
4.644283e+00 4.913000e+03 3.198568e+00 1.536000e+03
3.937392e+00 3.593700e+04 2.339648e+01 1.536000e+03
3.798186e+00 2.746250e+05 1.787923e+02 1.536000e+03
4.757296e+00 7.290000e+02 2.373047e-01 3.072000e+03
3.274016e+00 4.913000e+03 1.599284e+00 3.072000e+03
3.783909e+00 3.593700e+04 1.169824e+01 3.072000e+03
3.738202e+00 2.746250e+05 8.939616e+01 3.072000e+03
2.435329e+00 2.146689e+06 6.987920e+02 3.072000e+03
5.231540e+00 7.290000e+02 1.186523e-01 6.144000e+03
4.057183e+00 4.913000e+03 7.996419e-01 6.144000e+03
2.321620e+00 3.593700e+04 5.849121e+00 6.144000e+03
2.580753e+00 2.746250e+05 4.469808e+01 6.144000e+03
2.976507e+00 2.146689e+06 3.493960e+02 6.144000e+03
5.282081e+00 7.290000e+02 5.932617e-02 1.228800e+04
4.357967e+00 4.913000e+03 3.998210e-01 1.228800e+04
2.088824e+00 3.593700e+04 2.924561e+00 1.228800e+04
3.749584e+00 2.746250e+05 2.234904e+01 1.228800e+04
2.906783e+00 2.146689e+06 1.746980e+02 1.228800e+04
5.156872e+00 7.290000e+02 2.966309e-02 2.457600e+04
5.507548e+00 4.913000e+03 1.999105e-01 2.457600e+04
2.254283e+00 3.593700e+04 1.462280e+00 2.457600e+04
2.609133e+00 2.746250e+05 1.117452e+01 2.457600e+04
2.153708e+00 2.146689e+06 8.734900e+01 2.457600e+04
2.852907e+00 1.697459e+07 6.906980e+02 2.457600e+04
4.909586e+00 7.290000e+02 1.483154e-02 4.915200e+04
4.235550e+00 4.913000e+03 9.995524e-02 4.915200e+04
3.160543e+00 3.593700e+04 7.311401e-01 4.915200e+04
4.012531e+00 2.746250e+05 5.587260e+00 4.915200e+04
7.643747e+00 2.146689e+06 4.367450e+01 4.915200e+04
6.533982e+00 1.697459e+07 3.453490e+02 4.915200e+04
2.822972e+00 7.290000e+02 7.415771e-03 9.830400e+04
5.932700e+00 4.913000e+03 4.997762e-02 9.830400e+04
2.404492e+00 3.593700e+04 3.655701e-01 9.830400e+04
1.813935e+00 2.746250e+05 2.793630e+00 9.830400e+04
3.935013e+00 2.146689e+06 2.183725e+01 9.830400e+04
3.308481e+00 1.697459e+07 1.726745e+02 9.830400e+04
4.419713e+00 7.290000e+02 4.943848e-03 1.474560e+05
4.428074e+00 4.913000e+03 3.331841e-02 1.474560e+05
2.186933e+00 3.593700e+04 2.437134e-01 1.474560e+05
1.581819e+00 2.746250e+05 1.862420e+00 1.474560e+05
5.325132e+00 2.146689e+06 1.455817e+01 1.474560e+05
4.754084e+00 1.697459e+07 1.151163e+02 1.474560e+05
2.722150e+00 1.350057e+08 9.155660e+02 1.474560e+05


==> data/large-scaling/large-scaling-9-1/speedup_1.tex <==
speedup n_dofs n_dofs_norm ranks
9.388654e-01 2.746250e+05 5.721354e+03 4.800000e+01
1.158638e+00 2.746250e+05 2.860677e+03 9.600000e+01
1.614026e+00 2.746250e+05 1.430339e+03 1.920000e+02
1.023404e+00 2.146689e+06 5.590336e+03 3.840000e+02
1.438694e+00 2.146689e+06 2.795168e+03 7.680000e+02
2.021244e+00 2.146689e+06 1.397584e+03 1.536000e+03
1.283140e+00 1.697459e+07 5.525584e+03 3.072000e+03
1.778728e+00 1.697459e+07 2.762792e+03 6.144000e+03
1.944309e+00 1.697459e+07 1.381396e+03 1.228800e+04
1.821431e+00 1.350057e+08 5.493396e+03 2.457600e+04
3.363013e+00 1.350057e+08 2.746698e+03 4.915200e+04
2.099399e+00 1.350057e+08 1.373349e+03 9.830400e+04
1.309441e+00 1.076891e+09 7.303132e+03 1.474560e+05


==> data/large-scaling/large-scaling-9-1/speedup_2.tex <==
speedup n_dofs n_dofs_norm ranks
7.639626e-01 2.146689e+06 4.472269e+04 4.800000e+01
7.872726e-01 2.146689e+06 2.236134e+04 9.600000e+01
8.328399e-01 2.146689e+06 1.118067e+04 1.920000e+02
7.877305e-01 1.697459e+07 4.420467e+04 3.840000e+02
9.428383e-01 1.697459e+07 2.210233e+04 7.680000e+02
1.042128e+00 1.697459e+07 1.105117e+04 1.536000e+03
8.866919e-01 1.350057e+08 4.394717e+04 3.072000e+03
1.013913e+00 1.350057e+08 2.197358e+04 6.144000e+03
1.224944e+00 1.350057e+08 1.098679e+04 1.228800e+04
1.033927e+00 1.076891e+09 4.381879e+04 2.457600e+04
1.486185e+00 1.076891e+09 2.190940e+04 4.915200e+04
1.073203e+00 1.076891e+09 1.095470e+04 9.830400e+04
9.517567e-01 8.602524e+09 5.833960e+04 1.474560e+05


==> data/large-scaling/large-scaling-9-1/speedup_3.tex <==
speedup n_dofs n_dofs_norm ranks


==> data/large-scaling/large-scaling-9-4/data_0004_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 1.637700e-01 7.486875e+02 1.000000e+01 2.194358e+05 3.593700e+04 4.000000e+00 9.000000e+00
2 1.445000e-01 3.743438e+02 1.000000e+01 1.243495e+05 3.593700e+04 4.000000e+00 9.000000e+00
4 1.395800e-01 1.871719e+02 1.000000e+01 6.436631e+04 3.593700e+04 4.000000e+00 9.000000e+00
8 1.384000e-01 9.358594e+01 1.000000e+01 3.245755e+04 3.593700e+04 4.000000e+00 9.000000e+00
16 1.374700e-01 4.679297e+01 1.000000e+01 1.633856e+04 3.593700e+04 4.000000e+00 9.000000e+00
32 1.588100e-01 2.339648e+01 1.000000e+01 7.071540e+03 3.593700e+04 4.000000e+00 9.000000e+00
64 1.701600e-01 1.169824e+01 1.000000e+01 3.299927e+03 3.593700e+04 4.000000e+00 9.000000e+00
128 1.451100e-01 5.849121e+00 1.000000e+01 1.934793e+03 3.593700e+04 4.000000e+00 9.000000e+00
256 1.527000e-01 2.924561e+00 1.000000e+01 9.193118e+02 3.593700e+04 4.000000e+00 9.000000e+00
512 1.566900e-01 1.462280e+00 1.000000e+01 4.479511e+02 3.593700e+04 4.000000e+00 9.000000e+00
1024 1.647300e-01 7.311401e-01 1.000000e+01 2.130439e+02 3.593700e+04 4.000000e+00 9.000000e+00
2048 1.479300e-01 3.655701e-01 1.000000e+01 1.186194e+02 3.593700e+04 4.000000e+00 9.000000e+00
3072 1.566000e-01 2.437134e-01 1.000000e+01 7.470142e+01 3.593700e+04 4.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-4/data_0004_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 4.123300e-02 7.486875e+02 1.000000e+01 8.715592e+05 3.593700e+04 4.000000e+00 9.000000e+00
2 3.220500e-02 3.743438e+02 1.000000e+01 5.579413e+05 3.593700e+04 4.000000e+00 9.000000e+00
4 2.853600e-02 1.871719e+02 1.000000e+01 3.148392e+05 3.593700e+04 4.000000e+00 9.000000e+00
8 2.524900e-02 9.358594e+01 1.000000e+01 1.779130e+05 3.593700e+04 4.000000e+00 9.000000e+00
16 2.267200e-02 4.679297e+01 1.000000e+01 9.906768e+04 3.593700e+04 4.000000e+00 9.000000e+00
32 2.529000e-02 2.339648e+01 1.000000e+01 4.440614e+04 3.593700e+04 4.000000e+00 9.000000e+00
64 3.263800e-02 1.169824e+01 1.000000e+01 1.720435e+04 3.593700e+04 4.000000e+00 9.000000e+00
128 2.329900e-02 5.849121e+00 1.000000e+01 1.205021e+04 3.593700e+04 4.000000e+00 9.000000e+00
256 2.576800e-02 2.924561e+00 1.000000e+01 5.447800e+03 3.593700e+04 4.000000e+00 9.000000e+00
512 2.858200e-02 1.462280e+00 1.000000e+01 2.455722e+03 3.593700e+04 4.000000e+00 9.000000e+00
1024 2.723000e-02 7.311401e-01 1.000000e+01 1.288826e+03 3.593700e+04 4.000000e+00 9.000000e+00
2048 2.804600e-02 3.655701e-01 1.000000e+01 6.256637e+02 3.593700e+04 4.000000e+00 9.000000e+00
3072 2.859700e-02 2.437134e-01 1.000000e+01 4.090724e+02 3.593700e+04 4.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-4/data_0005_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 3.791100e-01 5.721354e+03 1.000000e+01 7.243940e+05 2.746250e+05 5.000000e+00 9.000000e+00
2 3.167100e-01 2.860677e+03 1.000000e+01 4.335591e+05 2.746250e+05 5.000000e+00 9.000000e+00
4 2.912000e-01 1.430339e+03 1.000000e+01 2.357701e+05 2.746250e+05 5.000000e+00 9.000000e+00
8 2.856700e-01 7.151693e+02 1.000000e+01 1.201671e+05 2.746250e+05 5.000000e+00 9.000000e+00
16 2.583600e-01 3.575846e+02 1.000000e+01 6.643467e+04 2.746250e+05 5.000000e+00 9.000000e+00
32 2.799200e-01 1.787923e+02 1.000000e+01 3.065887e+04 2.746250e+05 5.000000e+00 9.000000e+00
64 3.088900e-01 8.939616e+01 1.000000e+01 1.389173e+04 2.746250e+05 5.000000e+00 9.000000e+00
128 2.707500e-01 4.469808e+01 1.000000e+01 7.924313e+03 2.746250e+05 5.000000e+00 9.000000e+00
256 2.811800e-01 2.234904e+01 1.000000e+01 3.815186e+03 2.746250e+05 5.000000e+00 9.000000e+00
512 2.775100e-01 1.117452e+01 1.000000e+01 1.932820e+03 2.746250e+05 5.000000e+00 9.000000e+00
1024 2.588100e-01 5.587260e+00 1.000000e+01 1.036237e+03 2.746250e+05 5.000000e+00 9.000000e+00
2048 2.538000e-01 2.793630e+00 1.000000e+01 5.283461e+02 2.746250e+05 5.000000e+00 9.000000e+00
3072 2.611100e-01 1.862420e+00 1.000000e+01 3.423697e+02 2.746250e+05 5.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-4/data_0005_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 3.280100e-01 5.721354e+03 1.000000e+01 8.372458e+05 2.746250e+05 5.000000e+00 9.000000e+00
2 1.715600e-01 2.860677e+03 1.000000e+01 8.003760e+05 2.746250e+05 5.000000e+00 9.000000e+00
4 9.355800e-02 1.430339e+03 1.000000e+01 7.338362e+05 2.746250e+05 5.000000e+00 9.000000e+00
8 6.148500e-02 7.151693e+02 1.000000e+01 5.583171e+05 2.746250e+05 5.000000e+00 9.000000e+00
16 4.883900e-02 3.575846e+02 1.000000e+01 3.514417e+05 2.746250e+05 5.000000e+00 9.000000e+00
32 5.017500e-02 1.787923e+02 1.000000e+01 1.710420e+05 2.746250e+05 5.000000e+00 9.000000e+00
64 4.985200e-02 8.939616e+01 1.000000e+01 8.607509e+04 2.746250e+05 5.000000e+00 9.000000e+00
128 4.022600e-02 4.469808e+01 1.000000e+01 5.333634e+04 2.746250e+05 5.000000e+00 9.000000e+00
256 4.160600e-02 2.234904e+01 1.000000e+01 2.578363e+04 2.746250e+05 5.000000e+00 9.000000e+00
512 3.959700e-02 1.117452e+01 1.000000e+01 1.354590e+04 2.746250e+05 5.000000e+00 9.000000e+00
1024 3.940800e-02 5.587260e+00 1.000000e+01 6.805432e+03 2.746250e+05 5.000000e+00 9.000000e+00
2048 3.752400e-02 2.793630e+00 1.000000e+01 3.573559e+03 2.746250e+05 5.000000e+00 9.000000e+00
3072 3.932600e-02 1.862420e+00 1.000000e+01 2.273208e+03 2.746250e+05 5.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-4/data_0006_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 2.605300e+00 4.472269e+04 1.000000e+01 8.239700e+05 2.146689e+06 6.000000e+00 9.000000e+00
2 1.311000e+00 2.236134e+04 1.000000e+01 8.187220e+05 2.146689e+06 6.000000e+00 9.000000e+00
4 7.435100e-01 1.118067e+04 1.000000e+01 7.218091e+05 2.146689e+06 6.000000e+00 9.000000e+00
8 5.453900e-01 5.590336e+03 1.000000e+01 4.920078e+05 2.146689e+06 6.000000e+00 9.000000e+00
16 4.785800e-01 2.795168e+03 1.000000e+01 2.803462e+05 2.146689e+06 6.000000e+00 9.000000e+00
32 4.300400e-01 1.397584e+03 1.000000e+01 1.559949e+05 2.146689e+06 6.000000e+00 9.000000e+00
64 4.612600e-01 6.987920e+02 1.000000e+01 7.271824e+04 2.146689e+06 6.000000e+00 9.000000e+00
128 3.769500e-01 3.493960e+02 1.000000e+01 4.449133e+04 2.146689e+06 6.000000e+00 9.000000e+00
256 3.898500e-01 1.746980e+02 1.000000e+01 2.150956e+04 2.146689e+06 6.000000e+00 9.000000e+00
512 4.622500e-01 8.734900e+01 1.000000e+01 9.070313e+03 2.146689e+06 6.000000e+00 9.000000e+00
1024 4.814400e-01 4.367450e+01 1.000000e+01 4.354387e+03 2.146689e+06 6.000000e+00 9.000000e+00
2048 3.592200e-01 2.183725e+01 1.000000e+01 2.917956e+03 2.146689e+06 6.000000e+00 9.000000e+00
3072 3.728100e-01 1.455817e+01 1.000000e+01 1.874392e+03 2.146689e+06 6.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-4/data_0006_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 4.519700e+00 4.472269e+04 1.000000e+01 4.749627e+05 2.146689e+06 6.000000e+00 9.000000e+00
2 2.201400e+00 2.236134e+04 1.000000e+01 4.875736e+05 2.146689e+06 6.000000e+00 9.000000e+00
4 7.938900e-01 1.118067e+04 1.000000e+01 6.760033e+05 2.146689e+06 6.000000e+00 9.000000e+00
8 3.466100e-01 5.590336e+03 1.000000e+01 7.741731e+05 2.146689e+06 6.000000e+00 9.000000e+00
16 1.772900e-01 2.795168e+03 1.000000e+01 7.567717e+05 2.146689e+06 6.000000e+00 9.000000e+00
32 1.170100e-01 1.397584e+03 1.000000e+01 5.733188e+05 2.146689e+06 6.000000e+00 9.000000e+00
64 9.792300e-02 6.987920e+02 1.000000e+01 3.425346e+05 2.146689e+06 6.000000e+00 9.000000e+00
128 6.967800e-02 3.493960e+02 1.000000e+01 2.406930e+05 2.146689e+06 6.000000e+00 9.000000e+00
256 1.301500e-01 1.746980e+02 1.000000e+01 6.442953e+04 2.146689e+06 6.000000e+00 9.000000e+00
512 6.034500e-02 8.734900e+01 1.000000e+01 6.947969e+04 2.146689e+06 6.000000e+00 9.000000e+00
1024 7.879700e-02 4.367450e+01 1.000000e+01 2.660477e+04 2.146689e+06 6.000000e+00 9.000000e+00
2048 5.300000e-02 2.183725e+01 1.000000e+01 1.977713e+04 2.146689e+06 6.000000e+00 9.000000e+00
3072 5.440600e-02 1.455817e+01 1.000000e+01 1.284402e+04 2.146689e+06 6.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-4/data_0007_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1 2.637200e+01 3.536374e+05 1.000000e+01 6.436597e+05 1.697459e+07 7.000000e+00 9.000000e+00
2 1.367800e+01 1.768187e+05 1.000000e+01 6.205071e+05 1.697459e+07 7.000000e+00 9.000000e+00
4 6.533800e+00 8.840934e+04 1.000000e+01 6.494916e+05 1.697459e+07 7.000000e+00 9.000000e+00
8 2.813600e+00 4.420467e+04 1.000000e+01 7.541314e+05 1.697459e+07 7.000000e+00 9.000000e+00
16 1.484300e+00 2.210233e+04 1.000000e+01 7.147558e+05 1.697459e+07 7.000000e+00 9.000000e+00
32 8.924500e-01 1.105117e+04 1.000000e+01 5.943818e+05 1.697459e+07 7.000000e+00 9.000000e+00
64 7.528500e-01 5.525584e+03 1.000000e+01 3.522986e+05 1.697459e+07 7.000000e+00 9.000000e+00
128 7.365200e-01 2.762792e+03 1.000000e+01 1.800549e+05 1.697459e+07 7.000000e+00 9.000000e+00
256 5.827400e-01 1.381396e+03 1.000000e+01 1.137849e+05 1.697459e+07 7.000000e+00 9.000000e+00
512 7.802400e-01 6.906980e+02 1.000000e+01 4.249142e+04 1.697459e+07 7.000000e+00 9.000000e+00
1024 1.278400e+00 3.453490e+02 1.000000e+01 1.296680e+04 1.697459e+07 7.000000e+00 9.000000e+00
2048 4.852200e-01 1.726745e+02 1.000000e+01 1.708169e+04 1.697459e+07 7.000000e+00 9.000000e+00
3072 4.833300e-01 1.151163e+02 1.000000e+01 1.143232e+04 1.697459e+07 7.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-4/data_0007_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
2 1.900800e+01 1.768187e+05 1.000000e+01 4.465118e+05 1.697459e+07 7.000000e+00 9.000000e+00
4 9.136300e+00 8.840934e+04 1.000000e+01 4.644821e+05 1.697459e+07 7.000000e+00 9.000000e+00
8 4.409900e+00 4.420467e+04 1.000000e+01 4.811502e+05 1.697459e+07 7.000000e+00 9.000000e+00
16 2.168000e+00 2.210233e+04 1.000000e+01 4.893506e+05 1.697459e+07 7.000000e+00 9.000000e+00
32 8.573600e-01 1.105117e+04 1.000000e+01 6.187086e+05 1.697459e+07 7.000000e+00 9.000000e+00
64 4.060600e-01 5.525584e+03 1.000000e+01 6.531744e+05 1.697459e+07 7.000000e+00 9.000000e+00
128 2.012400e-01 2.762792e+03 1.000000e+01 6.589843e+05 1.697459e+07 7.000000e+00 9.000000e+00
256 1.974100e-01 1.381396e+03 1.000000e+01 3.358847e+05 1.697459e+07 7.000000e+00 9.000000e+00
512 1.760100e-01 6.906980e+02 1.000000e+01 1.883615e+05 1.697459e+07 7.000000e+00 9.000000e+00
1024 2.111300e-01 3.453490e+02 1.000000e+01 7.851443e+04 1.697459e+07 7.000000e+00 9.000000e+00
2048 9.683600e-02 1.726745e+02 1.000000e+01 8.559188e+04 1.697459e+07 7.000000e+00 9.000000e+00
3072 9.380000e-02 1.151163e+02 1.000000e+01 5.890814e+04 1.697459e+07 7.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-4/data_0008_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
8 2.833200e+01 3.515773e+05 1.000000e+01 5.956414e+05 1.350057e+08 8.000000e+00 9.000000e+00
16 1.354600e+01 1.757887e+05 1.000000e+01 6.229039e+05 1.350057e+08 8.000000e+00 9.000000e+00
32 6.359700e+00 8.789433e+04 1.000000e+01 6.633848e+05 1.350057e+08 8.000000e+00 9.000000e+00
64 3.536300e+00 4.394717e+04 1.000000e+01 5.965173e+05 1.350057e+08 8.000000e+00 9.000000e+00
128 2.125200e+00 2.197358e+04 1.000000e+01 4.962978e+05 1.350057e+08 8.000000e+00 9.000000e+00
256 1.494000e+00 1.098679e+04 1.000000e+01 3.529893e+05 1.350057e+08 8.000000e+00 9.000000e+00
512 1.503400e+00 5.493396e+03 1.000000e+01 1.753911e+05 1.350057e+08 8.000000e+00 9.000000e+00
1024 2.733900e+00 2.746698e+03 1.000000e+01 4.822470e+04 1.350057e+08 8.000000e+00 9.000000e+00
2048 8.492100e-01 1.373349e+03 1.000000e+01 7.762597e+04 1.350057e+08 8.000000e+00 9.000000e+00
3072 8.557100e-01 9.155660e+02 1.000000e+01 5.135755e+04 1.350057e+08 8.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-4/data_0008_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
16 1.789800e+01 1.757887e+05 1.000000e+01 4.714413e+05 1.350057e+08 8.000000e+00 9.000000e+00
32 9.008500e+00 8.789433e+04 1.000000e+01 4.683275e+05 1.350057e+08 8.000000e+00 9.000000e+00
64 4.571700e+00 4.394717e+04 1.000000e+01 4.614179e+05 1.350057e+08 8.000000e+00 9.000000e+00
128 2.441200e+00 2.197358e+04 1.000000e+01 4.320547e+05 1.350057e+08 8.000000e+00 9.000000e+00
256 1.048100e+00 1.098679e+04 1.000000e+01 5.031638e+05 1.350057e+08 8.000000e+00 9.000000e+00
512 6.455800e-01 5.493396e+03 1.000000e+01 4.084436e+05 1.350057e+08 8.000000e+00 9.000000e+00
1024 5.528100e-01 2.746698e+03 1.000000e+01 2.384933e+05 1.350057e+08 8.000000e+00 9.000000e+00
2048 1.856200e-01 1.373349e+03 1.000000e+01 3.551382e+05 1.350057e+08 8.000000e+00 9.000000e+00
3072 1.676200e-01 9.155660e+02 1.000000e+01 2.621833e+05 1.350057e+08 8.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-4/data_0009_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
64 2.908500e+01 3.505503e+05 1.000000e+01 5.785256e+05 1.076891e+09 9.000000e+00 9.000000e+00
128 1.573600e+01 1.752752e+05 1.000000e+01 5.346472e+05 1.076891e+09 9.000000e+00 9.000000e+00
256 8.144300e+00 8.763758e+04 1.000000e+01 5.165090e+05 1.076891e+09 9.000000e+00 9.000000e+00
512 5.305500e+00 4.381879e+04 1.000000e+01 3.964380e+05 1.076891e+09 9.000000e+00 9.000000e+00
1024 5.295100e+00 2.190940e+04 1.000000e+01 1.986083e+05 1.076891e+09 9.000000e+00 9.000000e+00
2048 1.498600e+00 1.095470e+04 1.000000e+01 3.508778e+05 1.076891e+09 9.000000e+00 9.000000e+00
3072 1.413900e+00 7.303132e+03 1.000000e+01 2.479315e+05 1.076891e+09 9.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-4/data_0009_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
128 1.914300e+01 1.752752e+05 1.000000e+01 4.394927e+05 1.076891e+09 9.000000e+00 9.000000e+00
256 9.643600e+00 8.763758e+04 1.000000e+01 4.362068e+05 1.076891e+09 9.000000e+00 9.000000e+00
512 5.528000e+00 4.381879e+04 1.000000e+01 3.804815e+05 1.076891e+09 9.000000e+00 9.000000e+00
1024 2.968500e+00 2.190940e+04 1.000000e+01 3.542702e+05 1.076891e+09 9.000000e+00 9.000000e+00
2048 1.066700e+00 1.095470e+04 1.000000e+01 4.929460e+05 1.076891e+09 9.000000e+00 9.000000e+00
3072 7.851200e-01 7.303132e+03 1.000000e+01 4.464927e+05 1.076891e+09 9.000000e+00 9.000000e+00


==> data/large-scaling/large-scaling-9-4/data_0010_0.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
512 3.518400e+01 3.500376e+05 1.000000e+01 4.775410e+05 8.602524e+09 1.000000e+01 9.000000e+00
1024 2.138000e+01 1.750188e+05 1.000000e+01 3.929327e+05 8.602524e+09 1.000000e+01 9.000000e+00
2048 8.048600e+00 8.750940e+04 1.000000e+01 5.218859e+05 8.602524e+09 1.000000e+01 9.000000e+00
3072 5.998700e+00 5.833960e+04 1.000000e+01 4.668179e+05 8.602524e+09 1.000000e+01 9.000000e+00


==> data/large-scaling/large-scaling-9-4/data_0010_1.tex <==
n_ranks t_per_timestep n_dofs_per_proc n_timesteps throughput_per_node n_dofs n_levels n_stages
1024 2.069400e+01 1.750188e+05 1.000000e+01 4.059583e+05 8.602524e+09 1.000000e+01 9.000000e+00
2048 1.001600e+01 8.750940e+04 1.000000e+01 4.193741e+05 8.602524e+09 1.000000e+01 9.000000e+00
3072 6.909100e+00 5.833960e+04 1.000000e+01 4.053061e+05 8.602524e+09 1.000000e+01 9.000000e+00


==> data/large-scaling/large-scaling-9-4/speedup_0.tex <==
speedup n_dofs n_dofs_norm ranks
3.971819e+00 3.593700e+04 7.486875e+02 4.800000e+01
4.486881e+00 3.593700e+04 3.743438e+02 9.600000e+01
4.891365e+00 3.593700e+04 1.871719e+02 1.920000e+02
5.481405e+00 3.593700e+04 9.358594e+01 3.840000e+02
4.646174e+00 2.746250e+05 7.151693e+02 3.840000e+02
6.063426e+00 3.593700e+04 4.679297e+01 7.680000e+02
5.290035e+00 2.746250e+05 3.575846e+02 7.680000e+02
6.279557e+00 3.593700e+04 2.339648e+01 1.536000e+03
5.578874e+00 2.746250e+05 1.787923e+02 1.536000e+03
5.213555e+00 3.593700e+04 1.169824e+01 3.072000e+03
6.196141e+00 2.746250e+05 8.939616e+01 3.072000e+03
4.710436e+00 2.146689e+06 6.987920e+02 3.072000e+03
6.228164e+00 3.593700e+04 5.849121e+00 6.144000e+03
6.730721e+00 2.746250e+05 4.469808e+01 6.144000e+03
5.409885e+00 2.146689e+06 3.493960e+02 6.144000e+03
5.925955e+00 3.593700e+04 2.924561e+00 1.228800e+04
6.758160e+00 2.746250e+05 2.234904e+01 1.228800e+04
2.995390e+00 2.146689e+06 1.746980e+02 1.228800e+04
5.482122e+00 3.593700e+04 1.462280e+00 2.457600e+04
7.008359e+00 2.746250e+05 1.117452e+01 2.457600e+04
7.660121e+00 2.146689e+06 8.734900e+01 2.457600e+04
4.432930e+00 1.697459e+07 6.906980e+02 2.457600e+04
6.049578e+00 3.593700e+04 7.311401e-01 4.915200e+04
6.567448e+00 2.746250e+05 5.587260e+00 4.915200e+04
6.109877e+00 2.146689e+06 4.367450e+01 4.915200e+04
6.055037e+00 1.697459e+07 3.453490e+02 4.915200e+04
5.274549e+00 3.593700e+04 3.655701e-01 9.830400e+04
6.763671e+00 2.746250e+05 2.793630e+00 9.830400e+04
6.777736e+00 2.146689e+06 2.183725e+01 9.830400e+04
5.010740e+00 1.697459e+07 1.726745e+02 9.830400e+04
5.476099e+00 3.593700e+04 2.437134e-01 1.474560e+05
6.639628e+00 2.746250e+05 1.862420e+00 1.474560e+05
6.852369e+00 2.146689e+06 1.455817e+01 1.474560e+05
5.152772e+00 1.697459e+07 1.151163e+02 1.474560e+05
5.105059e+00 1.350057e+08 9.155660e+02 1.474560e+05


==> data/large-scaling/large-scaling-9-4/speedup_1.tex <==
speedup n_dofs n_dofs_norm ranks
1.155788e+00 2.746250e+05 5.721354e+03 4.800000e+01
1.846060e+00 2.746250e+05 2.860677e+03 9.600000e+01
3.112508e+00 2.746250e+05 1.430339e+03 1.920000e+02
1.573498e+00 2.146689e+06 5.590336e+03 3.840000e+02
2.699419e+00 2.146689e+06 2.795168e+03 7.680000e+02
3.675241e+00 2.146689e+06 1.397584e+03 1.536000e+03
1.854036e+00 1.697459e+07 5.525584e+03 3.072000e+03
3.659909e+00 1.697459e+07 2.762792e+03 6.144000e+03
2.951927e+00 1.697459e+07 1.381396e+03 1.228800e+04
2.328759e+00 1.350057e+08 5.493396e+03 2.457600e+04
4.945460e+00 1.350057e+08 2.746698e+03 4.915200e+04
4.574992e+00 1.350057e+08 1.373349e+03 9.830400e+04
1.800871e+00 1.076891e+09 7.303132e+03 1.474560e+05


==> data/large-scaling/large-scaling-9-4/speedup_2.tex <==
speedup n_dofs n_dofs_norm ranks
5.764321e-01 2.146689e+06 4.472269e+04 4.800000e+01
5.955301e-01 2.146689e+06 2.236134e+04 9.600000e+01
9.365403e-01 2.146689e+06 1.118067e+04 1.920000e+02
7.151473e-01 1.697459e+07 8.840934e+04 1.920000e+02
6.380190e-01 1.697459e+07 4.420467e+04 3.840000e+02
6.846402e-01 1.697459e+07 2.210233e+04 7.680000e+02
1.040928e+00 1.697459e+07 1.105117e+04 1.536000e+03
7.059666e-01 1.350057e+08 8.789433e+04 1.536000e+03
7.735197e-01 1.350057e+08 4.394717e+04 3.072000e+03
8.705555e-01 1.350057e+08 2.197358e+04 6.144000e+03
1.425437e+00 1.350057e+08 1.098679e+04 1.228800e+04
8.445290e-01 1.076891e+09 8.763758e+04 1.228800e+04
9.597504e-01 1.076891e+09 4.381879e+04 2.457600e+04
1.783763e+00 1.076891e+09 2.190940e+04 4.915200e+04
1.404894e+00 1.076891e+09 1.095470e+04 9.830400e+04
8.035743e-01 8.602524e+09 8.750940e+04 9.830400e+04
8.682318e-01 8.602524e+09 5.833960e+04 1.474560e+05


==> data/large-scaling/large-scaling-9-4/speedup_3.tex <==
speedup n_dofs n_dofs_norm ranks
7.195918e-01 1.697459e+07 1.768187e+05 9.600000e+01
7.568443e-01 1.350057e+08 1.757887e+05 7.680000e+02
8.220237e-01 1.076891e+09 1.752752e+05 6.144000e+03
1.033150e+00 8.602524e+09 1.750188e+05 4.915200e+04


==> data/large-scaling/speedup/speedup_0.tex <==
\begin{minipage}{0.23\textwidth}
\begin{tikzpicture}[thick,scale=0.7, every node/.style={scale=0.75}]
    \begin{semilogyaxis}[
      width=1.4\textwidth,
      height=1.2\textwidth,
      title style={font=\tiny},every axis title/.style={above left,at={(1,1)},draw=black,fill=white},
      %title={$Q=8$},
      xlabel={DoFs},
      ylabel={Time per iterations [sec]},
      legend pos={south west},
      legend cell align={left},
      cycle list name=colorGPL,
      grid,
      semithick,
      mark options={solid}
      ]
  
  \addplot+[only marks, red,every mark/.append style={fill=blue!80!black},mark=o] table [x=speedup,y=n_dofs] {data/large-scaling/large-scaling-2-1/speedup_0.tex};
  \addplot+[only marks, red,every mark/.append style={fill=blue!80!black},mark=x] table [x=speedup,y=n_dofs] {data/large-scaling/large-scaling-2-4/speedup_0.tex};

  \addplot+[only marks, blue,every mark/.append style={fill=blue!80!black},mark=x] table [x=speedup,y=n_dofs] {data/large-scaling/large-scaling-4-1/speedup_0.tex};
  \addplot+[only marks, blue,every mark/.append style={fill=blue!80!black},mark=x] table [x=speedup,y=n_dofs] {data/large-scaling/large-scaling-4-4/speedup_0.tex};

  \addplot+[only marks, orange,every mark/.append style={fill=blue!80!black},mark=o] table [x=speedup,y=n_dofs] {data/large-scaling/large-scaling-9-1/speedup_0.tex};
  \addplot+[only marks, orange,every mark/.append style={fill=blue!80!black},mark=x] table [x=speedup,y=n_dofs] {data/large-scaling/large-scaling-9-4/speedup_0.tex};

  %\addplot+[solid, blue,every mark/.append style={fill=blue!80!black},mark=x] table [x=dofs,y=t_1] {data/parameters-all/parameters-q/data_3.tex};
  %\addplot+[solid, orange,every mark/.append style={fill=orange!80!black},mark=square] table [x=dofs,y=t_2] {data/parameters-all/parameters-q/data_3.tex};
  
  
    \end{semilogyaxis}
\end{tikzpicture}
\end{minipage}

==> data/parameters-all/parameters-q/data_0.tex <==
dofs t_0 t_1 t_2 t_3 t_4 t_5 t_6
7.290000e+02 7.608556e-03 4.247333e-03 7.215222e-03 7.296556e-03 7.395000e-03 7.903778e-03 7.992333e-03
4.913000e+03 1.259111e-02 7.769556e-03 1.219889e-02 1.385667e-02 1.223667e-02 1.517111e-02 1.549222e-02
3.593700e+04 1.699889e-02 9.778556e-03 1.638778e-02 1.656000e-02 1.663333e-02 2.061000e-02 2.072667e-02
2.746250e+05 2.894556e-02 1.831111e-02 2.577444e-02 2.633222e-02 2.664556e-02 2.918889e-02 3.583889e-02
2.146689e+06 7.293444e-02 6.441222e-02 7.274111e-02 7.722222e-02 7.587889e-02 7.984111e-02 7.895556e-02
1.697459e+07 3.533111e-01 3.613111e-01 3.319444e-01 4.002444e-01 4.095111e-01 4.335111e-01 4.369000e-01
1.350057e+08 2.683889e+00 -1.111111e-01 -1.111111e-01 -1.111111e-01 -1.111111e-01 -1.111111e-01 -1.111111e-01


==> data/parameters-all/parameters-q/data_1.tex <==
dofs t_0 t_1 t_2 t_3 t_4 t_5 t_6
7.290000e+02 2.041000e-02 6.675444e-03 1.854667e-02 1.756111e-02 8.670444e-03 1.465778e-02 9.574667e-03
4.913000e+03 3.415000e-02 1.187778e-02 3.183889e-02 2.659222e-02 1.705111e-02 3.038222e-02 1.805556e-02
3.593700e+04 4.345000e-02 1.768444e-02 4.229333e-02 3.898889e-02 2.109889e-02 4.104333e-02 2.610000e-02
2.746250e+05 8.259000e-02 3.264444e-02 6.306333e-02 5.555111e-02 3.924111e-02 6.270778e-02 4.210333e-02
2.146689e+06 1.844889e-01 1.436889e-01 1.859333e-01 1.468111e-01 1.243667e-01 1.628889e-01 1.378444e-01
1.697459e+07 8.960556e-01 9.266111e-01 9.243444e-01 7.768111e-01 7.791778e-01 8.739111e-01 8.510889e-01


==> data/parameters-all/parameters-q/data_2.tex <==
dofs t_0 t_1 t_2 t_3 t_4 t_5 t_6
7.290000e+02 3.974000e-02 9.233667e-03 3.460778e-02 2.597778e-02 1.070711e-02 2.134667e-02 8.578222e-03
4.913000e+03 6.089222e-02 1.180556e-02 4.873778e-02 3.854222e-02 2.238889e-02 3.963778e-02 1.460667e-02
3.593700e+04 7.935667e-02 1.706111e-02 6.957667e-02 5.197889e-02 1.997667e-02 5.922778e-02 2.131111e-02
2.746250e+05 1.418222e-01 4.690111e-02 1.150111e-01 8.570889e-02 4.134222e-02 9.251778e-02 4.544222e-02
2.146689e+06 3.311222e-01 2.359111e-01 3.052111e-01 2.210889e-01 1.764778e-01 2.531444e-01 2.004889e-01
1.697459e+07 1.772444e+00 1.832222e+00 1.717222e+00 1.229222e+00 1.115222e+00 1.342333e+00 1.370222e+00


==> data/parameters-all/parameters-q/data_3.tex <==
dofs t_0 t_1 t_2 t_3 t_4 t_5 t_6
7.290000e+02 6.070222e-02 1.119000e-02 4.905333e-02 3.630444e-02 1.040300e-02 3.169556e-02 1.054433e-02
4.913000e+03 8.309000e-02 1.486778e-02 7.523333e-02 5.026333e-02 1.825778e-02 5.423222e-02 1.989667e-02
3.593700e+04 1.199444e-01 2.450111e-02 1.133000e-01 8.066778e-02 2.910889e-02 8.652111e-02 3.132444e-02
2.746250e+05 1.953667e-01 6.870333e-02 1.753000e-01 1.082511e-01 5.134556e-02 1.328778e-01 6.361556e-02
2.146689e+06 5.178111e-01 3.915778e-01 4.361889e-01 2.741222e-01 2.143556e-01 3.567667e-01 2.856333e-01
1.697459e+07 2.833778e+00 3.174667e+00 2.589444e+00 1.518444e+00 1.507667e+00 1.892222e+00 2.142333e+00


==> data/parameters-complex/parameters-q/data_0.tex <==
dofs throughput speedup t_irk t_spirk i_outer
7.290000e+02 9.596033e+04 9.802843e-01  7.447111e-03 7.596889e-03 6.000000e+00  1.400000e+01 1.400000e+01  1.400000e+01
4.913000e+03 3.933197e+05 1.005960e+00  1.256556e-02 1.249111e-02 6.000000e+00  1.400000e+01 1.400000e+01  1.400000e+01
3.593700e+04 1.879441e+06 9.872160e-01  1.887667e-02 1.912111e-02 6.000000e+00  1.400000e+01 1.400000e+01  1.400000e+01
2.746250e+05 9.381049e+06 9.984059e-01  2.922778e-02 2.927444e-02 6.000000e+00  1.400000e+01 1.400000e+01  1.400000e+01
2.146689e+06 3.009752e+07 9.964014e-01  7.106778e-02 7.132444e-02 6.000000e+00  1.400000e+01 1.400000e+01  1.400000e+01
1.697459e+07 4.280868e+07 9.927985e-01  3.936667e-01 3.965222e-01 6.000000e+00  1.400000e+01 1.400000e+01  1.400000e+01
1.350057e+08 5.092846e+07 1.019700e+00  2.703111e+00 2.650889e+00 5.111100e+00  1.222220e+01 1.222220e+01  1.222220e+01


==> data/parameters-complex/parameters-q/data_1.tex <==
dofs throughput speedup t_irk t_spirk i_outer
7.290000e+02 8.465806e+04 1.886452e+00  1.624444e-02 8.611111e-03 6.777800e+00  1.511110e+01 1.555560e+01  1.600000e+01
4.913000e+03 2.894351e+05 1.558552e+00  2.645556e-02 1.697444e-02 6.666700e+00  1.400000e+01 1.533330e+01  1.666670e+01
3.593700e+04 1.503361e+06 1.669564e+00  3.991000e-02 2.390444e-02 6.444400e+00  1.377780e+01 1.488890e+01  1.600000e+01
2.746250e+05 7.093402e+06 1.577230e+00  6.106333e-02 3.871556e-02 6.388900e+00  1.400000e+01 1.477780e+01  1.555560e+01
2.146689e+06 1.827661e+07 1.207454e+00  1.418222e-01 1.174556e-01 5.944400e+00  1.377780e+01 1.388890e+01  1.400000e+01
1.697459e+07 2.187542e+07 9.905924e-01  7.686667e-01 7.759667e-01 5.777800e+00  1.311110e+01 1.355560e+01  1.400000e+01
1.350057e+08 2.301844e+07 9.564089e-01  5.609444e+00 5.865111e+00 5.500000e+00  1.200000e+01 1.300000e+01  1.400000e+01


==> data/parameters-complex/parameters-q/data_2.tex <==
dofs throughput speedup t_irk t_spirk i_outer
7.290000e+02 6.849072e+04 2.419880e+00  2.575667e-02 1.064378e-02 7.333300e+00  1.600000e+01 1.666670e+01  1.800000e+01
4.913000e+03 2.826270e+05 2.419623e+00  4.206111e-02 1.738333e-02 7.000000e+00  1.400000e+01 1.600000e+01  1.800000e+01
3.593700e+04 1.594601e+06 2.591628e+00  5.840667e-02 2.253667e-02 6.333300e+00  1.400000e+01 1.466670e+01  1.600000e+01
2.746250e+05 5.553964e+06 1.664914e+00  8.232444e-02 4.944667e-02 6.333300e+00  1.400000e+01 1.466670e+01  1.600000e+01
2.146689e+06 1.162537e+07 1.221433e+00  2.255444e-01 1.846556e-01 6.185200e+00  1.400000e+01 1.437040e+01  1.511110e+01
1.697459e+07 1.453166e+07 1.012651e+00  1.182889e+00 1.168111e+00 6.074100e+00  1.400000e+01 1.414810e+01  1.444440e+01


==> data/parameters-complex/parameters-q/data_3.tex <==
dofs throughput speedup t_irk t_spirk i_outer
7.290000e+02 7.020867e+04 3.359444e+00  3.488222e-02 1.038333e-02 7.472200e+00  1.400000e+01 1.694440e+01  1.800000e+01
4.913000e+03 2.322321e+05 2.813550e+00  5.952222e-02 2.115556e-02 7.416700e+00  1.400000e+01 1.683330e+01  1.933330e+01
3.593700e+04 1.312954e+06 2.917878e+00  7.986556e-02 2.737111e-02 6.527800e+00  1.400000e+01 1.505560e+01  1.622220e+01
2.746250e+05 5.429756e+06 2.147825e+00  1.086322e-01 5.057778e-02 6.250000e+00  1.200000e+01 1.450000e+01  1.600000e+01
2.146689e+06 9.921023e+06 1.327719e+00  2.872889e-01 2.163778e-01 5.777800e+00  1.200000e+01 1.355560e+01  1.422220e+01
1.697459e+07 1.121504e+07 1.012994e+00  1.533222e+00 1.513556e+00 5.777800e+00  1.200000e+01 1.355560e+01  1.422220e+01


==> data/parameters-vt/0001/data_0.tex <==
dofs throughput speedup
7.290000e+02 3.840211e+04 1.000000e+00
4.913000e+03 1.512778e+05 1.000000e+00
3.593700e+04 5.618473e+05 1.000000e+00
2.746250e+05 1.018555e+06 1.000000e+00
2.146689e+06 1.141114e+06 1.000000e+00
1.697459e+07 1.229251e+06 1.000000e+00


==> data/parameters-vt/0001/data_1.tex <==
dofs throughput speedup
7.290000e+02 1.345625e+05 3.504040e+00
4.913000e+03 4.441554e+05 2.936024e+00
3.593700e+04 9.295120e+05 1.654386e+00
2.746250e+05 1.111642e+06 1.091392e+00
2.146689e+06 1.097302e+06 9.616062e-01


==> data/parameters-vt/0001/data_2.tex <==
dofs throughput speedup
7.290000e+02 1.482276e+05 3.859883e+00
4.913000e+03 4.444947e+05 2.938267e+00
3.593700e+04 9.338598e+05 1.662124e+00
2.746250e+05 1.101241e+06 1.081180e+00
2.146689e+06 1.143207e+06 1.001834e+00


==> data/parameters-vt/0001/data_3.tex <==
dofs throughput speedup
7.290000e+02 1.327439e+05 3.456683e+00
4.913000e+03 4.504630e+05 2.977720e+00
3.593700e+04 9.617681e+05 1.711796e+00
2.746250e+05 1.110543e+06 1.090313e+00
2.146689e+06 1.071796e+06 9.392544e-01


==> data/parameters-vt/0016/data_0.tex <==
dofs throughput speedup
7.290000e+02 3.353437e+04 1.000000e+00
4.913000e+03 1.379970e+05 1.000000e+00
3.593700e+04 6.896520e+05 1.000000e+00
2.746250e+05 3.410879e+06 1.000000e+00
2.146689e+06 1.075495e+07 1.000000e+00
1.697459e+07 1.800254e+07 1.000000e+00
1.350057e+08 1.946917e+07 1.000000e+00


==> data/parameters-vt/0016/data_1.tex <==
dofs throughput speedup
7.290000e+02 9.161744e+04 2.732046e+00
4.913000e+03 3.449333e+05 2.499571e+00
3.593700e+04 2.092605e+06 3.034291e+00
2.746250e+05 7.764348e+06 2.276348e+00
2.146689e+06 1.355518e+07 1.260366e+00
1.697459e+07 1.818988e+07 1.010406e+00


==> data/parameters-vt/0016/data_2.tex <==
dofs throughput speedup
7.290000e+02 1.158962e+05 3.456042e+00
4.913000e+03 4.165128e+05 3.018274e+00
3.593700e+04 2.266683e+06 3.286705e+00
2.746250e+05 7.636958e+06 2.239000e+00
2.146689e+06 1.484000e+07 1.379829e+00
1.697459e+07 1.795514e+07 9.973673e-01


==> data/parameters-vt/0016/data_3.tex <==
dofs throughput speedup
7.290000e+02 1.013846e+05 3.023303e+00
4.913000e+03 4.396202e+05 3.185723e+00
3.593700e+04 2.415843e+06 3.502988e+00
2.746250e+05 7.867659e+06 2.306637e+00
2.146689e+06 1.318065e+07 1.225542e+00
1.697459e+07 1.569348e+07 8.717372e-01


==> data/parameters-vt/0064/data_0.tex <==
dofs throughput speedup
7.290000e+02 3.703014e+04 1.000000e+00
4.913000e+03 1.458296e+05 1.000000e+00
3.593700e+04 7.265871e+05 1.000000e+00
2.746250e+05 4.130389e+06 1.000000e+00
2.146689e+06 1.970946e+07 1.000000e+00
1.697459e+07 5.188010e+07 1.000000e+00
1.350057e+08 4.050576e+07 1.000000e+00
1.076891e+09 4.151823e+07 1.000000e+00


==> data/parameters-vt/0064/data_1.tex <==
dofs throughput speedup
7.290000e+02 1.087519e+05 2.936847e+00
4.913000e+03 4.093409e+05 2.806980e+00
3.593700e+04 1.706680e+06 2.348900e+00
2.746250e+05 8.366478e+06 2.025591e+00
2.146689e+06 3.158754e+07 1.602658e+00
1.697459e+07 4.891500e+07 9.428471e-01
1.350057e+08 3.294072e+07 8.132354e-01


==> data/parameters-vt/0064/data_2.tex <==
dofs throughput speedup
7.290000e+02 1.153846e+05 3.115965e+00
4.913000e+03 4.159643e+05 2.852399e+00
3.593700e+04 1.690799e+06 2.327043e+00
2.746250e+05 9.079846e+06 2.198303e+00
2.146689e+06 3.614022e+07 1.833648e+00
1.697459e+07 3.046835e+07 5.872839e-01
1.350057e+08 3.379743e+07 8.343857e-01


==> data/parameters-vt/0064/data_3.tex <==
dofs throughput speedup
7.290000e+02 1.030405e+05 2.782611e+00
4.913000e+03 4.523432e+05 3.101861e+00
3.593700e+04 2.578594e+06 3.548912e+00
2.746250e+05 1.248800e+07 3.023444e+00
2.146689e+06 2.035076e+07 1.032538e+00
1.697459e+07 2.902632e+07 5.594885e-01
1.350057e+08 3.141210e+07 7.754970e-01


==> data/parameters-vt/data_0.tex <==
dofs throughput speedup
7.290000e+02 3.601067e+04 1.000000e+00
4.913000e+03 1.838973e+05 1.000000e+00
3.593700e+04 9.640270e+05 1.000000e+00
2.746250e+05 4.055960e+06 1.000000e+00
2.146689e+06 1.109171e+07 1.000000e+00
1.697459e+07 1.633901e+07 1.000000e+00


==> data/parameters-vt/data_1.tex <==
dofs throughput speedup
7.290000e+02 1.309150e+05 3.635449e+00
4.913000e+03 5.312960e+05 2.889091e+00
3.593700e+04 2.727045e+06 2.828806e+00
2.746250e+05 7.730689e+06 1.906007e+00
2.146689e+06 1.178981e+07 1.062939e+00
1.697459e+07 1.427756e+07 8.738330e-01


==> data/parameters-vt/data_2.tex <==
dofs throughput speedup
7.290000e+02 1.238911e+05 3.440400e+00
4.913000e+03 5.264963e+05 2.862991e+00
3.593700e+04 2.722088e+06 2.823663e+00
2.746250e+05 7.562094e+06 1.864440e+00
2.146689e+06 1.223812e+07 1.103358e+00
1.697459e+07 1.476565e+07 9.037056e-01


==> data/parameters-vt/data_3.tex <==
dofs throughput speedup
7.290000e+02 1.261137e+05 3.502119e+00
4.913000e+03 5.688186e+05 3.093132e+00
3.593700e+04 2.791657e+06 2.895828e+00
2.746250e+05 7.528510e+06 1.856160e+00
2.146689e+06 1.184903e+07 1.068278e+00
1.697459e+07 1.350620e+07 8.266232e-01


==> data/parameters/parameters-dt/data_0.tex <==
dofs throughput speedup t_irk t_spirk i_outer
7.290000e+02 5.529849e+04 3.339376e+00  4.402300e-02 1.318300e-02 8.000000e+00  3.875000e+00 3.968800e+00  4.000000e+00
4.913000e+03 1.814120e+05 2.969242e+00  8.041300e-02 2.708200e-02 9.000000e+00  4.000000e+00 4.000000e+00  4.000000e+00
3.593700e+04 7.815619e+05 2.769405e+00  1.273400e-01 4.598100e-02 1.000000e+01  3.600000e+00 3.700000e+00  4.000000e+00
2.746250e+05 3.466656e+06 2.026029e+00  1.605000e-01 7.921900e-02 8.000000e+00  3.500000e+00 3.625000e+00  4.000000e+00
2.146689e+06 6.584128e+06 1.245737e+00  4.061600e-01 3.260400e-01 7.000000e+00  3.428600e+00 3.714300e+00  4.000000e+00
1.697459e+07 6.657486e+06 1.017610e+00  2.594600e+00 2.549700e+00 7.000000e+00  4.000000e+00 4.142900e+00  4.571400e+00


==> data/parameters/parameters-dt/data_1.tex <==
dofs throughput speedup t_irk t_spirk i_outer
7.290000e+02 5.068836e+04 2.978098e+00  4.283100e-02 1.438200e-02 7.900000e+00  3.379700e+00 3.946200e+00  4.506300e+00
4.913000e+03 2.086200e+05 2.980382e+00  7.018800e-02 2.355000e-02 8.000000e+00  4.000000e+00 4.000000e+00  4.000000e+00
3.593700e+04 1.139013e+06 3.087287e+00  9.740700e-02 3.155100e-02 7.000000e+00  4.000000e+00 4.000000e+00  4.000000e+00
2.746250e+05 3.977767e+06 2.157879e+00  1.489800e-01 6.904000e-02 6.000000e+00  4.000000e+00 4.541700e+00  4.833300e+00
2.146689e+06 6.470413e+06 1.276276e+00  4.234300e-01 3.317700e-01 6.000000e+00  4.000000e+00 4.537500e+00  4.816700e+00
1.697459e+07 8.070457e+06 1.029477e+00  2.165300e+00 2.103300e+00 5.000000e+00  4.800000e+00 4.900000e+00  5.000000e+00


==> data/parameters/parameters-dt/data_2.tex <==
dofs throughput speedup t_irk t_spirk i_outer
7.290000e+02 9.115007e+04 3.415064e+00  2.731300e-02 7.997800e-03 4.000000e+00  5.000000e+00 5.000000e+00  5.000000e+00
4.913000e+03 2.317344e+05 2.785765e+00  5.906100e-02 2.120100e-02 5.900000e+00  4.000000e+00 4.584700e+00  4.847500e+00
3.593700e+04 1.170129e+06 2.866013e+00  8.802100e-02 3.071200e-02 6.000000e+00  4.000000e+00 4.337500e+00  4.666700e+00
2.746250e+05 5.453020e+06 2.163337e+00  1.089500e-01 5.036200e-02 4.000000e+00  5.000000e+00 5.000000e+00  5.000000e+00
2.146689e+06 7.197857e+06 1.268911e+00  3.784400e-01 2.982400e-01 5.000000e+00  5.000000e+00 5.000000e+00  5.000000e+00
1.697459e+07 8.306221e+06 1.022167e+00  2.088900e+00 2.043600e+00 5.000000e+00  4.800000e+00 4.850000e+00  4.900000e+00


==> data/parameters/parameters-dt/data_3.tex <==
dofs throughput speedup t_irk t_spirk i_outer
7.290000e+02 1.106742e+05 3.315368e+00  2.183800e-02 6.586900e-03 4.000000e+00  3.875000e+00 3.931200e+00  4.000000e+00
4.913000e+03 3.227565e+05 3.138549e+00  4.777500e-02 1.522200e-02 4.000000e+00  5.025000e+00 5.137500e+00  5.175000e+00
3.593700e+04 1.589359e+06 2.703507e+00  6.112900e-02 2.261100e-02 4.000000e+00  4.000000e+00 4.500000e+00  5.000000e+00
2.746250e+05 5.286944e+06 2.182735e+00  1.133800e-01 5.194400e-02 4.000000e+00  5.200000e+00 5.218800e+00  5.225000e+00
2.146689e+06 8.698796e+06 1.274414e+00  3.145000e-01 2.467800e-01 4.000000e+00  5.075000e+00 5.093800e+00  5.100000e+00
1.697459e+07 9.748230e+06 1.029288e+00  1.792300e+00 1.741300e+00 4.000000e+00  5.075000e+00 5.093800e+00  5.100000e+00


==> data/parameters/parameters-dt/data_4.tex <==
dofs throughput speedup t_irk t_spirk i_outer
7.290000e+02 1.312166e+05 3.331533e+00  1.850900e-02 5.555700e-03 3.300000e+00  4.060600e+00 4.060600e+00  4.060600e+00
4.913000e+03 3.991064e+05 2.913160e+00  3.586100e-02 1.231000e-02 3.200000e+00  5.031200e+00 5.195300e+00  5.250000e+00
3.593700e+04 2.304540e+06 2.893998e+00  4.512900e-02 1.559400e-02 3.000000e+00  4.400000e+00 4.516700e+00  4.633300e+00
2.746250e+05 7.263866e+06 2.136536e+00  8.077600e-02 3.780700e-02 2.900000e+00  5.241400e+00 5.241400e+00  5.241400e+00
2.146689e+06 1.186082e+07 1.285430e+00  2.326500e-01 1.809900e-01 2.900000e+00  5.241400e+00 5.258600e+00  5.310300e+00
1.697459e+07 1.271696e+07 9.901858e-01  1.321700e+00 1.334800e+00 2.900000e+00  5.241400e+00 5.267200e+00  5.310300e+00


==> data/parameters/parameters-dt/plot_speedup.tex <==
 \begin{tikzpicture}[thick,scale=0.7, every node/.style={scale=0.9}]
    \begin{semilogxaxis}[
      width=1.45\textwidth,
      height=1.2\textwidth,
      title style={font=\tiny},every axis title/.style={above left,at={(1,1)},draw=black,fill=white},
      xlabel={DoFs},
      ylabel={Speedup},
      legend pos={south west},
      legend cell align={left},
      cycle list name=colorGPL,
      grid,
      semithick,
      mark options={solid}
      ]

\addplot+[solid, orange,every mark/.append style={fill=gnuplot@darkblue!80!black},mark=o] table [x=dofs,y=speedup] {data/parameters/parameters-dt/data_0.tex};
\addplot+[solid, gnuplot@darkblue,every mark/.append style={fill=gnuplot@darkblue!80!black},mark=square*] table [x=dofs,y=speedup] {data/parameters/parameters-dt/data_1.tex};
\addplot+[solid, gnuplot@red,every mark/.append style={fill=gnuplot@darkblue!80!black},mark=x] table [x=dofs,y=speedup] {data/parameters/parameters-dt/data_2.tex};
\addplot+[solid, gnuplot@green,every mark/.append style={fill=gnuplot@darkblue!80!black},mark=triangle] table [x=dofs,y=speedup] {data/parameters/parameters-dt/data_3.tex};
%\addplot+[solid, magenta,every mark/.append style={fill=gnuplot@darkblue!80!black},mark=x] table [x=dofs,y=speedup] {data/parameters/parameters-dt/data_4.tex};


    \end{semilogxaxis}
\end{tikzpicture}


==> data/parameters/parameters-dt/plot_throughput.tex <==
 \begin{tikzpicture}[thick,scale=0.7, every node/.style={scale=0.9}]
    \begin{semilogxaxis}[
      width=1.45\textwidth,
      height=1.2\textwidth,
      title style={font=\tiny},every axis title/.style={above left,at={(1,1)},draw=black,fill=white},
      xlabel={DoFs},
      ylabel={Throughput [DoFs/s/it]},
      legend pos={south west},
      legend cell align={left},
      cycle list name=colorGPL,
      grid,
      semithick,
      mark options={solid}
      ]

\addplot+[solid, orange,every mark/.append style={fill=gnuplot@darkblue!80!black},mark=o] table [x=dofs,y=throughput] {data/parameters/parameters-dt/data_0.tex};
\addplot+[solid, gnuplot@darkblue,every mark/.append style={fill=gnuplot@darkblue!80!black},mark=square*] table [x=dofs,y=throughput] {data/parameters/parameters-dt/data_1.tex};
\addplot+[solid, gnuplot@red,every mark/.append style={fill=gnuplot@darkblue!80!black},mark=triangle] table [x=dofs,y=throughput] {data/parameters/parameters-dt/data_2.tex};
\addplot+[solid, gnuplot@green,every mark/.append style={fill=gnuplot@darkblue!80!black},mark=x] table [x=dofs,y=throughput] {data/parameters/parameters-dt/data_3.tex};
%\addplot+[solid, magenta,every mark/.append style={fill=gnuplot@darkblue!80!black},mark=x] table [x=dofs,y=throughput] {data/parameters/parameters-dt/data_4.tex};


    \end{semilogxaxis}
\end{tikzpicture}


==> data/parameters/parameters-p/data_0.tex <==
dofs throughput speedup t_irk t_spirk i_outer
7.290000e+02 1.100913e+05 3.034432e+00  2.009333e-02 6.621778e-03 8.888900e+00  9.888900e+00 9.888900e+00  9.888900e+00
4.913000e+03 4.055117e+05 2.856842e+00  3.461222e-02 1.211556e-02 8.888900e+00  9.888900e+00 9.888900e+00  9.888900e+00
3.593700e+04 2.169090e+06 2.871773e+00  4.757889e-02 1.656778e-02 7.888900e+00  8.888900e+00 8.888900e+00  8.888900e+00
2.746250e+05 8.909325e+06 2.864790e+00  8.830556e-02 3.082444e-02 7.888900e+00  8.888900e+00 8.888900e+00  8.888900e+00
2.146689e+06 1.281605e+07 1.314760e+00  2.202222e-01 1.675000e-01 7.888900e+00  8.888900e+00 8.888900e+00  8.888900e+00
1.697459e+07 1.607206e+07 1.005870e+00  1.062356e+00 1.056156e+00 7.000000e+00  8.000000e+00 8.000000e+00  8.000000e+00


==> data/parameters/parameters-p/data_1.tex <==
dofs throughput speedup t_irk t_spirk i_outer
4.913000e+03 6.308243e+05 2.967158e+00  2.310889e-02 7.788222e-03 8.888900e+00  9.888900e+00 9.888900e+00  9.888900e+00
3.593700e+04 2.844117e+06 2.799859e+00  3.537778e-02 1.263556e-02 8.000000e+00  9.000000e+00 9.000000e+00  9.000000e+00
2.746250e+05 1.268346e+07 2.688562e+00  5.821333e-02 2.165222e-02 8.000000e+00  9.000000e+00 9.000000e+00  9.000000e+00
2.146689e+06 3.485136e+07 1.694278e+00  1.043600e-01 6.159556e-02 8.000000e+00  9.000000e+00 9.000000e+00  9.000000e+00
1.697459e+07 3.337076e+07 9.437746e-01  4.800667e-01 5.086667e-01 8.000000e+00  9.000000e+00 9.000000e+00  9.000000e+00
1.350057e+08 2.898293e+07 8.595282e-01  4.003778e+00 4.658111e+00 8.000000e+00  9.000000e+00 9.000000e+00  9.000000e+00


==> data/parameters/parameters-p/data_2.tex <==
dofs throughput speedup t_irk t_spirk i_outer
1.562500e+04 1.681534e+06 3.115666e+00  2.895111e-02 9.292111e-03 9.000000e+00  1.000000e+01 1.000000e+01  1.000000e+01
1.176490e+05 6.875144e+06 2.933316e+00  5.019556e-02 1.711222e-02 9.000000e+00  1.000000e+01 1.000000e+01  1.000000e+01
9.126730e+05 2.597659e+07 2.531134e+00  8.893000e-02 3.513444e-02 9.000000e+00  1.000000e+01 1.000000e+01  1.000000e+01
7.189057e+06 4.305971e+07 1.175429e+00  1.962444e-01 1.669556e-01 9.000000e+00  1.000000e+01 1.000000e+01  1.000000e+01
5.706662e+07 2.971017e+07 7.768265e-01  1.492111e+00 1.920778e+00 9.000000e+00  1.000000e+01 1.000000e+01  1.000000e+01


==> data/parameters/parameters-p/data_3.tex <==
dofs throughput speedup t_irk t_spirk i_outer
3.593700e+04 2.421449e+06 2.988920e+00  4.435889e-02 1.484111e-02 9.888900e+00  1.088890e+01 1.088890e+01  1.088890e+01
2.746250e+05 1.100848e+07 3.301933e+00  8.237222e-02 2.494667e-02 9.000000e+00  1.000000e+01 1.000000e+01  1.000000e+01
2.146689e+06 3.738140e+07 2.554369e+00  1.466889e-01 5.742667e-02 9.000000e+00  1.000000e+01 1.000000e+01  1.000000e+01
1.697459e+07 3.940046e+07 9.758601e-01  4.204222e-01 4.308222e-01 9.000000e+00  1.000000e+01 1.000000e+01  1.000000e+01
1.350057e+08 3.141697e+07 9.107692e-01  3.913778e+00 4.297222e+00 9.000000e+00  1.000000e+01 1.000000e+01  1.000000e+01


==> data/parameters/parameters-q/data_0.tex <==
dofs throughput speedup t_irk t_spirk i_outer
7.290000e+02 1.662233e+05 1.779053e+00  7.802333e-03 4.385667e-03 6.000000e+00  7.000000e+00 7.000000e+00  7.000000e+00
4.913000e+03 6.343993e+05 1.868893e+00  1.447333e-02 7.744333e-03 6.000000e+00  7.000000e+00 7.000000e+00  7.000000e+00
3.593700e+04 3.183082e+06 1.791261e+00  2.022333e-02 1.129000e-02 6.000000e+00  7.000000e+00 7.000000e+00  7.000000e+00
2.746250e+05 1.529376e+07 1.550832e+00  2.784778e-02 1.795667e-02 6.000000e+00  7.000000e+00 7.000000e+00  7.000000e+00
2.146689e+06 3.193897e+07 1.157346e+00  7.778778e-02 6.721222e-02 5.888900e+00  6.888900e+00 6.888900e+00  6.888900e+00
1.697459e+07 4.690122e+07 9.874129e-01  3.573667e-01 3.619222e-01 5.000000e+00  6.000000e+00 6.000000e+00  6.000000e+00
1.350057e+08 4.859039e+07 9.517716e-01  2.644444e+00 2.778444e+00 5.000000e+00  6.000000e+00 6.000000e+00  6.000000e+00


==> data/parameters/parameters-q/data_1.tex <==
dofs throughput speedup t_irk t_spirk i_outer
7.290000e+02 8.440539e+04 2.423455e+00  2.093111e-02 8.636889e-03 8.888900e+00  9.888900e+00 9.888900e+00  9.888900e+00
4.913000e+03 3.860735e+05 2.916005e+00  3.710778e-02 1.272556e-02 8.888900e+00  9.888900e+00 9.888900e+00  9.888900e+00
3.593700e+04 2.074219e+06 2.957673e+00  5.124333e-02 1.732556e-02 7.888900e+00  8.888900e+00 8.888900e+00  8.888900e+00
2.746250e+05 8.810555e+06 2.781948e+00  8.671333e-02 3.117000e-02 7.888900e+00  8.888900e+00 8.888900e+00  8.888900e+00
2.146689e+06 1.353808e+07 1.194731e+00  1.894444e-01 1.585667e-01 7.888900e+00  8.888900e+00 8.888900e+00  8.888900e+00
1.697459e+07 1.857357e+07 1.019817e+00  9.320222e-01 9.139111e-01 7.000000e+00  8.000000e+00 8.000000e+00  8.000000e+00


==> data/parameters/parameters-q/data_2.tex <==
dofs throughput speedup t_irk t_spirk i_outer
7.290000e+02 6.883419e+04 3.927777e+00  4.159778e-02 1.059067e-02 1.188890e+01  1.288890e+01 1.288890e+01  1.288890e+01
4.913000e+03 3.351296e+05 4.503335e+00  6.601889e-02 1.466000e-02 1.100000e+01  1.200000e+01 1.200000e+01  1.200000e+01
3.593700e+04 1.646221e+06 4.203695e+00  9.176667e-02 2.183000e-02 9.888900e+00  1.088890e+01 1.088890e+01  1.088890e+01
2.746250e+05 6.055530e+06 2.844718e+00  1.290111e-01 4.535111e-02 9.888900e+00  1.088890e+01 1.088890e+01  1.088890e+01
2.146689e+06 8.824024e+06 1.394839e+00  3.393333e-01 2.432778e-01 9.888900e+00  1.088890e+01 1.088890e+01  1.088890e+01
1.697459e+07 9.257747e+06 9.863653e-01  1.808556e+00 1.833556e+00 9.888900e+00  1.088890e+01 1.088890e+01  1.088890e+01


==> data/parameters/parameters-q/data_3.tex <==
dofs throughput speedup t_irk t_spirk i_outer
7.290000e+02 5.950481e+04 5.353981e+00  6.559222e-02 1.225111e-02 1.400000e+01  1.500000e+01 1.500000e+01  1.500000e+01
4.913000e+03 2.581261e+05 5.462989e+00  1.039789e-01 1.903333e-02 1.300000e+01  1.400000e+01 1.400000e+01  1.400000e+01
3.593700e+04 1.290892e+06 5.158651e+00  1.436111e-01 2.783889e-02 1.188890e+01  1.288890e+01 1.288890e+01  1.288890e+01
2.746250e+05 4.084993e+06 2.990497e+00  2.010444e-01 6.722778e-02 1.188890e+01  1.288890e+01 1.288890e+01  1.288890e+01
2.146689e+06 5.864024e+06 1.440981e+00  5.275111e-01 3.660778e-01 1.188890e+01  1.288890e+01 1.288890e+01  1.288890e+01
1.697459e+07 5.360210e+06 8.970562e-01  2.840778e+00 3.166778e+00 1.188890e+01  1.288890e+01 1.288890e+01  1.288890e+01


==> data/parameters/parameters-tolerance/data_0.tex <==
dofs throughput speedup t_irk t_spirk i_outer
7.290000e+02 1.726220e+05 3.100566e+00  1.309400e-02 4.223100e-03 8.900000e+00  1.112400e+00 1.112400e+00  1.112400e+00
4.913000e+03 6.208770e+05 2.678251e+00  2.119300e-02 7.913000e-03 9.000000e+00  1.111100e+00 1.111100e+00  1.111100e+00
3.593700e+04 2.956561e+06 2.689017e+00  3.268500e-02 1.215500e-02 8.900000e+00  1.112400e+00 1.112400e+00  1.112400e+00
2.746250e+05 1.011473e+07 2.015985e+00  5.473600e-02 2.715100e-02 8.900000e+00  1.112400e+00 1.112400e+00  1.112400e+00
2.146689e+06 1.710373e+07 1.228189e+00  1.541500e-01 1.255100e-01 8.000000e+00  1.125000e+00 1.125000e+00  1.125000e+00
1.697459e+07 1.868523e+07 9.763994e-01  8.870100e-01 9.084500e-01 8.000000e+00  1.125000e+00 1.125000e+00  1.125000e+00


==> data/parameters/parameters-tolerance/data_1.tex <==
dofs throughput speedup t_irk t_spirk i_outer
7.290000e+02 1.314722e+05 3.059027e+00  1.696200e-02 5.544900e-03 9.400000e+00  1.106400e+00 1.106400e+00  1.106400e+00
4.913000e+03 5.470194e+05 2.794442e+00  2.509800e-02 8.981400e-03 9.000000e+00  1.111100e+00 1.111100e+00  1.111100e+00
3.593700e+04 2.700812e+06 2.799865e+00  3.725500e-02 1.330600e-02 8.900000e+00  1.112400e+00 1.112400e+00  1.112400e+00
2.746250e+05 7.883141e+06 1.792003e+00  6.242800e-02 3.483700e-02 9.000000e+00  1.111100e+00 1.111100e+00  1.111100e+00
2.146689e+06 1.472958e+07 1.263963e+00  1.842100e-01 1.457400e-01 8.900000e+00  1.112400e+00 1.112400e+00  1.112400e+00
1.697459e+07 1.550758e+07 9.487484e-01  1.038500e+00 1.094600e+00 9.000000e+00  1.111100e+00 1.111100e+00  1.111100e+00


==> data/parameters/parameters-tolerance/data_2.tex <==
dofs throughput speedup t_irk t_spirk i_outer
7.290000e+02 9.290293e+04 2.748474e+00  2.156700e-02 7.846900e-03 9.000000e+00  1.211100e+00 1.552800e+00  1.733300e+00
4.913000e+03 3.870332e+05 2.358280e+00  2.993600e-02 1.269400e-02 9.000000e+00  1.200000e+00 1.369400e+00  1.555600e+00
3.593700e+04 2.065938e+06 2.638747e+00  4.590100e-02 1.739500e-02 8.000000e+00  1.125000e+00 1.600000e+00  1.762500e+00
2.746250e+05 6.625452e+06 2.172425e+00  9.004700e-02 4.145000e-02 6.900000e+00  2.275400e+00 2.286200e+00  2.289900e+00
2.146689e+06 1.019514e+07 1.243921e+00  2.619200e-01 2.105600e-01 6.900000e+00  2.144900e+00 2.221000e+00  2.289900e+00
1.697459e+07 1.199279e+07 1.012505e+00  1.433100e+00 1.415400e+00 7.100000e+00  2.126800e+00 2.133800e+00  2.140800e+00


==> data/parameters/parameters-tolerance/data_3.tex <==
dofs throughput speedup t_irk t_spirk i_outer
7.290000e+02 9.109539e+04 3.219954e+00  2.576800e-02 8.002600e-03 7.800000e+00  2.256400e+00 2.256400e+00  2.256400e+00
4.913000e+03 3.115409e+05 2.749588e+00  4.336100e-02 1.577000e-02 8.900000e+00  1.797800e+00 2.118000e+00  2.224700e+00
3.593700e+04 1.894912e+06 2.895070e+00  5.490500e-02 1.896500e-02 6.900000e+00  2.289900e+00 2.289900e+00  2.289900e+00
2.746250e+05 6.609825e+06 2.165110e+00  8.995600e-02 4.154800e-02 6.900000e+00  2.289900e+00 2.289900e+00  2.289900e+00
2.146689e+06 1.057378e+07 1.270023e+00  2.578400e-01 2.030200e-01 6.900000e+00  2.289900e+00 2.289900e+00  2.289900e+00
1.697459e+07 1.161848e+07 1.012526e+00  1.479300e+00 1.461000e+00 6.900000e+00  2.289900e+00 2.289900e+00  2.289900e+00


==> data/parameters/parameters-tolerance/data_4.tex <==
dofs throughput speedup t_irk t_spirk i_outer
7.290000e+02 8.331143e+04 3.048810e+00  2.667800e-02 8.750300e-03 7.800000e+00  2.256400e+00 2.339700e+00  2.448700e+00
4.913000e+03 3.399294e+05 2.862036e+00  4.136500e-02 1.445300e-02 7.900000e+00  2.253200e+00 2.303800e+00  2.354400e+00
3.593700e+04 1.564996e+06 2.785002e+00  6.395200e-02 2.296300e-02 6.900000e+00  2.565200e+00 2.713800e+00  2.869600e+00
2.746250e+05 5.976605e+06 2.094864e+00  9.625900e-02 4.595000e-02 6.900000e+00  2.289900e+00 2.474600e+00  2.565200e+00
2.146689e+06 7.693950e+06 1.286871e+00  3.590500e-01 2.790100e-01 7.000000e+00  2.700000e+00 3.028600e+00  3.400000e+00
1.697459e+07 9.238879e+06 9.431231e-01  1.732800e+00 1.837300e+00 6.100000e+00  2.672100e+00 3.155700e+00  3.327900e+00


==> data/parameters/parameters-tolerance/plot_speedup.tex <==
 \begin{tikzpicture}[thick,scale=0.7, every node/.style={scale=0.9}]
    \begin{semilogxaxis}[
      width=1.45\textwidth,
      height=1.2\textwidth,
      title style={font=\tiny},every axis title/.style={above left,at={(1,1)},draw=black,fill=white},
      xlabel={DoFs},
      ylabel={Speedup},
      legend pos={south west},
      legend cell align={left},
      cycle list name=colorGPL,
      grid,
      semithick,
      mark options={solid}
      ]

\addplot+[solid, orange,every mark/.append style={fill=gnuplot@darkblue!80!black},mark=o] table [x=dofs,y=speedup] {data/parameters/parameters-tolerance/data_0.tex};
\addplot+[solid, gnuplot@darkblue,every mark/.append style={fill=gnuplot@darkblue!80!black},mark=square*] table [x=dofs,y=speedup] {data/parameters/parameters-tolerance/data_1.tex};
\addplot+[solid, gnuplot@red,every mark/.append style={fill=gnuplot@darkblue!80!black},mark=x] table [x=dofs,y=speedup] {data/parameters/parameters-tolerance/data_2.tex};
\addplot+[solid, gnuplot@green,every mark/.append style={fill=gnuplot@darkblue!80!black},mark=triangle] table [x=dofs,y=speedup] {data/parameters/parameters-tolerance/data_3.tex};
%\addplot+[solid, magenta,every mark/.append style={fill=gnuplot@darkblue!80!black},mark=x] table [x=dofs,y=speedup] {data/parameters/parameters-tolerance/data_4.tex};


    \end{semilogxaxis}
\end{tikzpicture}


==> data/parameters/parameters-tolerance/plot_throughput.tex <==
 \begin{tikzpicture}[thick,scale=0.7, every node/.style={scale=0.9}]
    \begin{semilogxaxis}[
      width=1.4\textwidth,
      height=1.2\textwidth,
      title style={font=\tiny},every axis title/.style={above left,at={(1,1)},draw=black,fill=white},
      xlabel={DoFs},
      ylabel={Throughput [DoFs/s/it]},
      legend pos={south west},
      legend cell align={left},
      cycle list name=colorGPL,
      grid,
      semithick,
      mark options={solid}
      ]

\addplot+[solid, orange,every mark/.append style={fill=gnuplot@darkblue!80!black},mark=o] table [x=dofs,y=throughput] {data/parameters/parameters-tolerance/data_0.tex};
\addplot+[solid, gnuplot@darkblue,every mark/.append style={fill=gnuplot@darkblue!80!black},mark=square*] table [x=dofs,y=throughput] {data/parameters/parameters-tolerance/data_1.tex};
\addplot+[solid, gnuplot@red,every mark/.append style={fill=gnuplot@darkblue!80!black},mark=x] table [x=dofs,y=throughput] {data/parameters/parameters-tolerance/data_2.tex};
\addplot+[solid, gnuplot@green,every mark/.append style={fill=gnuplot@darkblue!80!black},mark=triangle] table [x=dofs,y=throughput] {data/parameters/parameters-tolerance/data_3.tex};
%\addplot+[solid, magenta,every mark/.append style={fill=gnuplot@darkblue!80!black},mark=x] table [x=dofs,y=throughput] {data/parameters/parameters-tolerance/data_4.tex};


    \end{semilogxaxis}
\end{tikzpicture}


==> data/small-scaling/data_0.tex <==
dofs time throughput speedup
7.290000e+02 6.646556e-03 1.096809e+05 2.998713e+00
4.913000e+03 1.162778e-02 4.225227e+05 3.121930e+00
3.593700e+04 1.616222e-02 2.223518e+06 3.206723e+00
2.746250e+05 3.343111e-02 8.214654e+06 3.450545e+00
2.146689e+06 1.455556e-01 1.474825e+07 3.437481e+00
1.697459e+07 9.284667e-01 1.828239e+07 3.675714e+00


==> data/small-scaling/data_1.tex <==
dofs time throughput speedup
7.290000e+02 2.015667e-02 3.616669e+04 9.888099e-01
4.913000e+03 3.416333e-02 1.438092e+05 1.062575e+00
3.593700e+04 4.805889e-02 7.477701e+05 1.078422e+00
2.746250e+05 7.439111e-02 3.691637e+06 1.550663e+00
2.146689e+06 1.804889e-01 1.189375e+07 2.772162e+00
1.697459e+07 9.115111e-01 1.862248e+07 3.744088e+00


==> data/small-scaling/data_2.tex <==
dofs time throughput speedup
7.290000e+02 1.993111e-02 3.657598e+04 1.000000e+00
4.913000e+03 3.630111e-02 1.353402e+05 1.000000e+00
3.593700e+04 5.182778e-02 6.933926e+05 1.000000e+00
2.746250e+05 1.153556e-01 2.380683e+06 1.000000e+00
2.146689e+06 5.003444e-01 4.290422e+06 1.000000e+00
1.697459e+07 3.412778e+00 4.973835e+06 1.000000e+00

